Seeing Double: ASASSN-18bt Exhibits a Two-Component Rise in the Early-Time K2 Light Curve

On 2018 Feb. 4.41, the All-Sky Automated Survey for SuperNovae (ASAS-SN) discovered ASASSN-18bt in the K2 Campaign 16 field. With a redshift of z=0.01098 and a peak apparent magnitude of B_{max}=14.31, ASASSN-18bt is the nearest and brightest SNe Ia yet observed by the Kepler spacecraft. Here we present the discovery of ASASSN-18bt, the K2 light curve, and pre-discovery data from ASAS-SN and the Asteroid Terrestrial-impact Last Alert System (ATLAS). The K2 early-time light curve has an unprecedented 30-minute cadence and photometric precision for an SN~Ia light curve, and it unambiguously shows a ~4 day nearly linear phase followed by a steeper rise. Thus, ASASSN-18bt joins a growing list of SNe Ia whose early light curves are not well described by a single power law. We show that a double-power-law model fits the data reasonably well, hinting that two physical processes must be responsible for the observed rise. However, we find that current models of the interaction with a non-degenerate companion predict an abrupt rise and cannot adequately explain the initial, slower linear phase. Instead, we find that existing, published models with shallow 56Ni are able to span the observed behavior and, with tuning, may be able to reproduce the ASASSN-18bt light curve. Regardless, more theoretical work is needed to satisfactorily model this and other early-time SNe~Ia light curves. Finally, we use Swift X-ray non-detections to constrain the presence of circumstellar material (CSM) at much larger distances and lower densities than possible with the optical light curve. For a constant density CSM these non-detections constrain rho<4.5 * 10^5 cm^-3 at a radius of 4 *10^15 cm from the progenitor star. Assuming a wind-like environment, we place mass-loss limits of Mdot< 8 * 10^-6 M_sun yr^-1 for v_w=100 km s^-1, ruling out some symbiotic progenitor systems.

==> tabphot_long.tex <==
\begin{deluxetable}{lrcc}
\tablewidth{210pt}
\tablecaption{Photometric Observations}
\tablehead{
\colhead{JD} &
\colhead{Band} &
\colhead{Magnitude} &
\colhead{Telescope} \\ 
\colhead{($-$2,450,000)} &
\colhead{} &
\colhead{}  &
\colhead{}  }
\startdata
8105.761 & $g$ & >18.69 & ASAS-SN/bi \\ 
8106.780 & $g$ & >19.16 & ASAS-SN/bi \\ 
8107.758 & $g$ & >18.91 & ASAS-SN/bi \\ 
8108.773 & $g$ & >18.84 & ASAS-SN/bi \\ 
8108.887 & $g$ & >19.20 & ASAS-SN/bq \\ 
8109.884 & $g$ & >19.10 & ASAS-SN/bq \\ 
8113.847 & $g$ & >19.33 & ASAS-SN/bq \\ 
8115.726 & $g$ & >18.52 & ASAS-SN/bi \\ 
8115.912 & $g$ & >19.28 & ASAS-SN/bq \\ 
8116.715 & $g$ & >18.12 & ASAS-SN/bi \\ 
8117.476 & $g$ & >17.93 & ASAS-SN/bm \\ 
8117.711 & $g$ & >17.89 & ASAS-SN/bi \\ 
8118.710 & $g$ & >17.19 & ASAS-SN/bi \\ 
8124.768 & $g$ & >18.16 & ASAS-SN/bi \\ 
8124.792 & $g$ & >18.37 & ASAS-SN/bq \\ 
8125.742 & $g$ & >18.27 & ASAS-SN/bi \\ 
8126.780 & $g$ & >17.98 & ASAS-SN/bi \\ 
8127.541 & $g$ & >18.31 & ASAS-SN/bm \\ 
8127.754 & $g$ & >18.62 & ASAS-SN/bi \\ 
8127.808 & $g$ & >19.06 & ASAS-SN/bq \\ 
8128.719 & $g$ & >18.90 & ASAS-SN/bi \\ 
8128.804 & $g$ & >19.14 & ASAS-SN/bq \\ 
8129.498 & $g$ & >18.66 & ASAS-SN/bm \\ 
8129.710 & $g$ & >19.08 & ASAS-SN/bi \\ 
8130.797 & $g$ & >18.89 & ASAS-SN/bq \\ 
8132.795 & $g$ & >19.15 & ASAS-SN/bq \\ 
8133.788 & $g$ & >19.24 & ASAS-SN/bq \\ 
8137.800 & $g$ & >19.06 & ASAS-SN/bq \\ 
8138.796 & $g$ & >18.91 & ASAS-SN/bq \\ 
8141.777 & $g$ & >18.88 & ASAS-SN/bq \\ 
8143.635 & $g$ & >18.46 & ASAS-SN/bi \\ 
8144.635 & $g$ & >18.23 & ASAS-SN/bi \\ 
8145.631 & $g$ & 18.740(0.710) & ASAS-SN/bi \\ 
8146.627 & $g$ & 17.010(0.220) & ASAS-SN/bi \\ 
8147.410 & $g$ & 17.330(0.270) & ASAS-SN/bm \\ 
8147.648 & $g$ & 16.910(0.200) & ASAS-SN/bq \\ 
8147.663 & $g$ & 16.730(0.180) & ASAS-SN/bi \\ 
8152.556 & $g$ & 15.500(0.070) & ASAS-SN/bm \\ 
8153.438 & $g$ & 15.130(0.040) & ASAS-SN/bm \\ 
8153.688 & $g$ & 15.140(0.040) & ASAS-SN/bi \\ 
8154.400 & $g$ & 14.930(0.030) & ASAS-SN/bm \\ 
8154.786 & $g$ & 14.890(0.030) & ASAS-SN/bq \\ 
8155.436 & $g$ & 14.760(0.030) & ASAS-SN/bm \\ 
8155.737 & $g$ & 14.720(0.020) & ASAS-SN/bq \\ 
8156.432 & $g$ & 14.630(0.020) & ASAS-SN/bm \\ 
8157.432 & $g$ & 14.490(0.020) & ASAS-SN/bm \\ 
8157.686 & $g$ & 14.570(0.020) & ASAS-SN/bi \\ 
8158.429 & $g$ & 14.450(0.020) & ASAS-SN/bm \\ 
8158.683 & $g$ & 14.460(0.020) & ASAS-SN/bi \\ 
8158.724 & $g$ & 14.440(0.020) & ASAS-SN/bq \\ 
8159.680 & $g$ & 14.380(0.020) & ASAS-SN/bi \\ 
8159.717 & $g$ & 14.420(0.020) & ASAS-SN/bq \\ 
8160.678 & $g$ & 14.320(0.020) & ASAS-SN/bi \\ 
8160.711 & $g$ & 14.420(0.020) & ASAS-SN/bq \\ 
8161.675 & $g$ & 14.260(0.020) & ASAS-SN/bi \\ 
8161.767 & $g$ & 14.270(0.020) & ASAS-SN/bq \\ 
8162.672 & $g$ & 14.280(0.020) & ASAS-SN/bi \\ 
8162.697 & $g$ & 14.260(0.020) & ASAS-SN/bq \\ 
8163.669 & $g$ & 14.250(0.020) & ASAS-SN/bi \\ 
8164.413 & $g$ & 14.320(0.020) & ASAS-SN/bm \\ 
8164.667 & $g$ & 14.270(0.020) & ASAS-SN/bi \\ 
8165.410 & $g$ & 14.300(0.020) & ASAS-SN/bm \\ 
8165.664 & $g$ & 14.310(0.020) & ASAS-SN/bi \\ 
8166.408 & $g$ & 14.290(0.020) & ASAS-SN/bm \\ 
8167.405 & $g$ & 14.430(0.020) & ASAS-SN/bm \\ 
8170.695 & $g$ & 14.490(0.020) & ASAS-SN/bq \\ 
8171.649 & $g$ & 14.540(0.020) & ASAS-SN/bi \\ 
8171.751 & $g$ & 14.540(0.020) & ASAS-SN/bq \\ 
8172.715 & $g$ & 14.610(0.020) & ASAS-SN/bi \\ 
8174.316 & $g$ & 14.860(0.030) & ASAS-SN/bm \\ 
8175.592 & $g$ & 14.860(0.030) & ASAS-SN/bq \\ 
7908.470 & $V$ & >17.57 & ASAS-SN/be \\ 
7914.454 & $V$ & >17.08 & ASAS-SN/be \\ 
8016.139 & $V$ & >17.14 & ASAS-SN/ba \\ 
8018.134 & $V$ & >17.79 & ASAS-SN/ba \\ 
8019.129 & $V$ & >17.93 & ASAS-SN/ba \\ 
8033.112 & $V$ & >17.39 & ASAS-SN/ba \\ 
8044.118 & $V$ & >18.55 & ASAS-SN/ba \\ 
8086.959 & $V$ & >17.59 & ASAS-SN/ba \\ 
8092.040 & $V$ & >17.31 & ASAS-SN/ba \\ 
8100.128 & $V$ & >17.89 & ASAS-SN/ba \\ 
8101.061 & $V$ & >18.61 & ASAS-SN/ba \\ 
8102.061 & $V$ & >18.58 & ASAS-SN/ba \\ 
8113.973 & $V$ & >18.68 & ASAS-SN/ba \\ 
8118.078 & $V$ & >17.88 & ASAS-SN/ba \\ 
8125.002 & $V$ & >17.47 & ASAS-SN/ba \\ 
8126.112 & $V$ & >17.93 & ASAS-SN/ba \\ 
8127.108 & $V$ & >18.25 & ASAS-SN/ba \\ 
8128.109 & $V$ & >18.30 & ASAS-SN/ba \\ 
8129.105 & $V$ & >18.42 & ASAS-SN/ba \\ 
8130.102 & $V$ & >18.31 & ASAS-SN/ba \\ 
8131.036 & $V$ & >18.61 & ASAS-SN/ba \\ 
8132.035 & $V$ & >18.57 & ASAS-SN/ba \\ 
8132.868 & $V$ & >18.63 & ASAS-SN/ba \\ 
8133.865 & $V$ & >18.54 & ASAS-SN/ba \\ 
8134.859 & $V$ & >18.26 & ASAS-SN/ba \\ 
8135.862 & $V$ & >18.67 & ASAS-SN/ba \\ 
8136.858 & $V$ & >18.18 & ASAS-SN/ba \\ 
8137.860 & $V$ & >18.72 & ASAS-SN/ba \\ 
8138.852 & $V$ & >18.75 & ASAS-SN/ba \\ 
8140.852 & $V$ & >18.45 & ASAS-SN/ba \\ 
8141.845 & $V$ & >18.38 & ASAS-SN/ba \\ 
8145.809 & $V$ & >17.58 & ASAS-SN/ba \\ 
8153.998 & $V$ & 15.157(0.040) & ASAS-SN/ba \\ 
8157.686 & $V$ & 14.717(0.034) & ASAS-SN/be \\ 
8158.683 & $V$ & 14.519(0.030) & ASAS-SN/be \\ 
8159.681 & $V$ & 14.440(0.028) & ASAS-SN/be \\ 
8160.678 & $V$ & 14.362(0.029) & ASAS-SN/be \\ 
8161.675 & $V$ & 14.341(0.028) & ASAS-SN/be \\ 
8161.912 & $V$ & 14.375(0.020) & ASAS-SN/ba \\ 
8162.672 & $V$ & 14.398(0.027) & ASAS-SN/be \\ 
8163.670 & $V$ & 14.319(0.026) & ASAS-SN/be \\ 
8164.667 & $V$ & 14.350(0.027) & ASAS-SN/be \\ 
8165.664 & $V$ & 14.361(0.026) & ASAS-SN/be \\ 
8166.662 & $V$ & 14.304(0.036) & ASAS-SN/be \\ 
8173.583 & $V$ & 14.681(0.038) & ASAS-SN/be \\ 
8174.742 & $V$ & 14.769(0.034) & ASAS-SN/be \\ 
8095.490 & $K2$ & >21.12 & K2 \\ 
8095.510 & $K2$ & >21.12 & K2 \\ 
8095.551 & $K2$ & >21.12 & K2 \\ 
8095.572 & $K2$ & >21.12 & K2 \\ 
8095.592 & $K2$ & >21.12 & K2 \\ 
8095.612 & $K2$ & >21.12 & K2 \\ 
8095.633 & $K2$ & >21.12 & K2 \\ 
8095.653 & $K2$ & >21.12 & K2 \\ 
8095.674 & $K2$ & >21.12 & K2 \\ 
8095.694 & $K2$ & >21.12 & K2 \\ 
8095.715 & $K2$ & >21.12 & K2 \\ 
8095.776 & $K2$ & >21.12 & K2 \\ 
8095.796 & $K2$ & >21.12 & K2 \\ 
8095.817 & $K2$ & >21.12 & K2 \\ 
8095.837 & $K2$ & >21.12 & K2 \\ 
8095.858 & $K2$ & >21.12 & K2 \\ 
8095.878 & $K2$ & >21.12 & K2 \\ 
8095.919 & $K2$ & >21.12 & K2 \\ 
8095.939 & $K2$ & >21.12 & K2 \\ 
8095.960 & $K2$ & >21.12 & K2 \\ 
8095.980 & $K2$ & >21.12 & K2 \\ 
8096.001 & $K2$ & >21.12 & K2 \\ 
8096.021 & $K2$ & >21.12 & K2 \\ 
8096.042 & $K2$ & >21.12 & K2 \\ 
8096.062 & $K2$ & >21.12 & K2 \\ 
8096.082 & $K2$ & >21.12 & K2 \\ 
8096.103 & $K2$ & >21.12 & K2 \\ 
8096.123 & $K2$ & >21.12 & K2 \\ 
8096.144 & $K2$ & >21.12 & K2 \\ 
8096.164 & $K2$ & >21.12 & K2 \\ 
8096.185 & $K2$ & >21.12 & K2 \\ 
8096.205 & $K2$ & >21.12 & K2 \\ 
8096.226 & $K2$ & >21.12 & K2 \\ 
8096.287 & $K2$ & >21.12 & K2 \\ 
8096.307 & $K2$ & >21.12 & K2 \\ 
8096.328 & $K2$ & >21.12 & K2 \\ 
8096.348 & $K2$ & >21.12 & K2 \\ 
8096.369 & $K2$ & >21.12 & K2 \\ 
8096.409 & $K2$ & >21.12 & K2 \\ 
8096.430 & $K2$ & >21.12 & K2 \\ 
8096.450 & $K2$ & >21.12 & K2 \\ 
8096.471 & $K2$ & >21.12 & K2 \\ 
8096.491 & $K2$ & >21.12 & K2 \\ 
8096.512 & $K2$ & >21.12 & K2 \\ 
8096.532 & $K2$ & >21.12 & K2 \\ 
8096.552 & $K2$ & >21.12 & K2 \\ 
8096.573 & $K2$ & >21.12 & K2 \\ 
8096.593 & $K2$ & >21.12 & K2 \\ 
8096.614 & $K2$ & >21.12 & K2 \\ 
8096.634 & $K2$ & >21.12 & K2 \\ 
8096.655 & $K2$ & >21.12 & K2 \\ 
8096.675 & $K2$ & >21.12 & K2 \\ 
8096.695 & $K2$ & >21.12 & K2 \\ 
8096.716 & $K2$ & >21.12 & K2 \\ 
8096.736 & $K2$ & >21.12 & K2 \\ 
8096.757 & $K2$ & >21.12 & K2 \\ 
8096.777 & $K2$ & >21.12 & K2 \\ 
8096.798 & $K2$ & >21.12 & K2 \\ 
8096.818 & $K2$ & >21.12 & K2 \\ 
8096.839 & $K2$ & >21.12 & K2 \\ 
8096.859 & $K2$ & >21.12 & K2 \\ 
8096.900 & $K2$ & >21.12 & K2 \\ 
8096.920 & $K2$ & >21.12 & K2 \\ 
8096.941 & $K2$ & >21.12 & K2 \\ 
8096.961 & $K2$ & >21.12 & K2 \\ 
8096.982 & $K2$ & >21.12 & K2 \\ 
8097.022 & $K2$ & >21.12 & K2 \\ 
8097.043 & $K2$ & >21.12 & K2 \\ 
8097.063 & $K2$ & >21.12 & K2 \\ 
8097.084 & $K2$ & >21.12 & K2 \\ 
8097.104 & $K2$ & >21.12 & K2 \\ 
8097.145 & $K2$ & >21.12 & K2 \\ 
8097.165 & $K2$ & >21.12 & K2 \\ 
8097.186 & $K2$ & >21.12 & K2 \\ 
8097.206 & $K2$ & >21.12 & K2 \\ 
8097.227 & $K2$ & >21.12 & K2 \\ 
8097.247 & $K2$ & >21.12 & K2 \\ 
8097.268 & $K2$ & >21.12 & K2 \\ 
8097.288 & $K2$ & >21.12 & K2 \\ 
8097.308 & $K2$ & >21.12 & K2 \\ 
8097.329 & $K2$ & >21.12 & K2 \\ 
8097.349 & $K2$ & >21.12 & K2 \\ 
8097.390 & $K2$ & >21.12 & K2 \\ 
8097.411 & $K2$ & >21.12 & K2 \\ 
8097.431 & $K2$ & >21.12 & K2 \\ 
8097.452 & $K2$ & >21.12 & K2 \\ 
8097.554 & $K2$ & >21.12 & K2 \\ 
8097.574 & $K2$ & >21.12 & K2 \\ 
8097.595 & $K2$ & >21.12 & K2 \\ 
8097.615 & $K2$ & >21.12 & K2 \\ 
8097.635 & $K2$ & >21.12 & K2 \\ 
8097.656 & $K2$ & >21.12 & K2 \\ 
8097.676 & $K2$ & >21.12 & K2 \\ 
8097.697 & $K2$ & >21.12 & K2 \\ 
8097.717 & $K2$ & >21.12 & K2 \\ 
8097.738 & $K2$ & >21.12 & K2 \\ 
8097.758 & $K2$ & >21.12 & K2 \\ 
8097.778 & $K2$ & >21.12 & K2 \\ 
8097.799 & $K2$ & >21.12 & K2 \\ 
8097.819 & $K2$ & >21.12 & K2 \\ 
8097.840 & $K2$ & >21.12 & K2 \\ 
8097.881 & $K2$ & >21.12 & K2 \\ 
8097.901 & $K2$ & >21.12 & K2 \\ 
8097.921 & $K2$ & >21.12 & K2 \\ 
8097.942 & $K2$ & >21.12 & K2 \\ 
8097.962 & $K2$ & >21.12 & K2 \\ 
8097.983 & $K2$ & >21.12 & K2 \\ 
8098.003 & $K2$ & >21.12 & K2 \\ 
8098.024 & $K2$ & >21.12 & K2 \\ 
8098.044 & $K2$ & >21.12 & K2 \\ 
8098.065 & $K2$ & >21.12 & K2 \\ 
8098.085 & $K2$ & >21.12 & K2 \\ 
8098.126 & $K2$ & >21.12 & K2 \\ 
8098.146 & $K2$ & >21.12 & K2 \\ 
8098.167 & $K2$ & >21.12 & K2 \\ 
8098.187 & $K2$ & >21.12 & K2 \\ 
8098.208 & $K2$ & >21.12 & K2 \\ 
8098.228 & $K2$ & >21.12 & K2 \\ 
8098.248 & $K2$ & >21.12 & K2 \\ 
8098.269 & $K2$ & >21.12 & K2 \\ 
8098.289 & $K2$ & >21.12 & K2 \\ 
8098.310 & $K2$ & >21.12 & K2 \\ 
8098.330 & $K2$ & >21.12 & K2 \\ 
8098.371 & $K2$ & >21.12 & K2 \\ 
8098.453 & $K2$ & >21.12 & K2 \\ 
8098.473 & $K2$ & >21.12 & K2 \\ 
8098.494 & $K2$ & >21.12 & K2 \\ 
8098.514 & $K2$ & >21.12 & K2 \\ 
8098.535 & $K2$ & >21.12 & K2 \\ 
8098.555 & $K2$ & >21.12 & K2 \\ 
8098.575 & $K2$ & >21.12 & K2 \\ 
8098.616 & $K2$ & >21.12 & K2 \\ 
8098.637 & $K2$ & >21.12 & K2 \\ 
8098.657 & $K2$ & >21.12 & K2 \\ 
8098.678 & $K2$ & >21.12 & K2 \\ 
8098.698 & $K2$ & >21.12 & K2 \\ 
8098.718 & $K2$ & >21.12 & K2 \\ 
8098.759 & $K2$ & >21.12 & K2 \\ 
8098.780 & $K2$ & >21.12 & K2 \\ 
8098.800 & $K2$ & >21.12 & K2 \\ 
8098.821 & $K2$ & >21.12 & K2 \\ 
8098.861 & $K2$ & >21.12 & K2 \\ 
8098.882 & $K2$ & >21.12 & K2 \\ 
8098.902 & $K2$ & >21.12 & K2 \\ 
8098.923 & $K2$ & >21.12 & K2 \\ 
8098.943 & $K2$ & >21.12 & K2 \\ 
8098.964 & $K2$ & >21.12 & K2 \\ 
8098.984 & $K2$ & >21.12 & K2 \\ 
8099.004 & $K2$ & >21.12 & K2 \\ 
8099.025 & $K2$ & >21.12 & K2 \\ 
8099.045 & $K2$ & >21.12 & K2 \\ 
8099.066 & $K2$ & >21.12 & K2 \\ 
8099.086 & $K2$ & >21.12 & K2 \\ 
8099.107 & $K2$ & >21.12 & K2 \\ 
8099.127 & $K2$ & >21.12 & K2 \\ 
8099.148 & $K2$ & >21.12 & K2 \\ 
8099.168 & $K2$ & >21.12 & K2 \\ 
8099.188 & $K2$ & >21.12 & K2 \\ 
8099.209 & $K2$ & >21.12 & K2 \\ 
8099.229 & $K2$ & >21.12 & K2 \\ 
8099.250 & $K2$ & >21.12 & K2 \\ 
8099.270 & $K2$ & >21.12 & K2 \\ 
8099.291 & $K2$ & >21.12 & K2 \\ 
8099.311 & $K2$ & >21.12 & K2 \\ 
8099.372 & $K2$ & >21.12 & K2 \\ 
8099.393 & $K2$ & >21.12 & K2 \\ 
8099.413 & $K2$ & >21.12 & K2 \\ 
8099.434 & $K2$ & >21.12 & K2 \\ 
8099.454 & $K2$ & >21.12 & K2 \\ 
8099.474 & $K2$ & >21.12 & K2 \\ 
8099.495 & $K2$ & >21.12 & K2 \\ 
8099.515 & $K2$ & >21.12 & K2 \\ 
8099.536 & $K2$ & >21.12 & K2 \\ 
8099.556 & $K2$ & >21.12 & K2 \\ 
8099.597 & $K2$ & >21.12 & K2 \\ 
8099.617 & $K2$ & >21.12 & K2 \\ 
8099.638 & $K2$ & >21.12 & K2 \\ 
8099.658 & $K2$ & >21.12 & K2 \\ 
8099.679 & $K2$ & >21.12 & K2 \\ 
8099.699 & $K2$ & >21.12 & K2 \\ 
8099.720 & $K2$ & >21.12 & K2 \\ 
8099.740 & $K2$ & >21.12 & K2 \\ 
8099.761 & $K2$ & >21.12 & K2 \\ 
8099.781 & $K2$ & >21.12 & K2 \\ 
8099.801 & $K2$ & >21.12 & K2 \\ 
8099.822 & $K2$ & >21.12 & K2 \\ 
8099.842 & $K2$ & >21.12 & K2 \\ 
8099.863 & $K2$ & >21.12 & K2 \\ 
8099.883 & $K2$ & >21.12 & K2 \\ 
8099.904 & $K2$ & >21.12 & K2 \\ 
8099.944 & $K2$ & >21.12 & K2 \\ 
8099.965 & $K2$ & >21.12 & K2 \\ 
8099.985 & $K2$ & >21.12 & K2 \\ 
8100.006 & $K2$ & >21.12 & K2 \\ 
8100.026 & $K2$ & >21.12 & K2 \\ 
8100.047 & $K2$ & >21.12 & K2 \\ 
8100.087 & $K2$ & >21.12 & K2 \\ 
8100.108 & $K2$ & >21.12 & K2 \\ 
8100.128 & $K2$ & >21.12 & K2 \\ 
8100.149 & $K2$ & >21.12 & K2 \\ 
8100.169 & $K2$ & >21.12 & K2 \\ 
8100.190 & $K2$ & >21.12 & K2 \\ 
8100.210 & $K2$ & >21.12 & K2 \\ 
8100.230 & $K2$ & >21.12 & K2 \\ 
8100.251 & $K2$ & >21.12 & K2 \\ 
8100.271 & $K2$ & >21.12 & K2 \\ 
8100.292 & $K2$ & >21.12 & K2 \\ 
8100.333 & $K2$ & >21.12 & K2 \\ 
8100.353 & $K2$ & >21.12 & K2 \\ 
8100.374 & $K2$ & >21.12 & K2 \\ 
8100.394 & $K2$ & >21.12 & K2 \\ 
8100.414 & $K2$ & >21.12 & K2 \\ 
8100.435 & $K2$ & >21.12 & K2 \\ 
8100.455 & $K2$ & >21.12 & K2 \\ 
8100.476 & $K2$ & >21.12 & K2 \\ 
8100.496 & $K2$ & >21.12 & K2 \\ 
8100.517 & $K2$ & >21.12 & K2 \\ 
8100.537 & $K2$ & >21.12 & K2 \\ 
8100.557 & $K2$ & >21.12 & K2 \\ 
8100.578 & $K2$ & >21.12 & K2 \\ 
8100.598 & $K2$ & >21.12 & K2 \\ 
8100.619 & $K2$ & >21.12 & K2 \\ 
8100.639 & $K2$ & >21.12 & K2 \\ 
8100.660 & $K2$ & >21.12 & K2 \\ 
8100.680 & $K2$ & >21.12 & K2 \\ 
8100.700 & $K2$ & >21.12 & K2 \\ 
8100.721 & $K2$ & >21.12 & K2 \\ 
8100.741 & $K2$ & >21.12 & K2 \\ 
8100.762 & $K2$ & >21.12 & K2 \\ 
8100.782 & $K2$ & >21.12 & K2 \\ 
8100.823 & $K2$ & >21.12 & K2 \\ 
8100.843 & $K2$ & >21.12 & K2 \\ 
8100.864 & $K2$ & >21.12 & K2 \\ 
8100.884 & $K2$ & >21.12 & K2 \\ 
8100.905 & $K2$ & >21.12 & K2 \\ 
8100.925 & $K2$ & >21.12 & K2 \\ 
8100.946 & $K2$ & >21.12 & K2 \\ 
8100.966 & $K2$ & >21.12 & K2 \\ 
8100.987 & $K2$ & >21.12 & K2 \\ 
8101.007 & $K2$ & >21.12 & K2 \\ 
8101.027 & $K2$ & >21.12 & K2 \\ 
8101.068 & $K2$ & >21.12 & K2 \\ 
8101.089 & $K2$ & >21.12 & K2 \\ 
8101.109 & $K2$ & >21.12 & K2 \\ 
8101.150 & $K2$ & >21.12 & K2 \\ 
8101.170 & $K2$ & >21.12 & K2 \\ 
8101.191 & $K2$ & >21.12 & K2 \\ 
8101.211 & $K2$ & >21.12 & K2 \\ 
8101.232 & $K2$ & >21.12 & K2 \\ 
8101.252 & $K2$ & >21.12 & K2 \\ 
8101.273 & $K2$ & >21.12 & K2 \\ 
8101.313 & $K2$ & >21.12 & K2 \\ 
8101.334 & $K2$ & >21.12 & K2 \\ 
8101.354 & $K2$ & >21.12 & K2 \\ 
8101.375 & $K2$ & >21.12 & K2 \\ 
8101.395 & $K2$ & >21.12 & K2 \\ 
8101.416 & $K2$ & >21.12 & K2 \\ 
8101.436 & $K2$ & >21.12 & K2 \\ 
8101.457 & $K2$ & >21.12 & K2 \\ 
8101.477 & $K2$ & >21.12 & K2 \\ 
8101.518 & $K2$ & >21.12 & K2 \\ 
8101.559 & $K2$ & >21.12 & K2 \\ 
8101.579 & $K2$ & >21.12 & K2 \\ 
8101.600 & $K2$ & >21.12 & K2 \\ 
8101.620 & $K2$ & >21.12 & K2 \\ 
8101.640 & $K2$ & >21.12 & K2 \\ 
8101.661 & $K2$ & >21.12 & K2 \\ 
8101.681 & $K2$ & >21.12 & K2 \\ 
8101.702 & $K2$ & >21.12 & K2 \\ 
8101.722 & $K2$ & >21.12 & K2 \\ 
8101.743 & $K2$ & >21.12 & K2 \\ 
8101.763 & $K2$ & >21.12 & K2 \\ 
8101.804 & $K2$ & >21.12 & K2 \\ 
8101.824 & $K2$ & >21.12 & K2 \\ 
8101.845 & $K2$ & >21.12 & K2 \\ 
8101.865 & $K2$ & >21.12 & K2 \\ 
8101.886 & $K2$ & >21.12 & K2 \\ 
8101.906 & $K2$ & >21.12 & K2 \\ 
8101.926 & $K2$ & >21.12 & K2 \\ 
8101.947 & $K2$ & >21.12 & K2 \\ 
8101.967 & $K2$ & >21.12 & K2 \\ 
8101.988 & $K2$ & >21.12 & K2 \\ 
8102.008 & $K2$ & >21.12 & K2 \\ 
8102.029 & $K2$ & >21.12 & K2 \\ 
8102.049 & $K2$ & >21.12 & K2 \\ 
8102.070 & $K2$ & >21.12 & K2 \\ 
8102.090 & $K2$ & >21.12 & K2 \\ 
8102.110 & $K2$ & >21.12 & K2 \\ 
8102.131 & $K2$ & >21.12 & K2 \\ 
8102.151 & $K2$ & >21.12 & K2 \\ 
8102.172 & $K2$ & >21.12 & K2 \\ 
8102.192 & $K2$ & >21.12 & K2 \\ 
8102.213 & $K2$ & >21.12 & K2 \\ 
8102.233 & $K2$ & >21.12 & K2 \\ 
8102.253 & $K2$ & >21.12 & K2 \\ 
8102.294 & $K2$ & >21.12 & K2 \\ 
8102.315 & $K2$ & >21.12 & K2 \\ 
8102.335 & $K2$ & >21.12 & K2 \\ 
8102.356 & $K2$ & >21.12 & K2 \\ 
8102.376 & $K2$ & >21.12 & K2 \\ 
8102.417 & $K2$ & >21.12 & K2 \\ 
8102.437 & $K2$ & >21.12 & K2 \\ 
8102.458 & $K2$ & >21.12 & K2 \\ 
8102.478 & $K2$ & >21.12 & K2 \\ 
8102.499 & $K2$ & >21.12 & K2 \\ 
8102.519 & $K2$ & >21.12 & K2 \\ 
8102.539 & $K2$ & >21.12 & K2 \\ 
8102.560 & $K2$ & >21.12 & K2 \\ 
8102.580 & $K2$ & >21.12 & K2 \\ 
8102.601 & $K2$ & >21.12 & K2 \\ 
8102.621 & $K2$ & >21.12 & K2 \\ 
8102.642 & $K2$ & >21.12 & K2 \\ 
8102.662 & $K2$ & >21.12 & K2 \\ 
8102.683 & $K2$ & >21.12 & K2 \\ 
8102.703 & $K2$ & >21.12 & K2 \\ 
8102.723 & $K2$ & >21.12 & K2 \\ 
8102.744 & $K2$ & >21.12 & K2 \\ 
8102.785 & $K2$ & >21.12 & K2 \\ 
8102.805 & $K2$ & >21.12 & K2 \\ 
8102.826 & $K2$ & >21.12 & K2 \\ 
8102.846 & $K2$ & >21.12 & K2 \\ 
8102.866 & $K2$ & >21.12 & K2 \\ 
8102.887 & $K2$ & >21.12 & K2 \\ 
8102.907 & $K2$ & >21.12 & K2 \\ 
8102.928 & $K2$ & >21.12 & K2 \\ 
8102.948 & $K2$ & >21.12 & K2 \\ 
8102.969 & $K2$ & >21.12 & K2 \\ 
8102.989 & $K2$ & >21.12 & K2 \\ 
8103.030 & $K2$ & >21.12 & K2 \\ 
8103.071 & $K2$ & >21.12 & K2 \\ 
8103.091 & $K2$ & >21.12 & K2 \\ 
8103.112 & $K2$ & >21.12 & K2 \\ 
8103.132 & $K2$ & >21.12 & K2 \\ 
8103.152 & $K2$ & >21.12 & K2 \\ 
8103.173 & $K2$ & >21.12 & K2 \\ 
8103.193 & $K2$ & >21.12 & K2 \\ 
8103.214 & $K2$ & >21.12 & K2 \\ 
8103.234 & $K2$ & >21.12 & K2 \\ 
8103.296 & $K2$ & >21.12 & K2 \\ 
8103.316 & $K2$ & >21.12 & K2 \\ 
8103.336 & $K2$ & >21.12 & K2 \\ 
8103.357 & $K2$ & >21.12 & K2 \\ 
8103.377 & $K2$ & >21.12 & K2 \\ 
8103.398 & $K2$ & >21.12 & K2 \\ 
8103.418 & $K2$ & >21.12 & K2 \\ 
8103.439 & $K2$ & >21.12 & K2 \\ 
8103.459 & $K2$ & >21.12 & K2 \\ 
8103.479 & $K2$ & >21.12 & K2 \\ 
8103.500 & $K2$ & >21.12 & K2 \\ 
8103.520 & $K2$ & >21.12 & K2 \\ 
8103.541 & $K2$ & >21.12 & K2 \\ 
8103.561 & $K2$ & >21.12 & K2 \\ 
8103.582 & $K2$ & >21.12 & K2 \\ 
8103.602 & $K2$ & >21.12 & K2 \\ 
8103.622 & $K2$ & >21.12 & K2 \\ 
8103.643 & $K2$ & >21.12 & K2 \\ 
8103.663 & $K2$ & >21.12 & K2 \\ 
8103.684 & $K2$ & >21.12 & K2 \\ 
8103.704 & $K2$ & >21.12 & K2 \\ 
8103.725 & $K2$ & >21.12 & K2 \\ 
8103.766 & $K2$ & >21.12 & K2 \\ 
8103.786 & $K2$ & >21.12 & K2 \\ 
8103.806 & $K2$ & >21.12 & K2 \\ 
8103.827 & $K2$ & >21.12 & K2 \\ 
8103.847 & $K2$ & >21.12 & K2 \\ 
8103.868 & $K2$ & >21.12 & K2 \\ 
8103.888 & $K2$ & >21.12 & K2 \\ 
8103.929 & $K2$ & >21.12 & K2 \\ 
8103.949 & $K2$ & >21.12 & K2 \\ 
8103.970 & $K2$ & >21.12 & K2 \\ 
8104.011 & $K2$ & >21.12 & K2 \\ 
8104.031 & $K2$ & >21.12 & K2 \\ 
8104.052 & $K2$ & >21.12 & K2 \\ 
8104.072 & $K2$ & >21.12 & K2 \\ 
8104.092 & $K2$ & >21.12 & K2 \\ 
8104.113 & $K2$ & >21.12 & K2 \\ 
8104.133 & $K2$ & >21.12 & K2 \\ 
8104.154 & $K2$ & >21.12 & K2 \\ 
8104.174 & $K2$ & >21.12 & K2 \\ 
8104.195 & $K2$ & >21.12 & K2 \\ 
8104.215 & $K2$ & >21.12 & K2 \\ 
8104.256 & $K2$ & >21.12 & K2 \\ 
8104.276 & $K2$ & >21.12 & K2 \\ 
8104.297 & $K2$ & >21.12 & K2 \\ 
8104.317 & $K2$ & >21.12 & K2 \\ 
8104.338 & $K2$ & >21.12 & K2 \\ 
8104.358 & $K2$ & >21.12 & K2 \\ 
8104.379 & $K2$ & >21.12 & K2 \\ 
8104.399 & $K2$ & >21.12 & K2 \\ 
8104.419 & $K2$ & >21.12 & K2 \\ 
8104.440 & $K2$ & >21.12 & K2 \\ 
8104.460 & $K2$ & >21.12 & K2 \\ 
8104.481 & $K2$ & >21.12 & K2 \\ 
8104.501 & $K2$ & >21.12 & K2 \\ 
8104.522 & $K2$ & >21.12 & K2 \\ 
8104.542 & $K2$ & >21.12 & K2 \\ 
8104.562 & $K2$ & >21.12 & K2 \\ 
8104.583 & $K2$ & >21.12 & K2 \\ 
8104.603 & $K2$ & >21.12 & K2 \\ 
8104.624 & $K2$ & >21.12 & K2 \\ 
8104.644 & $K2$ & >21.12 & K2 \\ 
8104.665 & $K2$ & >21.12 & K2 \\ 
8104.685 & $K2$ & >21.12 & K2 \\ 
8104.705 & $K2$ & >21.12 & K2 \\ 
8104.746 & $K2$ & >21.12 & K2 \\ 
8104.767 & $K2$ & >21.12 & K2 \\ 
8104.787 & $K2$ & >21.12 & K2 \\ 
8104.808 & $K2$ & >21.12 & K2 \\ 
8104.828 & $K2$ & >21.12 & K2 \\ 
8104.848 & $K2$ & >21.12 & K2 \\ 
8104.869 & $K2$ & >21.12 & K2 \\ 
8104.889 & $K2$ & >21.12 & K2 \\ 
8104.910 & $K2$ & >21.12 & K2 \\ 
8104.930 & $K2$ & >21.12 & K2 \\ 
8104.951 & $K2$ & >21.12 & K2 \\ 
8104.992 & $K2$ & >21.12 & K2 \\ 
8105.012 & $K2$ & >21.12 & K2 \\ 
8105.032 & $K2$ & >21.12 & K2 \\ 
8105.053 & $K2$ & >21.12 & K2 \\ 
8105.073 & $K2$ & >21.12 & K2 \\ 
8105.094 & $K2$ & >21.12 & K2 \\ 
8105.114 & $K2$ & >21.12 & K2 \\ 
8105.135 & $K2$ & >21.12 & K2 \\ 
8105.155 & $K2$ & >21.12 & K2 \\ 
8105.175 & $K2$ & >21.12 & K2 \\ 
8105.196 & $K2$ & >21.12 & K2 \\ 
8105.237 & $K2$ & >21.12 & K2 \\ 
8105.257 & $K2$ & >21.12 & K2 \\ 
8105.278 & $K2$ & >21.12 & K2 \\ 
8105.298 & $K2$ & >21.12 & K2 \\ 
8105.318 & $K2$ & >21.12 & K2 \\ 
8105.339 & $K2$ & >21.12 & K2 \\ 
8105.359 & $K2$ & >21.12 & K2 \\ 
8105.380 & $K2$ & >21.12 & K2 \\ 
8105.400 & $K2$ & >21.12 & K2 \\ 
8105.421 & $K2$ & >21.12 & K2 \\ 
8105.441 & $K2$ & >21.12 & K2 \\ 
8105.461 & $K2$ & >21.12 & K2 \\ 
8105.482 & $K2$ & >21.12 & K2 \\ 
8105.502 & $K2$ & >21.12 & K2 \\ 
8105.523 & $K2$ & >21.12 & K2 \\ 
8105.543 & $K2$ & >21.12 & K2 \\ 
8105.564 & $K2$ & >21.12 & K2 \\ 
8105.584 & $K2$ & >21.12 & K2 \\ 
8105.605 & $K2$ & >21.12 & K2 \\ 
8105.625 & $K2$ & >21.12 & K2 \\ 
8105.645 & $K2$ & >21.12 & K2 \\ 
8105.666 & $K2$ & >21.12 & K2 \\ 
8105.686 & $K2$ & >21.12 & K2 \\ 
8105.727 & $K2$ & >21.12 & K2 \\ 
8105.748 & $K2$ & >21.12 & K2 \\ 
8105.768 & $K2$ & >21.12 & K2 \\ 
8105.788 & $K2$ & >21.12 & K2 \\ 
8105.809 & $K2$ & >21.12 & K2 \\ 
8105.829 & $K2$ & >21.12 & K2 \\ 
8105.850 & $K2$ & >21.12 & K2 \\ 
8105.870 & $K2$ & >21.12 & K2 \\ 
8105.891 & $K2$ & >21.12 & K2 \\ 
8105.911 & $K2$ & >21.12 & K2 \\ 
8105.931 & $K2$ & >21.12 & K2 \\ 
8105.952 & $K2$ & >21.12 & K2 \\ 
8105.972 & $K2$ & >21.12 & K2 \\ 
8105.993 & $K2$ & >21.12 & K2 \\ 
8106.013 & $K2$ & >21.12 & K2 \\ 
8106.034 & $K2$ & >21.12 & K2 \\ 
8106.054 & $K2$ & >21.12 & K2 \\ 
8106.075 & $K2$ & >21.12 & K2 \\ 
8106.095 & $K2$ & >21.12 & K2 \\ 
8106.115 & $K2$ & >21.12 & K2 \\ 
8106.136 & $K2$ & >21.12 & K2 \\ 
8106.156 & $K2$ & >21.12 & K2 \\ 
8106.177 & $K2$ & >21.12 & K2 \\ 
8106.218 & $K2$ & >21.12 & K2 \\ 
8106.238 & $K2$ & >21.12 & K2 \\ 
8106.258 & $K2$ & >21.12 & K2 \\ 
8106.279 & $K2$ & >21.12 & K2 \\ 
8106.299 & $K2$ & >21.12 & K2 \\ 
8106.320 & $K2$ & >21.12 & K2 \\ 
8106.340 & $K2$ & >21.12 & K2 \\ 
8106.361 & $K2$ & >21.12 & K2 \\ 
8106.381 & $K2$ & >21.12 & K2 \\ 
8106.401 & $K2$ & >21.12 & K2 \\ 
8106.422 & $K2$ & >21.12 & K2 \\ 
8106.463 & $K2$ & >21.12 & K2 \\ 
8106.483 & $K2$ & >21.12 & K2 \\ 
8106.504 & $K2$ & >21.12 & K2 \\ 
8106.524 & $K2$ & >21.12 & K2 \\ 
8106.544 & $K2$ & >21.12 & K2 \\ 
8106.565 & $K2$ & >21.12 & K2 \\ 
8106.585 & $K2$ & >21.12 & K2 \\ 
8106.606 & $K2$ & >21.12 & K2 \\ 
8106.626 & $K2$ & >21.12 & K2 \\ 
8106.647 & $K2$ & >21.12 & K2 \\ 
8106.667 & $K2$ & >21.12 & K2 \\ 
8106.708 & $K2$ & >21.12 & K2 \\ 
8106.728 & $K2$ & >21.12 & K2 \\ 
8106.749 & $K2$ & >21.12 & K2 \\ 
8106.769 & $K2$ & >21.12 & K2 \\ 
8106.790 & $K2$ & >21.12 & K2 \\ 
8106.810 & $K2$ & >21.12 & K2 \\ 
8106.831 & $K2$ & >21.12 & K2 \\ 
8106.851 & $K2$ & >21.12 & K2 \\ 
8106.871 & $K2$ & >21.12 & K2 \\ 
8106.892 & $K2$ & >21.12 & K2 \\ 
8106.912 & $K2$ & >21.12 & K2 \\ 
8106.953 & $K2$ & >21.12 & K2 \\ 
8106.974 & $K2$ & >21.12 & K2 \\ 
8106.994 & $K2$ & >21.12 & K2 \\ 
8107.014 & $K2$ & >21.12 & K2 \\ 
8107.035 & $K2$ & >21.12 & K2 \\ 
8107.055 & $K2$ & >21.12 & K2 \\ 
8107.076 & $K2$ & >21.12 & K2 \\ 
8107.096 & $K2$ & >21.12 & K2 \\ 
8107.117 & $K2$ & >21.12 & K2 \\ 
8107.137 & $K2$ & >21.12 & K2 \\ 
8107.157 & $K2$ & >21.12 & K2 \\ 
8107.219 & $K2$ & >21.12 & K2 \\ 
8107.239 & $K2$ & >21.12 & K2 \\ 
8107.260 & $K2$ & >21.12 & K2 \\ 
8107.280 & $K2$ & >21.12 & K2 \\ 
8107.301 & $K2$ & >21.12 & K2 \\ 
8107.341 & $K2$ & >21.12 & K2 \\ 
8107.362 & $K2$ & >21.12 & K2 \\ 
8107.382 & $K2$ & >21.12 & K2 \\ 
8107.403 & $K2$ & >21.12 & K2 \\ 
8107.444 & $K2$ & >21.12 & K2 \\ 
8107.464 & $K2$ & >21.12 & K2 \\ 
8107.484 & $K2$ & >21.12 & K2 \\ 
8107.505 & $K2$ & >21.12 & K2 \\ 
8107.525 & $K2$ & >21.12 & K2 \\ 
8107.546 & $K2$ & >21.12 & K2 \\ 
8107.566 & $K2$ & >21.12 & K2 \\ 
8107.587 & $K2$ & >21.12 & K2 \\ 
8107.607 & $K2$ & >21.12 & K2 \\ 
8107.627 & $K2$ & >21.12 & K2 \\ 
8107.648 & $K2$ & >21.12 & K2 \\ 
8107.668 & $K2$ & >21.12 & K2 \\ 
8107.689 & $K2$ & >21.12 & K2 \\ 
8107.709 & $K2$ & >21.12 & K2 \\ 
8107.730 & $K2$ & >21.12 & K2 \\ 
8107.750 & $K2$ & >21.12 & K2 \\ 
8107.770 & $K2$ & >21.12 & K2 \\ 
8107.791 & $K2$ & >21.12 & K2 \\ 
8107.811 & $K2$ & >21.12 & K2 \\ 
8107.832 & $K2$ & >21.12 & K2 \\ 
8107.852 & $K2$ & >21.12 & K2 \\ 
8107.873 & $K2$ & >21.12 & K2 \\ 
8107.893 & $K2$ & >21.12 & K2 \\ 
8107.934 & $K2$ & >21.12 & K2 \\ 
8107.954 & $K2$ & >21.12 & K2 \\ 
8107.975 & $K2$ & >21.12 & K2 \\ 
8107.995 & $K2$ & >21.12 & K2 \\ 
8108.016 & $K2$ & >21.12 & K2 \\ 
8108.036 & $K2$ & >21.12 & K2 \\ 
8108.057 & $K2$ & >21.12 & K2 \\ 
8108.077 & $K2$ & >21.12 & K2 \\ 
8108.097 & $K2$ & >21.12 & K2 \\ 
8108.118 & $K2$ & >21.12 & K2 \\ 
8108.138 & $K2$ & >21.12 & K2 \\ 
8108.179 & $K2$ & >21.12 & K2 \\ 
8108.200 & $K2$ & >21.12 & K2 \\ 
8108.240 & $K2$ & >21.12 & K2 \\ 
8108.261 & $K2$ & >21.12 & K2 \\ 
8108.281 & $K2$ & >21.12 & K2 \\ 
8108.302 & $K2$ & >21.12 & K2 \\ 
8108.322 & $K2$ & >21.12 & K2 \\ 
8108.343 & $K2$ & >21.12 & K2 \\ 
8108.363 & $K2$ & >21.12 & K2 \\ 
8108.384 & $K2$ & >21.12 & K2 \\ 
8108.404 & $K2$ & >21.12 & K2 \\ 
8108.424 & $K2$ & >21.12 & K2 \\ 
8108.445 & $K2$ & >21.12 & K2 \\ 
8108.465 & $K2$ & >21.12 & K2 \\ 
8108.486 & $K2$ & >21.12 & K2 \\ 
8108.506 & $K2$ & >21.12 & K2 \\ 
8108.527 & $K2$ & >21.12 & K2 \\ 
8108.547 & $K2$ & >21.12 & K2 \\ 
8108.567 & $K2$ & >21.12 & K2 \\ 
8108.588 & $K2$ & >21.12 & K2 \\ 
8108.608 & $K2$ & >21.12 & K2 \\ 
8108.629 & $K2$ & >21.12 & K2 \\ 
8108.670 & $K2$ & >21.12 & K2 \\ 
8108.690 & $K2$ & >21.12 & K2 \\ 
8108.710 & $K2$ & >21.12 & K2 \\ 
8108.731 & $K2$ & >21.12 & K2 \\ 
8108.751 & $K2$ & >21.12 & K2 \\ 
8108.772 & $K2$ & >21.12 & K2 \\ 
8108.792 & $K2$ & >21.12 & K2 \\ 
8108.813 & $K2$ & >21.12 & K2 \\ 
8108.833 & $K2$ & >21.12 & K2 \\ 
8108.853 & $K2$ & >21.12 & K2 \\ 
8108.874 & $K2$ & >21.12 & K2 \\ 
8108.915 & $K2$ & >21.12 & K2 \\ 
8108.935 & $K2$ & >21.12 & K2 \\ 
8108.956 & $K2$ & >21.12 & K2 \\ 
8108.976 & $K2$ & >21.12 & K2 \\ 
8108.997 & $K2$ & >21.12 & K2 \\ 
8109.017 & $K2$ & >21.12 & K2 \\ 
8109.037 & $K2$ & >21.12 & K2 \\ 
8109.058 & $K2$ & >21.12 & K2 \\ 
8109.078 & $K2$ & >21.12 & K2 \\ 
8109.099 & $K2$ & >21.12 & K2 \\ 
8109.119 & $K2$ & >21.12 & K2 \\ 
8109.160 & $K2$ & >21.12 & K2 \\ 
8109.180 & $K2$ & >21.12 & K2 \\ 
8109.201 & $K2$ & >21.12 & K2 \\ 
8109.221 & $K2$ & >21.12 & K2 \\ 
8109.242 & $K2$ & >21.12 & K2 \\ 
8109.262 & $K2$ & >21.12 & K2 \\ 
8109.283 & $K2$ & >21.12 & K2 \\ 
8109.303 & $K2$ & >21.12 & K2 \\ 
8109.323 & $K2$ & >21.12 & K2 \\ 
8109.344 & $K2$ & >21.12 & K2 \\ 
8109.364 & $K2$ & >21.12 & K2 \\ 
8109.405 & $K2$ & >21.12 & K2 \\ 
8109.426 & $K2$ & >21.12 & K2 \\ 
8109.466 & $K2$ & >21.12 & K2 \\ 
8109.487 & $K2$ & >21.12 & K2 \\ 
8109.507 & $K2$ & >21.12 & K2 \\ 
8109.528 & $K2$ & >21.12 & K2 \\ 
8109.548 & $K2$ & >21.12 & K2 \\ 
8109.569 & $K2$ & >21.12 & K2 \\ 
8109.589 & $K2$ & >21.12 & K2 \\ 
8109.610 & $K2$ & >21.12 & K2 \\ 
8109.650 & $K2$ & >21.12 & K2 \\ 
8109.671 & $K2$ & >21.12 & K2 \\ 
8109.691 & $K2$ & >21.12 & K2 \\ 
8109.712 & $K2$ & >21.12 & K2 \\ 
8109.732 & $K2$ & >21.12 & K2 \\ 
8109.753 & $K2$ & >21.12 & K2 \\ 
8109.773 & $K2$ & >21.12 & K2 \\ 
8109.793 & $K2$ & >21.12 & K2 \\ 
8109.814 & $K2$ & >21.12 & K2 \\ 
8109.834 & $K2$ & >21.12 & K2 \\ 
8109.855 & $K2$ & >21.12 & K2 \\ 
8109.875 & $K2$ & >21.12 & K2 \\ 
8109.896 & $K2$ & >21.12 & K2 \\ 
8109.916 & $K2$ & >21.12 & K2 \\ 
8109.936 & $K2$ & >21.12 & K2 \\ 
8109.957 & $K2$ & >21.12 & K2 \\ 
8109.977 & $K2$ & >21.12 & K2 \\ 
8109.998 & $K2$ & >21.12 & K2 \\ 
8110.018 & $K2$ & >21.12 & K2 \\ 
8110.039 & $K2$ & >21.12 & K2 \\ 
8110.059 & $K2$ & >21.12 & K2 \\ 
8110.079 & $K2$ & >21.12 & K2 \\ 
8110.100 & $K2$ & >21.12 & K2 \\ 
8110.141 & $K2$ & >21.12 & K2 \\ 
8110.161 & $K2$ & >21.12 & K2 \\ 
8110.182 & $K2$ & >21.12 & K2 \\ 
8110.202 & $K2$ & >21.12 & K2 \\ 
8110.223 & $K2$ & >21.12 & K2 \\ 
8110.263 & $K2$ & >21.12 & K2 \\ 
8110.284 & $K2$ & >21.12 & K2 \\ 
8110.304 & $K2$ & >21.12 & K2 \\ 
8110.325 & $K2$ & >21.12 & K2 \\ 
8110.345 & $K2$ & >21.12 & K2 \\ 
8110.386 & $K2$ & >21.12 & K2 \\ 
8110.406 & $K2$ & >21.12 & K2 \\ 
8110.427 & $K2$ & >21.12 & K2 \\ 
8110.447 & $K2$ & >21.12 & K2 \\ 
8110.468 & $K2$ & >21.12 & K2 \\ 
8110.488 & $K2$ & >21.12 & K2 \\ 
8110.509 & $K2$ & >21.12 & K2 \\ 
8110.529 & $K2$ & >21.12 & K2 \\ 
8110.549 & $K2$ & >21.12 & K2 \\ 
8110.570 & $K2$ & >21.12 & K2 \\ 
8110.590 & $K2$ & >21.12 & K2 \\ 
8110.631 & $K2$ & >21.12 & K2 \\ 
8110.652 & $K2$ & >21.12 & K2 \\ 
8110.672 & $K2$ & >21.12 & K2 \\ 
8110.692 & $K2$ & >21.12 & K2 \\ 
8110.713 & $K2$ & >21.12 & K2 \\ 
8110.733 & $K2$ & >21.12 & K2 \\ 
8110.754 & $K2$ & >21.12 & K2 \\ 
8110.774 & $K2$ & >21.12 & K2 \\ 
8110.795 & $K2$ & >21.12 & K2 \\ 
8110.815 & $K2$ & >21.12 & K2 \\ 
8110.836 & $K2$ & >21.12 & K2 \\ 
8110.876 & $K2$ & >21.12 & K2 \\ 
8110.897 & $K2$ & >21.12 & K2 \\ 
8110.917 & $K2$ & >21.12 & K2 \\ 
8110.938 & $K2$ & >21.12 & K2 \\ 
8110.958 & $K2$ & >21.12 & K2 \\ 
8110.979 & $K2$ & >21.12 & K2 \\ 
8110.999 & $K2$ & >21.12 & K2 \\ 
8111.019 & $K2$ & >21.12 & K2 \\ 
8111.040 & $K2$ & >21.12 & K2 \\ 
8111.060 & $K2$ & >21.12 & K2 \\ 
8111.081 & $K2$ & >21.12 & K2 \\ 
8111.122 & $K2$ & >21.12 & K2 \\ 
8111.162 & $K2$ & >21.12 & K2 \\ 
8111.183 & $K2$ & >21.12 & K2 \\ 
8111.203 & $K2$ & >21.12 & K2 \\ 
8111.224 & $K2$ & >21.12 & K2 \\ 
8111.244 & $K2$ & >21.12 & K2 \\ 
8111.265 & $K2$ & >21.12 & K2 \\ 
8111.285 & $K2$ & >21.12 & K2 \\ 
8111.306 & $K2$ & >21.12 & K2 \\ 
8111.326 & $K2$ & >21.12 & K2 \\ 
8111.367 & $K2$ & >21.12 & K2 \\ 
8111.387 & $K2$ & >21.12 & K2 \\ 
8111.408 & $K2$ & >21.12 & K2 \\ 
8111.428 & $K2$ & >21.12 & K2 \\ 
8111.449 & $K2$ & >21.12 & K2 \\ 
8111.469 & $K2$ & >21.12 & K2 \\ 
8111.510 & $K2$ & >21.12 & K2 \\ 
8111.530 & $K2$ & >21.12 & K2 \\ 
8111.551 & $K2$ & >21.12 & K2 \\ 
8111.571 & $K2$ & >21.12 & K2 \\ 
8111.612 & $K2$ & >21.12 & K2 \\ 
8111.632 & $K2$ & >21.12 & K2 \\ 
8111.653 & $K2$ & >21.12 & K2 \\ 
8111.673 & $K2$ & >21.12 & K2 \\ 
8111.694 & $K2$ & >21.12 & K2 \\ 
8111.714 & $K2$ & >21.12 & K2 \\ 
8111.735 & $K2$ & >21.12 & K2 \\ 
8111.755 & $K2$ & >21.12 & K2 \\ 
8111.775 & $K2$ & >21.12 & K2 \\ 
8111.796 & $K2$ & >21.12 & K2 \\ 
8111.816 & $K2$ & >21.12 & K2 \\ 
8111.837 & $K2$ & >21.12 & K2 \\ 
8111.857 & $K2$ & >21.12 & K2 \\ 
8111.878 & $K2$ & >21.12 & K2 \\ 
8111.898 & $K2$ & >21.12 & K2 \\ 
8111.919 & $K2$ & >21.12 & K2 \\ 
8111.939 & $K2$ & >21.12 & K2 \\ 
8111.959 & $K2$ & >21.12 & K2 \\ 
8111.980 & $K2$ & >21.12 & K2 \\ 
8112.000 & $K2$ & >21.12 & K2 \\ 
8112.021 & $K2$ & >21.12 & K2 \\ 
8112.041 & $K2$ & >21.12 & K2 \\ 
8112.062 & $K2$ & >21.12 & K2 \\ 
8112.102 & $K2$ & >21.12 & K2 \\ 
8112.123 & $K2$ & >21.12 & K2 \\ 
8112.143 & $K2$ & >21.12 & K2 \\ 
8112.164 & $K2$ & >21.12 & K2 \\ 
8112.184 & $K2$ & >21.12 & K2 \\ 
8112.205 & $K2$ & >21.12 & K2 \\ 
8112.225 & $K2$ & >21.12 & K2 \\ 
8112.245 & $K2$ & >21.12 & K2 \\ 
8112.266 & $K2$ & >21.12 & K2 \\ 
8112.286 & $K2$ & >21.12 & K2 \\ 
8112.307 & $K2$ & >21.12 & K2 \\ 
8112.348 & $K2$ & >21.12 & K2 \\ 
8112.368 & $K2$ & >21.12 & K2 \\ 
8112.388 & $K2$ & >21.12 & K2 \\ 
8112.409 & $K2$ & >21.12 & K2 \\ 
8112.429 & $K2$ & >21.12 & K2 \\ 
8112.450 & $K2$ & >21.12 & K2 \\ 
8112.470 & $K2$ & >21.12 & K2 \\ 
8112.491 & $K2$ & >21.12 & K2 \\ 
8112.511 & $K2$ & >21.12 & K2 \\ 
8112.532 & $K2$ & >21.12 & K2 \\ 
8112.552 & $K2$ & >21.12 & K2 \\ 
8112.593 & $K2$ & >21.12 & K2 \\ 
8112.613 & $K2$ & >21.12 & K2 \\ 
8112.634 & $K2$ & >21.12 & K2 \\ 
8112.654 & $K2$ & >21.12 & K2 \\ 
8112.675 & $K2$ & >21.12 & K2 \\ 
8112.695 & $K2$ & >21.12 & K2 \\ 
8112.715 & $K2$ & >21.12 & K2 \\ 
8112.736 & $K2$ & >21.12 & K2 \\ 
8112.756 & $K2$ & >21.12 & K2 \\ 
8112.777 & $K2$ & >21.12 & K2 \\ 
8112.797 & $K2$ & >21.12 & K2 \\ 
8112.838 & $K2$ & >21.12 & K2 \\ 
8112.858 & $K2$ & >21.12 & K2 \\ 
8112.879 & $K2$ & >21.12 & K2 \\ 
8112.899 & $K2$ & >21.12 & K2 \\ 
8112.920 & $K2$ & >21.12 & K2 \\ 
8112.940 & $K2$ & >21.12 & K2 \\ 
8112.961 & $K2$ & >21.12 & K2 \\ 
8112.981 & $K2$ & >21.12 & K2 \\ 
8113.001 & $K2$ & >21.12 & K2 \\ 
8113.022 & $K2$ & >21.12 & K2 \\ 
8113.042 & $K2$ & >21.12 & K2 \\ 
8113.083 & $K2$ & >21.12 & K2 \\ 
8113.104 & $K2$ & >21.12 & K2 \\ 
8113.124 & $K2$ & >21.12 & K2 \\ 
8113.145 & $K2$ & >21.12 & K2 \\ 
8113.165 & $K2$ & >21.12 & K2 \\ 
8113.185 & $K2$ & >21.12 & K2 \\ 
8113.206 & $K2$ & >21.12 & K2 \\ 
8113.226 & $K2$ & >21.12 & K2 \\ 
8113.247 & $K2$ & >21.12 & K2 \\ 
8113.267 & $K2$ & >21.12 & K2 \\ 
8113.288 & $K2$ & >21.12 & K2 \\ 
8113.308 & $K2$ & >21.12 & K2 \\ 
8113.328 & $K2$ & >21.12 & K2 \\ 
8113.349 & $K2$ & >21.12 & K2 \\ 
8113.369 & $K2$ & >21.12 & K2 \\ 
8113.390 & $K2$ & >21.12 & K2 \\ 
8113.410 & $K2$ & >21.12 & K2 \\ 
8113.431 & $K2$ & >21.12 & K2 \\ 
8113.451 & $K2$ & >21.12 & K2 \\ 
8113.471 & $K2$ & >21.12 & K2 \\ 
8113.492 & $K2$ & >21.12 & K2 \\ 
8113.512 & $K2$ & >21.12 & K2 \\ 
8113.533 & $K2$ & >21.12 & K2 \\ 
8113.574 & $K2$ & >21.12 & K2 \\ 
8113.594 & $K2$ & >21.12 & K2 \\ 
8113.615 & $K2$ & >21.12 & K2 \\ 
8113.635 & $K2$ & >21.12 & K2 \\ 
8113.655 & $K2$ & >21.12 & K2 \\ 
8113.676 & $K2$ & >21.12 & K2 \\ 
8113.696 & $K2$ & >21.12 & K2 \\ 
8113.717 & $K2$ & >21.12 & K2 \\ 
8113.737 & $K2$ & >21.12 & K2 \\ 
8113.758 & $K2$ & >21.12 & K2 \\ 
8113.778 & $K2$ & >21.12 & K2 \\ 
8113.819 & $K2$ & >21.12 & K2 \\ 
8113.839 & $K2$ & >21.12 & K2 \\ 
8113.860 & $K2$ & >21.12 & K2 \\ 
8113.880 & $K2$ & >21.12 & K2 \\ 
8113.901 & $K2$ & >21.12 & K2 \\ 
8113.921 & $K2$ & >21.12 & K2 \\ 
8113.941 & $K2$ & >21.12 & K2 \\ 
8113.962 & $K2$ & >21.12 & K2 \\ 
8113.982 & $K2$ & >21.12 & K2 \\ 
8114.003 & $K2$ & >21.12 & K2 \\ 
8114.023 & $K2$ & >21.12 & K2 \\ 
8114.064 & $K2$ & >21.12 & K2 \\ 
8114.084 & $K2$ & >21.12 & K2 \\ 
8114.105 & $K2$ & >21.12 & K2 \\ 
8114.125 & $K2$ & >21.12 & K2 \\ 
8114.146 & $K2$ & >21.12 & K2 \\ 
8114.166 & $K2$ & >21.12 & K2 \\ 
8114.187 & $K2$ & >21.12 & K2 \\ 
8114.207 & $K2$ & >21.12 & K2 \\ 
8114.228 & $K2$ & >21.12 & K2 \\ 
8114.248 & $K2$ & >21.12 & K2 \\ 
8114.268 & $K2$ & >21.12 & K2 \\ 
8114.309 & $K2$ & >21.12 & K2 \\ 
8114.330 & $K2$ & >21.12 & K2 \\ 
8114.350 & $K2$ & >21.12 & K2 \\ 
8114.371 & $K2$ & >21.12 & K2 \\ 
8114.391 & $K2$ & >21.12 & K2 \\ 
8114.411 & $K2$ & >21.12 & K2 \\ 
8114.432 & $K2$ & >21.12 & K2 \\ 
8114.452 & $K2$ & >21.12 & K2 \\ 
8114.473 & $K2$ & >21.12 & K2 \\ 
8114.493 & $K2$ & >21.12 & K2 \\ 
8114.514 & $K2$ & >21.12 & K2 \\ 
8114.554 & $K2$ & >21.12 & K2 \\ 
8114.575 & $K2$ & >21.12 & K2 \\ 
8114.595 & $K2$ & >21.12 & K2 \\ 
8114.616 & $K2$ & >21.12 & K2 \\ 
8114.636 & $K2$ & >21.12 & K2 \\ 
8114.657 & $K2$ & >21.12 & K2 \\ 
8114.677 & $K2$ & >21.12 & K2 \\ 
8114.820 & $K2$ & >21.12 & K2 \\ 
8114.841 & $K2$ & >21.12 & K2 \\ 
8114.861 & $K2$ & >21.12 & K2 \\ 
8114.881 & $K2$ & >21.12 & K2 \\ 
8114.902 & $K2$ & >21.12 & K2 \\ 
8114.922 & $K2$ & >21.12 & K2 \\ 
8114.943 & $K2$ & >21.12 & K2 \\ 
8114.963 & $K2$ & >21.12 & K2 \\ 
8114.984 & $K2$ & >21.12 & K2 \\ 
8115.004 & $K2$ & >21.12 & K2 \\ 
8115.045 & $K2$ & >21.12 & K2 \\ 
8115.065 & $K2$ & >21.12 & K2 \\ 
8115.086 & $K2$ & >21.12 & K2 \\ 
8115.106 & $K2$ & >21.12 & K2 \\ 
8115.127 & $K2$ & >21.12 & K2 \\ 
8115.147 & $K2$ & >21.12 & K2 \\ 
8115.167 & $K2$ & >21.12 & K2 \\ 
8115.188 & $K2$ & >21.12 & K2 \\ 
8115.208 & $K2$ & >21.12 & K2 \\ 
8115.229 & $K2$ & >21.12 & K2 \\ 
8115.249 & $K2$ & >21.12 & K2 \\ 
8115.290 & $K2$ & >21.12 & K2 \\ 
8115.310 & $K2$ & >21.12 & K2 \\ 
8115.331 & $K2$ & >21.12 & K2 \\ 
8115.351 & $K2$ & >21.12 & K2 \\ 
8115.372 & $K2$ & >21.12 & K2 \\ 
8115.392 & $K2$ & >21.12 & K2 \\ 
8115.413 & $K2$ & >21.12 & K2 \\ 
8115.433 & $K2$ & >21.12 & K2 \\ 
8115.454 & $K2$ & >21.12 & K2 \\ 
8115.474 & $K2$ & >21.12 & K2 \\ 
8115.494 & $K2$ & >21.12 & K2 \\ 
8115.535 & $K2$ & >21.12 & K2 \\ 
8115.556 & $K2$ & >21.12 & K2 \\ 
8115.576 & $K2$ & >21.12 & K2 \\ 
8115.597 & $K2$ & >21.12 & K2 \\ 
8115.617 & $K2$ & >21.12 & K2 \\ 
8115.637 & $K2$ & >21.12 & K2 \\ 
8115.658 & $K2$ & >21.12 & K2 \\ 
8115.678 & $K2$ & >21.12 & K2 \\ 
8115.699 & $K2$ & >21.12 & K2 \\ 
8115.719 & $K2$ & >21.12 & K2 \\ 
8115.740 & $K2$ & >21.12 & K2 \\ 
8115.780 & $K2$ & >21.12 & K2 \\ 
8115.801 & $K2$ & >21.12 & K2 \\ 
8115.821 & $K2$ & >21.12 & K2 \\ 
8115.842 & $K2$ & >21.12 & K2 \\ 
8115.862 & $K2$ & >21.12 & K2 \\ 
8115.883 & $K2$ & >21.12 & K2 \\ 
8115.903 & $K2$ & >21.12 & K2 \\ 
8115.924 & $K2$ & >21.12 & K2 \\ 
8115.944 & $K2$ & >21.12 & K2 \\ 
8115.964 & $K2$ & >21.12 & K2 \\ 
8115.985 & $K2$ & >21.12 & K2 \\ 
8116.026 & $K2$ & >21.12 & K2 \\ 
8116.046 & $K2$ & >21.12 & K2 \\ 
8116.067 & $K2$ & >21.12 & K2 \\ 
8116.087 & $K2$ & >21.12 & K2 \\ 
8116.107 & $K2$ & >21.12 & K2 \\ 
8116.128 & $K2$ & >21.12 & K2 \\ 
8116.148 & $K2$ & >21.12 & K2 \\ 
8116.169 & $K2$ & >21.12 & K2 \\ 
8116.189 & $K2$ & >21.12 & K2 \\ 
8116.210 & $K2$ & >21.12 & K2 \\ 
8116.230 & $K2$ & >21.12 & K2 \\ 
8116.250 & $K2$ & >21.12 & K2 \\ 
8116.271 & $K2$ & >21.12 & K2 \\ 
8116.291 & $K2$ & >21.12 & K2 \\ 
8116.312 & $K2$ & >21.12 & K2 \\ 
8116.332 & $K2$ & >21.12 & K2 \\ 
8116.353 & $K2$ & >21.12 & K2 \\ 
8116.373 & $K2$ & >21.12 & K2 \\ 
8116.537 & $K2$ & >21.12 & K2 \\ 
8116.557 & $K2$ & >21.12 & K2 \\ 
8116.598 & $K2$ & >21.12 & K2 \\ 
8116.618 & $K2$ & >21.12 & K2 \\ 
8116.639 & $K2$ & >21.12 & K2 \\ 
8116.659 & $K2$ & >21.12 & K2 \\ 
8116.680 & $K2$ & >21.12 & K2 \\ 
8116.700 & $K2$ & >21.12 & K2 \\ 
8116.720 & $K2$ & >21.12 & K2 \\ 
8116.761 & $K2$ & >21.12 & K2 \\ 
8116.782 & $K2$ & >21.12 & K2 \\ 
8116.802 & $K2$ & >21.12 & K2 \\ 
8116.823 & $K2$ & >21.12 & K2 \\ 
8116.843 & $K2$ & >21.12 & K2 \\ 
8116.863 & $K2$ & >21.12 & K2 \\ 
8116.884 & $K2$ & >21.12 & K2 \\ 
8116.904 & $K2$ & >21.12 & K2 \\ 
8116.925 & $K2$ & >21.12 & K2 \\ 
8116.945 & $K2$ & >21.12 & K2 \\ 
8116.966 & $K2$ & >21.12 & K2 \\ 
8117.006 & $K2$ & >21.12 & K2 \\ 
8117.027 & $K2$ & >21.12 & K2 \\ 
8117.047 & $K2$ & >21.12 & K2 \\ 
8117.068 & $K2$ & >21.12 & K2 \\ 
8117.088 & $K2$ & >21.12 & K2 \\ 
8117.109 & $K2$ & >21.12 & K2 \\ 
8117.129 & $K2$ & >21.12 & K2 \\ 
8117.150 & $K2$ & >21.12 & K2 \\ 
8117.170 & $K2$ & >21.12 & K2 \\ 
8117.190 & $K2$ & >21.12 & K2 \\ 
8117.211 & $K2$ & >21.12 & K2 \\ 
8117.252 & $K2$ & >21.12 & K2 \\ 
8117.272 & $K2$ & >21.12 & K2 \\ 
8117.293 & $K2$ & >21.12 & K2 \\ 
8117.313 & $K2$ & >21.12 & K2 \\ 
8117.333 & $K2$ & >21.12 & K2 \\ 
8117.354 & $K2$ & >21.12 & K2 \\ 
8117.374 & $K2$ & >21.12 & K2 \\ 
8117.395 & $K2$ & >21.12 & K2 \\ 
8117.415 & $K2$ & >21.12 & K2 \\ 
8117.436 & $K2$ & >21.12 & K2 \\ 
8117.456 & $K2$ & >21.12 & K2 \\ 
8117.497 & $K2$ & >21.12 & K2 \\ 
8117.517 & $K2$ & >21.12 & K2 \\ 
8117.538 & $K2$ & >21.12 & K2 \\ 
8117.558 & $K2$ & >21.12 & K2 \\ 
8117.579 & $K2$ & >21.12 & K2 \\ 
8117.599 & $K2$ & >21.12 & K2 \\ 
8117.619 & $K2$ & >21.12 & K2 \\ 
8117.640 & $K2$ & >21.12 & K2 \\ 
8117.660 & $K2$ & >21.12 & K2 \\ 
8117.681 & $K2$ & >21.12 & K2 \\ 
8117.701 & $K2$ & >21.12 & K2 \\ 
8117.742 & $K2$ & >21.12 & K2 \\ 
8117.763 & $K2$ & >21.12 & K2 \\ 
8117.783 & $K2$ & >21.12 & K2 \\ 
8117.803 & $K2$ & >21.12 & K2 \\ 
8117.824 & $K2$ & >21.12 & K2 \\ 
8117.844 & $K2$ & >21.12 & K2 \\ 
8117.865 & $K2$ & >21.12 & K2 \\ 
8117.885 & $K2$ & >21.12 & K2 \\ 
8117.906 & $K2$ & >21.12 & K2 \\ 
8117.926 & $K2$ & >21.12 & K2 \\ 
8117.946 & $K2$ & >21.12 & K2 \\ 
8117.987 & $K2$ & >21.12 & K2 \\ 
8118.008 & $K2$ & >21.12 & K2 \\ 
8118.028 & $K2$ & >21.12 & K2 \\ 
8118.049 & $K2$ & >21.12 & K2 \\ 
8118.069 & $K2$ & >21.12 & K2 \\ 
8118.089 & $K2$ & >21.12 & K2 \\ 
8118.110 & $K2$ & >21.12 & K2 \\ 
8118.130 & $K2$ & >21.12 & K2 \\ 
8118.151 & $K2$ & >21.12 & K2 \\ 
8118.171 & $K2$ & >21.12 & K2 \\ 
8118.192 & $K2$ & >21.12 & K2 \\ 
8118.232 & $K2$ & >21.12 & K2 \\ 
8118.253 & $K2$ & >21.12 & K2 \\ 
8118.273 & $K2$ & >21.12 & K2 \\ 
8118.294 & $K2$ & >21.12 & K2 \\ 
8118.314 & $K2$ & >21.12 & K2 \\ 
8118.335 & $K2$ & >21.12 & K2 \\ 
8118.355 & $K2$ & >21.12 & K2 \\ 
8118.376 & $K2$ & >21.12 & K2 \\ 
8118.396 & $K2$ & >21.12 & K2 \\ 
8118.416 & $K2$ & >21.12 & K2 \\ 
8118.437 & $K2$ & >21.12 & K2 \\ 
8118.478 & $K2$ & >21.12 & K2 \\ 
8118.498 & $K2$ & >21.12 & K2 \\ 
8118.519 & $K2$ & >21.12 & K2 \\ 
8118.539 & $K2$ & >21.12 & K2 \\ 
8118.559 & $K2$ & >21.12 & K2 \\ 
8118.580 & $K2$ & >21.12 & K2 \\ 
8118.600 & $K2$ & >21.12 & K2 \\ 
8118.621 & $K2$ & >21.12 & K2 \\ 
8118.641 & $K2$ & >21.12 & K2 \\ 
8118.662 & $K2$ & >21.12 & K2 \\ 
8118.682 & $K2$ & >21.12 & K2 \\ 
8118.723 & $K2$ & >21.12 & K2 \\ 
8118.743 & $K2$ & >21.12 & K2 \\ 
8118.764 & $K2$ & >21.12 & K2 \\ 
8118.784 & $K2$ & >21.12 & K2 \\ 
8118.805 & $K2$ & >21.12 & K2 \\ 
8118.825 & $K2$ & >21.12 & K2 \\ 
8118.968 & $K2$ & >21.12 & K2 \\ 
8118.989 & $K2$ & >21.12 & K2 \\ 
8119.009 & $K2$ & >21.12 & K2 \\ 
8119.029 & $K2$ & >21.12 & K2 \\ 
8119.050 & $K2$ & >21.12 & K2 \\ 
8119.070 & $K2$ & >21.12 & K2 \\ 
8119.091 & $K2$ & >21.12 & K2 \\ 
8119.111 & $K2$ & >21.12 & K2 \\ 
8119.132 & $K2$ & >21.12 & K2 \\ 
8119.152 & $K2$ & >21.12 & K2 \\ 
8119.172 & $K2$ & >21.12 & K2 \\ 
8119.193 & $K2$ & >21.12 & K2 \\ 
8119.213 & $K2$ & >21.12 & K2 \\ 
8119.234 & $K2$ & >21.12 & K2 \\ 
8119.254 & $K2$ & >21.12 & K2 \\ 
8119.275 & $K2$ & >21.12 & K2 \\ 
8119.295 & $K2$ & >21.12 & K2 \\ 
8119.315 & $K2$ & >21.12 & K2 \\ 
8119.336 & $K2$ & >21.12 & K2 \\ 
8119.356 & $K2$ & >21.12 & K2 \\ 
8119.377 & $K2$ & >21.12 & K2 \\ 
8119.397 & $K2$ & >21.12 & K2 \\ 
8119.418 & $K2$ & >21.12 & K2 \\ 
8119.459 & $K2$ & >21.12 & K2 \\ 
8119.479 & $K2$ & >21.12 & K2 \\ 
8119.499 & $K2$ & >21.12 & K2 \\ 
8119.520 & $K2$ & >21.12 & K2 \\ 
8119.540 & $K2$ & >21.12 & K2 \\ 
8119.561 & $K2$ & >21.12 & K2 \\ 
8119.581 & $K2$ & >21.12 & K2 \\ 
8119.602 & $K2$ & >21.12 & K2 \\ 
8119.622 & $K2$ & >21.12 & K2 \\ 
8119.642 & $K2$ & >21.12 & K2 \\ 
8119.663 & $K2$ & >21.12 & K2 \\ 
8119.704 & $K2$ & >21.12 & K2 \\ 
8119.724 & $K2$ & >21.12 & K2 \\ 
8119.745 & $K2$ & >21.12 & K2 \\ 
8119.765 & $K2$ & >21.12 & K2 \\ 
8119.785 & $K2$ & >21.12 & K2 \\ 
8119.806 & $K2$ & >21.12 & K2 \\ 
8119.826 & $K2$ & >21.12 & K2 \\ 
8119.847 & $K2$ & >21.12 & K2 \\ 
8119.867 & $K2$ & >21.12 & K2 \\ 
8119.888 & $K2$ & >21.12 & K2 \\ 
8119.908 & $K2$ & >21.12 & K2 \\ 
8119.949 & $K2$ & >21.12 & K2 \\ 
8119.969 & $K2$ & >21.12 & K2 \\ 
8119.990 & $K2$ & >21.12 & K2 \\ 
8120.010 & $K2$ & >21.12 & K2 \\ 
8120.031 & $K2$ & >21.12 & K2 \\ 
8120.051 & $K2$ & >21.12 & K2 \\ 
8120.072 & $K2$ & >21.12 & K2 \\ 
8120.092 & $K2$ & >21.12 & K2 \\ 
8120.112 & $K2$ & >21.12 & K2 \\ 
8120.133 & $K2$ & >21.12 & K2 \\ 
8120.153 & $K2$ & >21.12 & K2 \\ 
8120.194 & $K2$ & >21.12 & K2 \\ 
8120.215 & $K2$ & >21.12 & K2 \\ 
8120.235 & $K2$ & >21.12 & K2 \\ 
8120.255 & $K2$ & >21.12 & K2 \\ 
8120.276 & $K2$ & >21.12 & K2 \\ 
8120.296 & $K2$ & >21.12 & K2 \\ 
8120.317 & $K2$ & >21.12 & K2 \\ 
8120.337 & $K2$ & >21.12 & K2 \\ 
8120.358 & $K2$ & >21.12 & K2 \\ 
8120.378 & $K2$ & >21.12 & K2 \\ 
8120.398 & $K2$ & >21.12 & K2 \\ 
8120.439 & $K2$ & >21.12 & K2 \\ 
8120.460 & $K2$ & >21.12 & K2 \\ 
8120.480 & $K2$ & >21.12 & K2 \\ 
8120.501 & $K2$ & >21.12 & K2 \\ 
8120.521 & $K2$ & >21.12 & K2 \\ 
8120.541 & $K2$ & >21.12 & K2 \\ 
8120.562 & $K2$ & >21.12 & K2 \\ 
8120.582 & $K2$ & >21.12 & K2 \\ 
8120.603 & $K2$ & >21.12 & K2 \\ 
8120.623 & $K2$ & >21.12 & K2 \\ 
8120.644 & $K2$ & >21.12 & K2 \\ 
8120.685 & $K2$ & >21.12 & K2 \\ 
8120.705 & $K2$ & >21.12 & K2 \\ 
8120.725 & $K2$ & >21.12 & K2 \\ 
8120.746 & $K2$ & >21.12 & K2 \\ 
8120.766 & $K2$ & >21.12 & K2 \\ 
8120.787 & $K2$ & >21.12 & K2 \\ 
8120.807 & $K2$ & >21.12 & K2 \\ 
8120.828 & $K2$ & >21.12 & K2 \\ 
8120.848 & $K2$ & >21.12 & K2 \\ 
8120.868 & $K2$ & >21.12 & K2 \\ 
8120.889 & $K2$ & >21.12 & K2 \\ 
8120.930 & $K2$ & >21.12 & K2 \\ 
8120.950 & $K2$ & >21.12 & K2 \\ 
8120.971 & $K2$ & >21.12 & K2 \\ 
8120.991 & $K2$ & >21.12 & K2 \\ 
8121.011 & $K2$ & >21.12 & K2 \\ 
8121.032 & $K2$ & >21.12 & K2 \\ 
8121.052 & $K2$ & >21.12 & K2 \\ 
8121.073 & $K2$ & >21.12 & K2 \\ 
8121.093 & $K2$ & >21.12 & K2 \\ 
8121.114 & $K2$ & >21.12 & K2 \\ 
8121.134 & $K2$ & >21.12 & K2 \\ 
8121.155 & $K2$ & >21.12 & K2 \\ 
8121.175 & $K2$ & >21.12 & K2 \\ 
8121.195 & $K2$ & >21.12 & K2 \\ 
8121.216 & $K2$ & >21.12 & K2 \\ 
8121.236 & $K2$ & >21.12 & K2 \\ 
8121.257 & $K2$ & >21.12 & K2 \\ 
8121.277 & $K2$ & >21.12 & K2 \\ 
8121.298 & $K2$ & >21.12 & K2 \\ 
8121.318 & $K2$ & >21.12 & K2 \\ 
8121.338 & $K2$ & >21.12 & K2 \\ 
8121.359 & $K2$ & >21.12 & K2 \\ 
8121.379 & $K2$ & >21.12 & K2 \\ 
8121.420 & $K2$ & >21.12 & K2 \\ 
8121.441 & $K2$ & >21.12 & K2 \\ 
8121.461 & $K2$ & >21.12 & K2 \\ 
8121.481 & $K2$ & >21.12 & K2 \\ 
8121.502 & $K2$ & >21.12 & K2 \\ 
8121.522 & $K2$ & >21.12 & K2 \\ 
8121.543 & $K2$ & >21.12 & K2 \\ 
8121.563 & $K2$ & >21.12 & K2 \\ 
8121.584 & $K2$ & >21.12 & K2 \\ 
8121.604 & $K2$ & >21.12 & K2 \\ 
8121.624 & $K2$ & >21.12 & K2 \\ 
8121.665 & $K2$ & >21.12 & K2 \\ 
8121.686 & $K2$ & >21.12 & K2 \\ 
8121.706 & $K2$ & >21.12 & K2 \\ 
8121.747 & $K2$ & >21.12 & K2 \\ 
8121.768 & $K2$ & >21.12 & K2 \\ 
8121.788 & $K2$ & >21.12 & K2 \\ 
8121.808 & $K2$ & >21.12 & K2 \\ 
8121.829 & $K2$ & >21.12 & K2 \\ 
8121.849 & $K2$ & >21.12 & K2 \\ 
8121.870 & $K2$ & >21.12 & K2 \\ 
8121.911 & $K2$ & >21.12 & K2 \\ 
8121.931 & $K2$ & >21.12 & K2 \\ 
8121.951 & $K2$ & >21.12 & K2 \\ 
8121.972 & $K2$ & >21.12 & K2 \\ 
8121.992 & $K2$ & >21.12 & K2 \\ 
8122.013 & $K2$ & >21.12 & K2 \\ 
8122.033 & $K2$ & >21.12 & K2 \\ 
8122.054 & $K2$ & >21.12 & K2 \\ 
8122.074 & $K2$ & >21.12 & K2 \\ 
8122.094 & $K2$ & >21.12 & K2 \\ 
8122.115 & $K2$ & >21.12 & K2 \\ 
8122.156 & $K2$ & >21.12 & K2 \\ 
8122.176 & $K2$ & >21.12 & K2 \\ 
8122.197 & $K2$ & >21.12 & K2 \\ 
8122.217 & $K2$ & >21.12 & K2 \\ 
8122.237 & $K2$ & >21.12 & K2 \\ 
8122.258 & $K2$ & >21.12 & K2 \\ 
8122.278 & $K2$ & >21.12 & K2 \\ 
8122.299 & $K2$ & >21.12 & K2 \\ 
8122.319 & $K2$ & >21.12 & K2 \\ 
8122.340 & $K2$ & >21.12 & K2 \\ 
8122.360 & $K2$ & >21.12 & K2 \\ 
8122.401 & $K2$ & >21.12 & K2 \\ 
8122.421 & $K2$ & >21.12 & K2 \\ 
8122.442 & $K2$ & >21.12 & K2 \\ 
8122.462 & $K2$ & >21.12 & K2 \\ 
8122.483 & $K2$ & >21.12 & K2 \\ 
8122.503 & $K2$ & >21.12 & K2 \\ 
8122.524 & $K2$ & >21.12 & K2 \\ 
8122.544 & $K2$ & >21.12 & K2 \\ 
8122.564 & $K2$ & >21.12 & K2 \\ 
8122.585 & $K2$ & >21.12 & K2 \\ 
8122.605 & $K2$ & >21.12 & K2 \\ 
8122.646 & $K2$ & >21.12 & K2 \\ 
8122.667 & $K2$ & >21.12 & K2 \\ 
8122.687 & $K2$ & >21.12 & K2 \\ 
8122.707 & $K2$ & >21.12 & K2 \\ 
8122.728 & $K2$ & >21.12 & K2 \\ 
8122.748 & $K2$ & >21.12 & K2 \\ 
8122.769 & $K2$ & >21.12 & K2 \\ 
8122.789 & $K2$ & >21.12 & K2 \\ 
8122.810 & $K2$ & >21.12 & K2 \\ 
8122.830 & $K2$ & >21.12 & K2 \\ 
8122.850 & $K2$ & >21.12 & K2 \\ 
8122.912 & $K2$ & >21.12 & K2 \\ 
8122.932 & $K2$ & >21.12 & K2 \\ 
8122.953 & $K2$ & >21.12 & K2 \\ 
8122.973 & $K2$ & >21.12 & K2 \\ 
8122.994 & $K2$ & >21.12 & K2 \\ 
8123.014 & $K2$ & >21.12 & K2 \\ 
8123.034 & $K2$ & >21.12 & K2 \\ 
8123.055 & $K2$ & >21.12 & K2 \\ 
8123.075 & $K2$ & >21.12 & K2 \\ 
8123.096 & $K2$ & >21.12 & K2 \\ 
8123.137 & $K2$ & >21.12 & K2 \\ 
8123.157 & $K2$ & >21.12 & K2 \\ 
8123.177 & $K2$ & >21.12 & K2 \\ 
8123.198 & $K2$ & >21.12 & K2 \\ 
8123.218 & $K2$ & >21.12 & K2 \\ 
8123.239 & $K2$ & >21.12 & K2 \\ 
8123.259 & $K2$ & >21.12 & K2 \\ 
8123.280 & $K2$ & >21.12 & K2 \\ 
8123.300 & $K2$ & >21.12 & K2 \\ 
8123.320 & $K2$ & >21.12 & K2 \\ 
8123.341 & $K2$ & >21.12 & K2 \\ 
8123.382 & $K2$ & >21.12 & K2 \\ 
8123.402 & $K2$ & >21.12 & K2 \\ 
8123.423 & $K2$ & >21.12 & K2 \\ 
8123.443 & $K2$ & >21.12 & K2 \\ 
8123.464 & $K2$ & >21.12 & K2 \\ 
8123.484 & $K2$ & >21.12 & K2 \\ 
8123.504 & $K2$ & >21.12 & K2 \\ 
8123.525 & $K2$ & >21.12 & K2 \\ 
8123.545 & $K2$ & >21.12 & K2 \\ 
8123.566 & $K2$ & >21.12 & K2 \\ 
8123.586 & $K2$ & >21.12 & K2 \\ 
8123.627 & $K2$ & >21.12 & K2 \\ 
8123.647 & $K2$ & >21.12 & K2 \\ 
8123.668 & $K2$ & >21.12 & K2 \\ 
8123.688 & $K2$ & >21.12 & K2 \\ 
8123.709 & $K2$ & >21.12 & K2 \\ 
8123.729 & $K2$ & >21.12 & K2 \\ 
8123.750 & $K2$ & >21.12 & K2 \\ 
8123.770 & $K2$ & >21.12 & K2 \\ 
8123.790 & $K2$ & >21.12 & K2 \\ 
8123.811 & $K2$ & >21.12 & K2 \\ 
8123.831 & $K2$ & >21.12 & K2 \\ 
8123.872 & $K2$ & >21.12 & K2 \\ 
8123.893 & $K2$ & >21.12 & K2 \\ 
8123.913 & $K2$ & >21.12 & K2 \\ 
8123.933 & $K2$ & >21.12 & K2 \\ 
8123.954 & $K2$ & >21.12 & K2 \\ 
8123.974 & $K2$ & >21.12 & K2 \\ 
8123.995 & $K2$ & >21.12 & K2 \\ 
8124.015 & $K2$ & >21.12 & K2 \\ 
8124.036 & $K2$ & >21.12 & K2 \\ 
8124.056 & $K2$ & >21.12 & K2 \\ 
8124.077 & $K2$ & >21.12 & K2 \\ 
8124.117 & $K2$ & >21.12 & K2 \\ 
8124.138 & $K2$ & >21.12 & K2 \\ 
8124.158 & $K2$ & >21.12 & K2 \\ 
8124.199 & $K2$ & >21.12 & K2 \\ 
8124.220 & $K2$ & >21.12 & K2 \\ 
8124.240 & $K2$ & >21.12 & K2 \\ 
8124.260 & $K2$ & >21.12 & K2 \\ 
8124.281 & $K2$ & >21.12 & K2 \\ 
8124.301 & $K2$ & >21.12 & K2 \\ 
8124.322 & $K2$ & >21.12 & K2 \\ 
8124.363 & $K2$ & >21.12 & K2 \\ 
8124.383 & $K2$ & >21.12 & K2 \\ 
8124.403 & $K2$ & >21.12 & K2 \\ 
8124.424 & $K2$ & >21.12 & K2 \\ 
8124.444 & $K2$ & >21.12 & K2 \\ 
8124.465 & $K2$ & >21.12 & K2 \\ 
8124.485 & $K2$ & >21.12 & K2 \\ 
8124.506 & $K2$ & >21.12 & K2 \\ 
8124.526 & $K2$ & >21.12 & K2 \\ 
8124.546 & $K2$ & >21.12 & K2 \\ 
8124.567 & $K2$ & >21.12 & K2 \\ 
8124.608 & $K2$ & >21.12 & K2 \\ 
8124.628 & $K2$ & >21.12 & K2 \\ 
8124.649 & $K2$ & >21.12 & K2 \\ 
8124.669 & $K2$ & >21.12 & K2 \\ 
8124.690 & $K2$ & >21.12 & K2 \\ 
8124.710 & $K2$ & >21.12 & K2 \\ 
8124.730 & $K2$ & >21.12 & K2 \\ 
8124.751 & $K2$ & >21.12 & K2 \\ 
8124.792 & $K2$ & >21.12 & K2 \\ 
8124.812 & $K2$ & >21.12 & K2 \\ 
8124.853 & $K2$ & >21.12 & K2 \\ 
8124.873 & $K2$ & >21.12 & K2 \\ 
8124.894 & $K2$ & >21.12 & K2 \\ 
8124.914 & $K2$ & >21.12 & K2 \\ 
8124.935 & $K2$ & >21.12 & K2 \\ 
8124.955 & $K2$ & >21.12 & K2 \\ 
8124.976 & $K2$ & >21.12 & K2 \\ 
8124.996 & $K2$ & >21.12 & K2 \\ 
8125.016 & $K2$ & >21.12 & K2 \\ 
8125.037 & $K2$ & >21.12 & K2 \\ 
8125.057 & $K2$ & >21.12 & K2 \\ 
8125.078 & $K2$ & >21.12 & K2 \\ 
8125.098 & $K2$ & >21.12 & K2 \\ 
8125.119 & $K2$ & >21.12 & K2 \\ 
8125.139 & $K2$ & >21.12 & K2 \\ 
8125.159 & $K2$ & >21.12 & K2 \\ 
8125.180 & $K2$ & >21.12 & K2 \\ 
8125.200 & $K2$ & >21.12 & K2 \\ 
8125.221 & $K2$ & >21.12 & K2 \\ 
8125.241 & $K2$ & >21.12 & K2 \\ 
8125.262 & $K2$ & >21.12 & K2 \\ 
8125.282 & $K2$ & >21.12 & K2 \\ 
8125.303 & $K2$ & >21.12 & K2 \\ 
8125.343 & $K2$ & >21.12 & K2 \\ 
8125.364 & $K2$ & >21.12 & K2 \\ 
8125.384 & $K2$ & >21.12 & K2 \\ 
8125.405 & $K2$ & >21.12 & K2 \\ 
8125.425 & $K2$ & >21.12 & K2 \\ 
8125.446 & $K2$ & >21.12 & K2 \\ 
8125.466 & $K2$ & >21.12 & K2 \\ 
8125.486 & $K2$ & >21.12 & K2 \\ 
8125.507 & $K2$ & >21.12 & K2 \\ 
8125.527 & $K2$ & >21.12 & K2 \\ 
8125.548 & $K2$ & >21.12 & K2 \\ 
8125.589 & $K2$ & >21.12 & K2 \\ 
8125.609 & $K2$ & >21.12 & K2 \\ 
8125.629 & $K2$ & >21.12 & K2 \\ 
8125.650 & $K2$ & >21.12 & K2 \\ 
8125.670 & $K2$ & >21.12 & K2 \\ 
8125.691 & $K2$ & >21.12 & K2 \\ 
8125.711 & $K2$ & >21.12 & K2 \\ 
8125.732 & $K2$ & >21.12 & K2 \\ 
8125.752 & $K2$ & >21.12 & K2 \\ 
8125.772 & $K2$ & >21.12 & K2 \\ 
8125.793 & $K2$ & >21.12 & K2 \\ 
8125.834 & $K2$ & >21.12 & K2 \\ 
8125.854 & $K2$ & >21.12 & K2 \\ 
8125.875 & $K2$ & >21.12 & K2 \\ 
8125.895 & $K2$ & >21.12 & K2 \\ 
8125.916 & $K2$ & >21.12 & K2 \\ 
8125.936 & $K2$ & >21.12 & K2 \\ 
8125.956 & $K2$ & >21.12 & K2 \\ 
8125.977 & $K2$ & >21.12 & K2 \\ 
8125.997 & $K2$ & >21.12 & K2 \\ 
8126.018 & $K2$ & >21.12 & K2 \\ 
8126.038 & $K2$ & >21.12 & K2 \\ 
8126.079 & $K2$ & >21.12 & K2 \\ 
8126.099 & $K2$ & >21.12 & K2 \\ 
8126.120 & $K2$ & >21.12 & K2 \\ 
8126.140 & $K2$ & >21.12 & K2 \\ 
8126.161 & $K2$ & >21.12 & K2 \\ 
8126.181 & $K2$ & >21.12 & K2 \\ 
8126.202 & $K2$ & >21.12 & K2 \\ 
8126.222 & $K2$ & >21.12 & K2 \\ 
8126.242 & $K2$ & >21.12 & K2 \\ 
8126.263 & $K2$ & >21.12 & K2 \\ 
8126.283 & $K2$ & >21.12 & K2 \\ 
8126.324 & $K2$ & >21.12 & K2 \\ 
8126.345 & $K2$ & >21.12 & K2 \\ 
8126.365 & $K2$ & >21.12 & K2 \\ 
8126.386 & $K2$ & >21.12 & K2 \\ 
8126.406 & $K2$ & >21.12 & K2 \\ 
8126.426 & $K2$ & >21.12 & K2 \\ 
8126.447 & $K2$ & >21.12 & K2 \\ 
8126.467 & $K2$ & >21.12 & K2 \\ 
8126.488 & $K2$ & >21.12 & K2 \\ 
8126.508 & $K2$ & >21.12 & K2 \\ 
8126.529 & $K2$ & >21.12 & K2 \\ 
8126.569 & $K2$ & >21.12 & K2 \\ 
8126.590 & $K2$ & >21.12 & K2 \\ 
8126.610 & $K2$ & >21.12 & K2 \\ 
8126.631 & $K2$ & >21.12 & K2 \\ 
8126.651 & $K2$ & >21.12 & K2 \\ 
8126.672 & $K2$ & >21.12 & K2 \\ 
8126.692 & $K2$ & >21.12 & K2 \\ 
8126.712 & $K2$ & >21.12 & K2 \\ 
8126.733 & $K2$ & >21.12 & K2 \\ 
8126.753 & $K2$ & >21.12 & K2 \\ 
8126.774 & $K2$ & >21.12 & K2 \\ 
8126.815 & $K2$ & >21.12 & K2 \\ 
8126.835 & $K2$ & >21.12 & K2 \\ 
8126.855 & $K2$ & >21.12 & K2 \\ 
8126.876 & $K2$ & >21.12 & K2 \\ 
8126.896 & $K2$ & >21.12 & K2 \\ 
8126.917 & $K2$ & >21.12 & K2 \\ 
8126.937 & $K2$ & >21.12 & K2 \\ 
8126.958 & $K2$ & >21.12 & K2 \\ 
8126.999 & $K2$ & >21.12 & K2 \\ 
8127.019 & $K2$ & >21.12 & K2 \\ 
8127.039 & $K2$ & >21.12 & K2 \\ 
8127.060 & $K2$ & >21.12 & K2 \\ 
8127.080 & $K2$ & >21.12 & K2 \\ 
8127.101 & $K2$ & >21.12 & K2 \\ 
8127.121 & $K2$ & >21.12 & K2 \\ 
8127.142 & $K2$ & >21.12 & K2 \\ 
8127.162 & $K2$ & >21.12 & K2 \\ 
8127.182 & $K2$ & >21.12 & K2 \\ 
8127.203 & $K2$ & >21.12 & K2 \\ 
8127.223 & $K2$ & >21.12 & K2 \\ 
8127.244 & $K2$ & >21.12 & K2 \\ 
8127.264 & $K2$ & >21.12 & K2 \\ 
8127.305 & $K2$ & >21.12 & K2 \\ 
8127.325 & $K2$ & >21.12 & K2 \\ 
8127.366 & $K2$ & >21.12 & K2 \\ 
8127.387 & $K2$ & >21.12 & K2 \\ 
8127.407 & $K2$ & >21.12 & K2 \\ 
8127.428 & $K2$ & >21.12 & K2 \\ 
8127.448 & $K2$ & >21.12 & K2 \\ 
8127.468 & $K2$ & >21.12 & K2 \\ 
8127.489 & $K2$ & >21.12 & K2 \\ 
8127.509 & $K2$ & >21.12 & K2 \\ 
8127.550 & $K2$ & >21.12 & K2 \\ 
8127.571 & $K2$ & >21.12 & K2 \\ 
8127.591 & $K2$ & >21.12 & K2 \\ 
8127.612 & $K2$ & >21.12 & K2 \\ 
8127.632 & $K2$ & >21.12 & K2 \\ 
8127.652 & $K2$ & >21.12 & K2 \\ 
8127.673 & $K2$ & >21.12 & K2 \\ 
8127.693 & $K2$ & >21.12 & K2 \\ 
8127.714 & $K2$ & >21.12 & K2 \\ 
8127.734 & $K2$ & >21.12 & K2 \\ 
8127.755 & $K2$ & >21.12 & K2 \\ 
8127.795 & $K2$ & >21.12 & K2 \\ 
8127.816 & $K2$ & >21.12 & K2 \\ 
8127.836 & $K2$ & >21.12 & K2 \\ 
8127.857 & $K2$ & >21.12 & K2 \\ 
8127.877 & $K2$ & >21.12 & K2 \\ 
8127.898 & $K2$ & >21.12 & K2 \\ 
8127.918 & $K2$ & >21.12 & K2 \\ 
8127.938 & $K2$ & >21.12 & K2 \\ 
8127.959 & $K2$ & >21.12 & K2 \\ 
8127.979 & $K2$ & >21.12 & K2 \\ 
8128.000 & $K2$ & >21.12 & K2 \\ 
8128.041 & $K2$ & >21.12 & K2 \\ 
8128.061 & $K2$ & >21.12 & K2 \\ 
8128.081 & $K2$ & >21.12 & K2 \\ 
8128.102 & $K2$ & >21.12 & K2 \\ 
8128.122 & $K2$ & >21.12 & K2 \\ 
8128.143 & $K2$ & >21.12 & K2 \\ 
8128.163 & $K2$ & >21.12 & K2 \\ 
8128.184 & $K2$ & >21.12 & K2 \\ 
8128.204 & $K2$ & >21.12 & K2 \\ 
8128.225 & $K2$ & >21.12 & K2 \\ 
8128.245 & $K2$ & >21.12 & K2 \\ 
8128.286 & $K2$ & >21.12 & K2 \\ 
8128.306 & $K2$ & >21.12 & K2 \\ 
8128.327 & $K2$ & >21.12 & K2 \\ 
8128.347 & $K2$ & >21.12 & K2 \\ 
8128.368 & $K2$ & >21.12 & K2 \\ 
8128.388 & $K2$ & >21.12 & K2 \\ 
8128.408 & $K2$ & >21.12 & K2 \\ 
8128.429 & $K2$ & >21.12 & K2 \\ 
8128.449 & $K2$ & >21.12 & K2 \\ 
8128.470 & $K2$ & >21.12 & K2 \\ 
8128.490 & $K2$ & >21.12 & K2 \\ 
8128.531 & $K2$ & >21.12 & K2 \\ 
8128.551 & $K2$ & >21.12 & K2 \\ 
8128.572 & $K2$ & >21.12 & K2 \\ 
8128.592 & $K2$ & >21.12 & K2 \\ 
8128.613 & $K2$ & >21.12 & K2 \\ 
8128.633 & $K2$ & >21.12 & K2 \\ 
8128.654 & $K2$ & >21.12 & K2 \\ 
8128.674 & $K2$ & >21.12 & K2 \\ 
8128.695 & $K2$ & >21.12 & K2 \\ 
8128.715 & $K2$ & >21.12 & K2 \\ 
8128.735 & $K2$ & >21.12 & K2 \\ 
8128.776 & $K2$ & >21.12 & K2 \\ 
8128.797 & $K2$ & >21.12 & K2 \\ 
8128.817 & $K2$ & >21.12 & K2 \\ 
8128.838 & $K2$ & >21.12 & K2 \\ 
8128.858 & $K2$ & >21.12 & K2 \\ 
8128.878 & $K2$ & >21.12 & K2 \\ 
8128.899 & $K2$ & >21.12 & K2 \\ 
8128.919 & $K2$ & >21.12 & K2 \\ 
8128.940 & $K2$ & >21.12 & K2 \\ 
8128.960 & $K2$ & >21.12 & K2 \\ 
8128.981 & $K2$ & >21.12 & K2 \\ 
8129.021 & $K2$ & >21.12 & K2 \\ 
8129.042 & $K2$ & >21.12 & K2 \\ 
8129.062 & $K2$ & >21.12 & K2 \\ 
8129.083 & $K2$ & >21.12 & K2 \\ 
8129.103 & $K2$ & >21.12 & K2 \\ 
8129.124 & $K2$ & >21.12 & K2 \\ 
8129.144 & $K2$ & >21.12 & K2 \\ 
8129.164 & $K2$ & >21.12 & K2 \\ 
8129.185 & $K2$ & >21.12 & K2 \\ 
8129.205 & $K2$ & >21.12 & K2 \\ 
8129.226 & $K2$ & >21.12 & K2 \\ 
8129.246 & $K2$ & >21.12 & K2 \\ 
8129.267 & $K2$ & >21.12 & K2 \\ 
8129.287 & $K2$ & >21.12 & K2 \\ 
8129.308 & $K2$ & >21.12 & K2 \\ 
8129.328 & $K2$ & >21.12 & K2 \\ 
8129.348 & $K2$ & >21.12 & K2 \\ 
8129.369 & $K2$ & >21.12 & K2 \\ 
8129.389 & $K2$ & >21.12 & K2 \\ 
8129.410 & $K2$ & >21.12 & K2 \\ 
8129.430 & $K2$ & >21.12 & K2 \\ 
8129.451 & $K2$ & >21.12 & K2 \\ 
8129.471 & $K2$ & >21.12 & K2 \\ 
8129.512 & $K2$ & >21.12 & K2 \\ 
8129.532 & $K2$ & >21.12 & K2 \\ 
8129.553 & $K2$ & >21.12 & K2 \\ 
8129.573 & $K2$ & >21.12 & K2 \\ 
8129.594 & $K2$ & >21.12 & K2 \\ 
8129.614 & $K2$ & >21.12 & K2 \\ 
8129.634 & $K2$ & >21.12 & K2 \\ 
8129.655 & $K2$ & >21.12 & K2 \\ 
8129.675 & $K2$ & >21.12 & K2 \\ 
8129.696 & $K2$ & >21.12 & K2 \\ 
8129.716 & $K2$ & >21.12 & K2 \\ 
8129.737 & $K2$ & >21.12 & K2 \\ 
8129.757 & $K2$ & >21.12 & K2 \\ 
8129.777 & $K2$ & >21.12 & K2 \\ 
8129.798 & $K2$ & >21.12 & K2 \\ 
8129.818 & $K2$ & >21.12 & K2 \\ 
8129.839 & $K2$ & >21.12 & K2 \\ 
8129.859 & $K2$ & >21.12 & K2 \\ 
8129.880 & $K2$ & >21.12 & K2 \\ 
8129.900 & $K2$ & >21.12 & K2 \\ 
8129.921 & $K2$ & >21.12 & K2 \\ 
8129.941 & $K2$ & >21.12 & K2 \\ 
8129.961 & $K2$ & >21.12 & K2 \\ 
8129.982 & $K2$ & >21.12 & K2 \\ 
8130.002 & $K2$ & >21.12 & K2 \\ 
8130.023 & $K2$ & >21.12 & K2 \\ 
8130.043 & $K2$ & >21.12 & K2 \\ 
8130.064 & $K2$ & >21.12 & K2 \\ 
8130.084 & $K2$ & >21.12 & K2 \\ 
8130.104 & $K2$ & >21.12 & K2 \\ 
8130.125 & $K2$ & >21.12 & K2 \\ 
8130.145 & $K2$ & >21.12 & K2 \\ 
8130.166 & $K2$ & >21.12 & K2 \\ 
8130.186 & $K2$ & >21.12 & K2 \\ 
8130.207 & $K2$ & >21.12 & K2 \\ 
8130.227 & $K2$ & >21.12 & K2 \\ 
8130.247 & $K2$ & >21.12 & K2 \\ 
8130.268 & $K2$ & >21.12 & K2 \\ 
8130.288 & $K2$ & >21.12 & K2 \\ 
8130.309 & $K2$ & >21.12 & K2 \\ 
8130.329 & $K2$ & >21.12 & K2 \\ 
8130.350 & $K2$ & >21.12 & K2 \\ 
8130.370 & $K2$ & >21.12 & K2 \\ 
8130.390 & $K2$ & >21.12 & K2 \\ 
8130.411 & $K2$ & >21.12 & K2 \\ 
8130.431 & $K2$ & >21.12 & K2 \\ 
8130.452 & $K2$ & >21.12 & K2 \\ 
8130.472 & $K2$ & >21.12 & K2 \\ 
8130.493 & $K2$ & >21.12 & K2 \\ 
8130.513 & $K2$ & >21.12 & K2 \\ 
8130.534 & $K2$ & >21.12 & K2 \\ 
8130.554 & $K2$ & >21.12 & K2 \\ 
8130.574 & $K2$ & >21.12 & K2 \\ 
8130.595 & $K2$ & >21.12 & K2 \\ 
8130.615 & $K2$ & >21.12 & K2 \\ 
8130.636 & $K2$ & >21.12 & K2 \\ 
8130.656 & $K2$ & >21.12 & K2 \\ 
8130.677 & $K2$ & >21.12 & K2 \\ 
8130.738 & $K2$ & >21.12 & K2 \\ 
8130.758 & $K2$ & >21.12 & K2 \\ 
8130.779 & $K2$ & >21.12 & K2 \\ 
8130.799 & $K2$ & >21.12 & K2 \\ 
8130.820 & $K2$ & >21.12 & K2 \\ 
8130.840 & $K2$ & >21.12 & K2 \\ 
8130.860 & $K2$ & >21.12 & K2 \\ 
8130.881 & $K2$ & >21.12 & K2 \\ 
8130.901 & $K2$ & >21.12 & K2 \\ 
8130.922 & $K2$ & >21.12 & K2 \\ 
8130.942 & $K2$ & >21.12 & K2 \\ 
8130.963 & $K2$ & >21.12 & K2 \\ 
8130.983 & $K2$ & >21.12 & K2 \\ 
8131.004 & $K2$ & >21.12 & K2 \\ 
8131.024 & $K2$ & >21.12 & K2 \\ 
8131.044 & $K2$ & >21.12 & K2 \\ 
8131.065 & $K2$ & >21.12 & K2 \\ 
8131.085 & $K2$ & >21.12 & K2 \\ 
8131.106 & $K2$ & >21.12 & K2 \\ 
8131.126 & $K2$ & >21.12 & K2 \\ 
8131.147 & $K2$ & >21.12 & K2 \\ 
8131.167 & $K2$ & >21.12 & K2 \\ 
8131.187 & $K2$ & >21.12 & K2 \\ 
8131.208 & $K2$ & >21.12 & K2 \\ 
8131.228 & $K2$ & >21.12 & K2 \\ 
8131.249 & $K2$ & >21.12 & K2 \\ 
8131.269 & $K2$ & >21.12 & K2 \\ 
8131.290 & $K2$ & >21.12 & K2 \\ 
8131.310 & $K2$ & >21.12 & K2 \\ 
8131.330 & $K2$ & >21.12 & K2 \\ 
8131.351 & $K2$ & >21.12 & K2 \\ 
8131.371 & $K2$ & >21.12 & K2 \\ 
8131.392 & $K2$ & >21.12 & K2 \\ 
8131.412 & $K2$ & >21.12 & K2 \\ 
8131.433 & $K2$ & >21.12 & K2 \\ 
8131.453 & $K2$ & >21.12 & K2 \\ 
8131.473 & $K2$ & >21.12 & K2 \\ 
8131.494 & $K2$ & >21.12 & K2 \\ 
8131.514 & $K2$ & >21.12 & K2 \\ 
8131.535 & $K2$ & >21.12 & K2 \\ 
8131.555 & $K2$ & >21.12 & K2 \\ 
8131.576 & $K2$ & >21.12 & K2 \\ 
8131.596 & $K2$ & >21.12 & K2 \\ 
8131.617 & $K2$ & >21.12 & K2 \\ 
8131.637 & $K2$ & >21.12 & K2 \\ 
8131.657 & $K2$ & >21.12 & K2 \\ 
8131.678 & $K2$ & >21.12 & K2 \\ 
8131.698 & $K2$ & >21.12 & K2 \\ 
8131.719 & $K2$ & >21.12 & K2 \\ 
8131.739 & $K2$ & >21.12 & K2 \\ 
8131.760 & $K2$ & >21.12 & K2 \\ 
8131.780 & $K2$ & >21.12 & K2 \\ 
8131.800 & $K2$ & >21.12 & K2 \\ 
8131.821 & $K2$ & >21.12 & K2 \\ 
8131.841 & $K2$ & >21.12 & K2 \\ 
8131.862 & $K2$ & >21.12 & K2 \\ 
8131.882 & $K2$ & >21.12 & K2 \\ 
8131.903 & $K2$ & >21.12 & K2 \\ 
8131.923 & $K2$ & >21.12 & K2 \\ 
8131.943 & $K2$ & >21.12 & K2 \\ 
8131.964 & $K2$ & >21.12 & K2 \\ 
8131.984 & $K2$ & >21.12 & K2 \\ 
8132.005 & $K2$ & >21.12 & K2 \\ 
8132.025 & $K2$ & >21.12 & K2 \\ 
8132.046 & $K2$ & >21.12 & K2 \\ 
8132.066 & $K2$ & >21.12 & K2 \\ 
8132.086 & $K2$ & >21.12 & K2 \\ 
8132.107 & $K2$ & >21.12 & K2 \\ 
8132.127 & $K2$ & >21.12 & K2 \\ 
8132.168 & $K2$ & >21.12 & K2 \\ 
8132.189 & $K2$ & >21.12 & K2 \\ 
8132.209 & $K2$ & >21.12 & K2 \\ 
8132.230 & $K2$ & >21.12 & K2 \\ 
8132.250 & $K2$ & >21.12 & K2 \\ 
8132.270 & $K2$ & >21.12 & K2 \\ 
8132.291 & $K2$ & >21.12 & K2 \\ 
8132.311 & $K2$ & >21.12 & K2 \\ 
8132.332 & $K2$ & >21.12 & K2 \\ 
8132.352 & $K2$ & >21.12 & K2 \\ 
8132.373 & $K2$ & >21.12 & K2 \\ 
8132.393 & $K2$ & >21.12 & K2 \\ 
8132.413 & $K2$ & >21.12 & K2 \\ 
8132.434 & $K2$ & >21.12 & K2 \\ 
8132.454 & $K2$ & >21.12 & K2 \\ 
8132.475 & $K2$ & >21.12 & K2 \\ 
8132.495 & $K2$ & >21.12 & K2 \\ 
8132.516 & $K2$ & >21.12 & K2 \\ 
8132.536 & $K2$ & >21.12 & K2 \\ 
8132.556 & $K2$ & >21.12 & K2 \\ 
8132.577 & $K2$ & >21.12 & K2 \\ 
8132.597 & $K2$ & >21.12 & K2 \\ 
8132.618 & $K2$ & >21.12 & K2 \\ 
8132.638 & $K2$ & >21.12 & K2 \\ 
8132.659 & $K2$ & >21.12 & K2 \\ 
8132.699 & $K2$ & >21.12 & K2 \\ 
8132.720 & $K2$ & >21.12 & K2 \\ 
8132.740 & $K2$ & >21.12 & K2 \\ 
8132.761 & $K2$ & >21.12 & K2 \\ 
8132.781 & $K2$ & >21.12 & K2 \\ 
8132.802 & $K2$ & >21.12 & K2 \\ 
8132.822 & $K2$ & >21.12 & K2 \\ 
8132.843 & $K2$ & >21.12 & K2 \\ 
8132.863 & $K2$ & >21.12 & K2 \\ 
8132.883 & $K2$ & >21.12 & K2 \\ 
8132.904 & $K2$ & >21.12 & K2 \\ 
8132.924 & $K2$ & >21.12 & K2 \\ 
8132.945 & $K2$ & >21.12 & K2 \\ 
8132.965 & $K2$ & >21.12 & K2 \\ 
8132.986 & $K2$ & >21.12 & K2 \\ 
8133.006 & $K2$ & >21.12 & K2 \\ 
8133.026 & $K2$ & >21.12 & K2 \\ 
8133.047 & $K2$ & >21.12 & K2 \\ 
8133.067 & $K2$ & >21.12 & K2 \\ 
8133.088 & $K2$ & >21.12 & K2 \\ 
8133.108 & $K2$ & >21.12 & K2 \\ 
8133.129 & $K2$ & >21.12 & K2 \\ 
8133.149 & $K2$ & >21.12 & K2 \\ 
8133.169 & $K2$ & >21.12 & K2 \\ 
8133.190 & $K2$ & >21.12 & K2 \\ 
8133.210 & $K2$ & >21.12 & K2 \\ 
8133.231 & $K2$ & >21.12 & K2 \\ 
8133.272 & $K2$ & >21.12 & K2 \\ 
8133.292 & $K2$ & >21.12 & K2 \\ 
8133.312 & $K2$ & >21.12 & K2 \\ 
8133.333 & $K2$ & >21.12 & K2 \\ 
8133.353 & $K2$ & >21.12 & K2 \\ 
8133.374 & $K2$ & >21.12 & K2 \\ 
8133.394 & $K2$ & >21.12 & K2 \\ 
8133.415 & $K2$ & >21.12 & K2 \\ 
8133.435 & $K2$ & >21.12 & K2 \\ 
8133.456 & $K2$ & >21.12 & K2 \\ 
8133.476 & $K2$ & >21.12 & K2 \\ 
8133.496 & $K2$ & >21.12 & K2 \\ 
8133.517 & $K2$ & >21.12 & K2 \\ 
8133.537 & $K2$ & >21.12 & K2 \\ 
8133.558 & $K2$ & >21.12 & K2 \\ 
8133.578 & $K2$ & >21.12 & K2 \\ 
8133.599 & $K2$ & >21.12 & K2 \\ 
8133.619 & $K2$ & >21.12 & K2 \\ 
8133.639 & $K2$ & >21.12 & K2 \\ 
8133.680 & $K2$ & >21.12 & K2 \\ 
8133.701 & $K2$ & >21.12 & K2 \\ 
8133.721 & $K2$ & >21.12 & K2 \\ 
8133.742 & $K2$ & >21.12 & K2 \\ 
8133.762 & $K2$ & >21.12 & K2 \\ 
8133.782 & $K2$ & >21.12 & K2 \\ 
8133.803 & $K2$ & >21.12 & K2 \\ 
8133.823 & $K2$ & >21.12 & K2 \\ 
8133.844 & $K2$ & >21.12 & K2 \\ 
8133.864 & $K2$ & >21.12 & K2 \\ 
8133.885 & $K2$ & >21.12 & K2 \\ 
8133.905 & $K2$ & >21.12 & K2 \\ 
8133.926 & $K2$ & >21.12 & K2 \\ 
8133.946 & $K2$ & >21.12 & K2 \\ 
8133.966 & $K2$ & >21.12 & K2 \\ 
8133.987 & $K2$ & >21.12 & K2 \\ 
8134.007 & $K2$ & >21.12 & K2 \\ 
8134.028 & $K2$ & >21.12 & K2 \\ 
8134.048 & $K2$ & >21.12 & K2 \\ 
8134.069 & $K2$ & >21.12 & K2 \\ 
8134.089 & $K2$ & >21.12 & K2 \\ 
8134.109 & $K2$ & >21.12 & K2 \\ 
8134.130 & $K2$ & >21.12 & K2 \\ 
8134.171 & $K2$ & >21.12 & K2 \\ 
8134.191 & $K2$ & >21.12 & K2 \\ 
8134.212 & $K2$ & >21.12 & K2 \\ 
8134.232 & $K2$ & >21.12 & K2 \\ 
8134.252 & $K2$ & >21.12 & K2 \\ 
8134.273 & $K2$ & >21.12 & K2 \\ 
8134.293 & $K2$ & >21.12 & K2 \\ 
8134.314 & $K2$ & >21.12 & K2 \\ 
8134.334 & $K2$ & >21.12 & K2 \\ 
8134.355 & $K2$ & >21.12 & K2 \\ 
8134.375 & $K2$ & >21.12 & K2 \\ 
8134.416 & $K2$ & >21.12 & K2 \\ 
8134.436 & $K2$ & >21.12 & K2 \\ 
8134.457 & $K2$ & >21.12 & K2 \\ 
8134.477 & $K2$ & >21.12 & K2 \\ 
8134.498 & $K2$ & >21.12 & K2 \\ 
8134.518 & $K2$ & >21.12 & K2 \\ 
8134.539 & $K2$ & >21.12 & K2 \\ 
8134.559 & $K2$ & >21.12 & K2 \\ 
8134.579 & $K2$ & >21.12 & K2 \\ 
8134.600 & $K2$ & >21.12 & K2 \\ 
8134.620 & $K2$ & >21.12 & K2 \\ 
8134.682 & $K2$ & >21.12 & K2 \\ 
8134.702 & $K2$ & >21.12 & K2 \\ 
8134.722 & $K2$ & >21.12 & K2 \\ 
8134.743 & $K2$ & >21.12 & K2 \\ 
8134.763 & $K2$ & >21.12 & K2 \\ 
8134.784 & $K2$ & >21.12 & K2 \\ 
8134.804 & $K2$ & >21.12 & K2 \\ 
8134.825 & $K2$ & >21.12 & K2 \\ 
8134.845 & $K2$ & >21.12 & K2 \\ 
8134.865 & $K2$ & >21.12 & K2 \\ 
8134.886 & $K2$ & >21.12 & K2 \\ 
8134.927 & $K2$ & >21.12 & K2 \\ 
8134.947 & $K2$ & >21.12 & K2 \\ 
8134.968 & $K2$ & >21.12 & K2 \\ 
8134.988 & $K2$ & >21.12 & K2 \\ 
8135.008 & $K2$ & >21.12 & K2 \\ 
8135.029 & $K2$ & >21.12 & K2 \\ 
8135.049 & $K2$ & >21.12 & K2 \\ 
8135.070 & $K2$ & >21.12 & K2 \\ 
8135.090 & $K2$ & >21.12 & K2 \\ 
8135.111 & $K2$ & >21.12 & K2 \\ 
8135.131 & $K2$ & >21.12 & K2 \\ 
8135.152 & $K2$ & >21.12 & K2 \\ 
8135.172 & $K2$ & >21.12 & K2 \\ 
8135.192 & $K2$ & >21.12 & K2 \\ 
8135.213 & $K2$ & >21.12 & K2 \\ 
8135.233 & $K2$ & >21.12 & K2 \\ 
8135.254 & $K2$ & >21.12 & K2 \\ 
8135.274 & $K2$ & >21.12 & K2 \\ 
8135.295 & $K2$ & >21.12 & K2 \\ 
8135.315 & $K2$ & >21.12 & K2 \\ 
8135.335 & $K2$ & >21.12 & K2 \\ 
8135.356 & $K2$ & >21.12 & K2 \\ 
8135.397 & $K2$ & >21.12 & K2 \\ 
8135.417 & $K2$ & >21.12 & K2 \\ 
8135.438 & $K2$ & >21.12 & K2 \\ 
8135.458 & $K2$ & >21.12 & K2 \\ 
8135.478 & $K2$ & >21.12 & K2 \\ 
8135.499 & $K2$ & >21.12 & K2 \\ 
8135.519 & $K2$ & >21.12 & K2 \\ 
8135.540 & $K2$ & >21.12 & K2 \\ 
8135.560 & $K2$ & >21.12 & K2 \\ 
8135.581 & $K2$ & >21.12 & K2 \\ 
8135.601 & $K2$ & >21.12 & K2 \\ 
8135.621 & $K2$ & >21.12 & K2 \\ 
8135.642 & $K2$ & >21.12 & K2 \\ 
8135.662 & $K2$ & >21.12 & K2 \\ 
8135.683 & $K2$ & >21.12 & K2 \\ 
8135.703 & $K2$ & >21.12 & K2 \\ 
8135.724 & $K2$ & >21.12 & K2 \\ 
8135.744 & $K2$ & >21.12 & K2 \\ 
8135.765 & $K2$ & >21.12 & K2 \\ 
8135.785 & $K2$ & >21.12 & K2 \\ 
8135.805 & $K2$ & >21.12 & K2 \\ 
8135.826 & $K2$ & >21.12 & K2 \\ 
8135.846 & $K2$ & >21.12 & K2 \\ 
8135.867 & $K2$ & >21.12 & K2 \\ 
8135.887 & $K2$ & >21.12 & K2 \\ 
8135.908 & $K2$ & >21.12 & K2 \\ 
8135.928 & $K2$ & >21.12 & K2 \\ 
8135.948 & $K2$ & >21.12 & K2 \\ 
8135.969 & $K2$ & >21.12 & K2 \\ 
8135.989 & $K2$ & >21.12 & K2 \\ 
8136.010 & $K2$ & >21.12 & K2 \\ 
8136.030 & $K2$ & >21.12 & K2 \\ 
8136.051 & $K2$ & >21.12 & K2 \\ 
8136.071 & $K2$ & >21.12 & K2 \\ 
8136.091 & $K2$ & >21.12 & K2 \\ 
8136.132 & $K2$ & >21.12 & K2 \\ 
8136.153 & $K2$ & >21.12 & K2 \\ 
8136.173 & $K2$ & >21.12 & K2 \\ 
8136.194 & $K2$ & >21.12 & K2 \\ 
8136.214 & $K2$ & >21.12 & K2 \\ 
8136.235 & $K2$ & >21.12 & K2 \\ 
8136.255 & $K2$ & >21.12 & K2 \\ 
8136.275 & $K2$ & >21.12 & K2 \\ 
8136.296 & $K2$ & >21.12 & K2 \\ 
8136.316 & $K2$ & >21.12 & K2 \\ 
8136.337 & $K2$ & >21.12 & K2 \\ 
8136.357 & $K2$ & >21.12 & K2 \\ 
8136.378 & $K2$ & >21.12 & K2 \\ 
8136.398 & $K2$ & >21.12 & K2 \\ 
8136.418 & $K2$ & >21.12 & K2 \\ 
8136.439 & $K2$ & >21.12 & K2 \\ 
8136.459 & $K2$ & >21.12 & K2 \\ 
8136.480 & $K2$ & >21.12 & K2 \\ 
8136.500 & $K2$ & >21.12 & K2 \\ 
8136.521 & $K2$ & >21.12 & K2 \\ 
8136.541 & $K2$ & >21.12 & K2 \\ 
8136.561 & $K2$ & >21.12 & K2 \\ 
8136.582 & $K2$ & >21.12 & K2 \\ 
8136.643 & $K2$ & >21.12 & K2 \\ 
8136.664 & $K2$ & >21.12 & K2 \\ 
8136.684 & $K2$ & >21.12 & K2 \\ 
8136.704 & $K2$ & >21.12 & K2 \\ 
8136.725 & $K2$ & >21.12 & K2 \\ 
8136.745 & $K2$ & >21.12 & K2 \\ 
8136.766 & $K2$ & >21.12 & K2 \\ 
8136.786 & $K2$ & >21.12 & K2 \\ 
8136.807 & $K2$ & >21.12 & K2 \\ 
8136.827 & $K2$ & >21.12 & K2 \\ 
8136.848 & $K2$ & >21.12 & K2 \\ 
8136.868 & $K2$ & >21.12 & K2 \\ 
8136.888 & $K2$ & >21.12 & K2 \\ 
8136.909 & $K2$ & >21.12 & K2 \\ 
8136.929 & $K2$ & >21.12 & K2 \\ 
8136.950 & $K2$ & >21.12 & K2 \\ 
8136.970 & $K2$ & >21.12 & K2 \\ 
8136.991 & $K2$ & >21.12 & K2 \\ 
8137.011 & $K2$ & >21.12 & K2 \\ 
8137.031 & $K2$ & >21.12 & K2 \\ 
8137.052 & $K2$ & >21.12 & K2 \\ 
8137.072 & $K2$ & >21.12 & K2 \\ 
8137.113 & $K2$ & >21.12 & K2 \\ 
8137.134 & $K2$ & >21.12 & K2 \\ 
8137.154 & $K2$ & >21.12 & K2 \\ 
8137.174 & $K2$ & >21.12 & K2 \\ 
8137.195 & $K2$ & >21.12 & K2 \\ 
8137.215 & $K2$ & >21.12 & K2 \\ 
8137.236 & $K2$ & >21.12 & K2 \\ 
8137.256 & $K2$ & >21.12 & K2 \\ 
8137.277 & $K2$ & >21.12 & K2 \\ 
8137.297 & $K2$ & >21.12 & K2 \\ 
8137.317 & $K2$ & >21.12 & K2 \\ 
8137.338 & $K2$ & >21.12 & K2 \\ 
8137.358 & $K2$ & >21.12 & K2 \\ 
8137.379 & $K2$ & >21.12 & K2 \\ 
8137.399 & $K2$ & >21.12 & K2 \\ 
8137.420 & $K2$ & >21.12 & K2 \\ 
8137.440 & $K2$ & >21.12 & K2 \\ 
8137.461 & $K2$ & >21.12 & K2 \\ 
8137.481 & $K2$ & >21.12 & K2 \\ 
8137.501 & $K2$ & >21.12 & K2 \\ 
8137.522 & $K2$ & >21.12 & K2 \\ 
8137.542 & $K2$ & >21.12 & K2 \\ 
8137.563 & $K2$ & >21.12 & K2 \\ 
8137.604 & $K2$ & >21.12 & K2 \\ 
8137.624 & $K2$ & >21.12 & K2 \\ 
8137.644 & $K2$ & >21.12 & K2 \\ 
8137.665 & $K2$ & >21.12 & K2 \\ 
8137.685 & $K2$ & >21.12 & K2 \\ 
8137.706 & $K2$ & >21.12 & K2 \\ 
8137.726 & $K2$ & >21.12 & K2 \\ 
8137.747 & $K2$ & >21.12 & K2 \\ 
8137.767 & $K2$ & >21.12 & K2 \\ 
8137.787 & $K2$ & >21.12 & K2 \\ 
8137.808 & $K2$ & >21.12 & K2 \\ 
8137.828 & $K2$ & >21.12 & K2 \\ 
8137.849 & $K2$ & >21.12 & K2 \\ 
8137.869 & $K2$ & >21.12 & K2 \\ 
8137.890 & $K2$ & >21.12 & K2 \\ 
8137.910 & $K2$ & >21.12 & K2 \\ 
8137.930 & $K2$ & >21.12 & K2 \\ 
8137.951 & $K2$ & >21.12 & K2 \\ 
8137.971 & $K2$ & >21.12 & K2 \\ 
8137.992 & $K2$ & >21.12 & K2 \\ 
8138.012 & $K2$ & >21.12 & K2 \\ 
8138.033 & $K2$ & >21.12 & K2 \\ 
8138.053 & $K2$ & >21.12 & K2 \\ 
8138.074 & $K2$ & >21.12 & K2 \\ 
8138.094 & $K2$ & >21.12 & K2 \\ 
8138.114 & $K2$ & >21.12 & K2 \\ 
8138.135 & $K2$ & >21.12 & K2 \\ 
8138.155 & $K2$ & >21.12 & K2 \\ 
8138.176 & $K2$ & >21.12 & K2 \\ 
8138.196 & $K2$ & >21.12 & K2 \\ 
8138.217 & $K2$ & >21.12 & K2 \\ 
8138.237 & $K2$ & >21.12 & K2 \\ 
8138.257 & $K2$ & >21.12 & K2 \\ 
8138.278 & $K2$ & >21.12 & K2 \\ 
8138.298 & $K2$ & >21.12 & K2 \\ 
8138.319 & $K2$ & >21.12 & K2 \\ 
8138.339 & $K2$ & >21.12 & K2 \\ 
8138.360 & $K2$ & >21.12 & K2 \\ 
8138.380 & $K2$ & >21.12 & K2 \\ 
8138.400 & $K2$ & >21.12 & K2 \\ 
8138.421 & $K2$ & >21.12 & K2 \\ 
8138.441 & $K2$ & >21.12 & K2 \\ 
8138.462 & $K2$ & >21.12 & K2 \\ 
8138.482 & $K2$ & >21.12 & K2 \\ 
8138.503 & $K2$ & >21.12 & K2 \\ 
8138.523 & $K2$ & >21.12 & K2 \\ 
8138.544 & $K2$ & >21.12 & K2 \\ 
8138.584 & $K2$ & >21.12 & K2 \\ 
8138.605 & $K2$ & >21.12 & K2 \\ 
8138.625 & $K2$ & >21.12 & K2 \\ 
8138.646 & $K2$ & >21.12 & K2 \\ 
8138.666 & $K2$ & >21.12 & K2 \\ 
8138.687 & $K2$ & >21.12 & K2 \\ 
8138.707 & $K2$ & >21.12 & K2 \\ 
8138.727 & $K2$ & >21.12 & K2 \\ 
8138.748 & $K2$ & >21.12 & K2 \\ 
8138.768 & $K2$ & >21.12 & K2 \\ 
8138.789 & $K2$ & >21.12 & K2 \\ 
8138.809 & $K2$ & >21.12 & K2 \\ 
8138.830 & $K2$ & >21.12 & K2 \\ 
8138.850 & $K2$ & >21.12 & K2 \\ 
8138.870 & $K2$ & >21.12 & K2 \\ 
8138.891 & $K2$ & >21.12 & K2 \\ 
8138.911 & $K2$ & >21.12 & K2 \\ 
8138.932 & $K2$ & >21.12 & K2 \\ 
8138.952 & $K2$ & >21.12 & K2 \\ 
8138.973 & $K2$ & >21.12 & K2 \\ 
8138.993 & $K2$ & >21.12 & K2 \\ 
8139.013 & $K2$ & >21.12 & K2 \\ 
8139.034 & $K2$ & >21.12 & K2 \\ 
8139.054 & $K2$ & >21.12 & K2 \\ 
8139.075 & $K2$ & >21.12 & K2 \\ 
8139.095 & $K2$ & >21.12 & K2 \\ 
8139.116 & $K2$ & >21.12 & K2 \\ 
8139.136 & $K2$ & >21.12 & K2 \\ 
8139.157 & $K2$ & >21.12 & K2 \\ 
8139.177 & $K2$ & >21.12 & K2 \\ 
8139.197 & $K2$ & >21.12 & K2 \\ 
8139.218 & $K2$ & >21.12 & K2 \\ 
8139.238 & $K2$ & >21.12 & K2 \\ 
8139.259 & $K2$ & >21.12 & K2 \\ 
8139.279 & $K2$ & >21.12 & K2 \\ 
8139.300 & $K2$ & >21.12 & K2 \\ 
8139.320 & $K2$ & >21.12 & K2 \\ 
8139.340 & $K2$ & >21.12 & K2 \\ 
8139.361 & $K2$ & >21.12 & K2 \\ 
8139.381 & $K2$ & >21.12 & K2 \\ 
8139.402 & $K2$ & >21.12 & K2 \\ 
8139.422 & $K2$ & >21.12 & K2 \\ 
8139.443 & $K2$ & >21.12 & K2 \\ 
8139.463 & $K2$ & >21.12 & K2 \\ 
8139.483 & $K2$ & >21.12 & K2 \\ 
8139.504 & $K2$ & >21.12 & K2 \\ 
8139.524 & $K2$ & >21.12 & K2 \\ 
8139.565 & $K2$ & >21.12 & K2 \\ 
8139.586 & $K2$ & >21.12 & K2 \\ 
8139.606 & $K2$ & >21.12 & K2 \\ 
8139.626 & $K2$ & >21.12 & K2 \\ 
8139.647 & $K2$ & >21.12 & K2 \\ 
8139.667 & $K2$ & >21.12 & K2 \\ 
8139.688 & $K2$ & >21.12 & K2 \\ 
8139.708 & $K2$ & >21.12 & K2 \\ 
8139.729 & $K2$ & >21.12 & K2 \\ 
8139.749 & $K2$ & >21.12 & K2 \\ 
8139.770 & $K2$ & >21.12 & K2 \\ 
8139.790 & $K2$ & >21.12 & K2 \\ 
8139.810 & $K2$ & >21.12 & K2 \\ 
8139.831 & $K2$ & >21.12 & K2 \\ 
8139.851 & $K2$ & >21.12 & K2 \\ 
8139.872 & $K2$ & >21.12 & K2 \\ 
8139.892 & $K2$ & >21.12 & K2 \\ 
8139.913 & $K2$ & >21.12 & K2 \\ 
8139.933 & $K2$ & >21.12 & K2 \\ 
8139.953 & $K2$ & >21.12 & K2 \\ 
8139.974 & $K2$ & >21.12 & K2 \\ 
8139.994 & $K2$ & >21.12 & K2 \\ 
8140.015 & $K2$ & >21.12 & K2 \\ 
8140.056 & $K2$ & >21.12 & K2 \\ 
8140.076 & $K2$ & >21.12 & K2 \\ 
8140.117 & $K2$ & >21.12 & K2 \\ 
8140.137 & $K2$ & >21.12 & K2 \\ 
8140.158 & $K2$ & >21.12 & K2 \\ 
8140.178 & $K2$ & >21.12 & K2 \\ 
8140.199 & $K2$ & >21.12 & K2 \\ 
8140.219 & $K2$ & >21.12 & K2 \\ 
8140.239 & $K2$ & >21.12 & K2 \\ 
8140.260 & $K2$ & >21.12 & K2 \\ 
8140.301 & $K2$ & >21.12 & K2 \\ 
8140.321 & $K2$ & >21.12 & K2 \\ 
8140.342 & $K2$ & >21.12 & K2 \\ 
8140.362 & $K2$ & >21.12 & K2 \\ 
8140.383 & $K2$ & >21.12 & K2 \\ 
8140.403 & $K2$ & >21.12 & K2 \\ 
8140.423 & $K2$ & >21.12 & K2 \\ 
8140.444 & $K2$ & >21.12 & K2 \\ 
8140.464 & $K2$ & >21.12 & K2 \\ 
8140.505 & $K2$ & >21.12 & K2 \\ 
8140.566 & $K2$ & >21.12 & K2 \\ 
8140.587 & $K2$ & >21.12 & K2 \\ 
8140.607 & $K2$ & >21.12 & K2 \\ 
8140.628 & $K2$ & >21.12 & K2 \\ 
8140.648 & $K2$ & >21.12 & K2 \\ 
8140.669 & $K2$ & >21.12 & K2 \\ 
8140.689 & $K2$ & >21.12 & K2 \\ 
8140.709 & $K2$ & >21.12 & K2 \\ 
8140.730 & $K2$ & >21.12 & K2 \\ 
8140.750 & $K2$ & >21.12 & K2 \\ 
8140.771 & $K2$ & >21.12 & K2 \\ 
8140.791 & $K2$ & >21.12 & K2 \\ 
8140.812 & $K2$ & >21.12 & K2 \\ 
8140.832 & $K2$ & >21.12 & K2 \\ 
8140.852 & $K2$ & >21.12 & K2 \\ 
8140.873 & $K2$ & >21.12 & K2 \\ 
8140.893 & $K2$ & >21.12 & K2 \\ 
8140.914 & $K2$ & >21.12 & K2 \\ 
8140.934 & $K2$ & >21.12 & K2 \\ 
8140.955 & $K2$ & >21.12 & K2 \\ 
8140.975 & $K2$ & >21.12 & K2 \\ 
8140.996 & $K2$ & >21.12 & K2 \\ 
8141.016 & $K2$ & >21.12 & K2 \\ 
8141.036 & $K2$ & >21.12 & K2 \\ 
8141.057 & $K2$ & >21.12 & K2 \\ 
8141.077 & $K2$ & >21.12 & K2 \\ 
8141.098 & $K2$ & >21.12 & K2 \\ 
8141.118 & $K2$ & >21.12 & K2 \\ 
8141.139 & $K2$ & >21.12 & K2 \\ 
8141.159 & $K2$ & >21.12 & K2 \\ 
8141.179 & $K2$ & >21.12 & K2 \\ 
8141.200 & $K2$ & >21.12 & K2 \\ 
8141.220 & $K2$ & >21.12 & K2 \\ 
8141.241 & $K2$ & >21.12 & K2 \\ 
8141.282 & $K2$ & >21.12 & K2 \\ 
8141.302 & $K2$ & >21.12 & K2 \\ 
8141.322 & $K2$ & >21.12 & K2 \\ 
8141.343 & $K2$ & >21.12 & K2 \\ 
8141.363 & $K2$ & >21.12 & K2 \\ 
8141.384 & $K2$ & >21.12 & K2 \\ 
8141.404 & $K2$ & >21.12 & K2 \\ 
8141.425 & $K2$ & >21.12 & K2 \\ 
8141.445 & $K2$ & >21.12 & K2 \\ 
8141.466 & $K2$ & >21.12 & K2 \\ 
8141.486 & $K2$ & >21.12 & K2 \\ 
8141.506 & $K2$ & >21.12 & K2 \\ 
8141.527 & $K2$ & >21.12 & K2 \\ 
8141.547 & $K2$ & >21.12 & K2 \\ 
8141.568 & $K2$ & >21.12 & K2 \\ 
8141.588 & $K2$ & >21.12 & K2 \\ 
8141.609 & $K2$ & >21.12 & K2 \\ 
8141.629 & $K2$ & >21.12 & K2 \\ 
8141.649 & $K2$ & >21.12 & K2 \\ 
8141.670 & $K2$ & >21.12 & K2 \\ 
8141.690 & $K2$ & >21.12 & K2 \\ 
8141.711 & $K2$ & >21.12 & K2 \\ 
8141.731 & $K2$ & >21.12 & K2 \\ 
8141.772 & $K2$ & >21.12 & K2 \\ 
8141.792 & $K2$ & >21.12 & K2 \\ 
8141.813 & $K2$ & >21.12 & K2 \\ 
8141.833 & $K2$ & >21.12 & K2 \\ 
8141.854 & $K2$ & >21.12 & K2 \\ 
8141.895 & $K2$ & >21.12 & K2 \\ 
8141.915 & $K2$ & >21.12 & K2 \\ 
8141.935 & $K2$ & >21.12 & K2 \\ 
8141.956 & $K2$ & >21.12 & K2 \\ 
8141.976 & $K2$ & >21.12 & K2 \\ 
8142.017 & $K2$ & >21.12 & K2 \\ 
8142.038 & $K2$ & >21.12 & K2 \\ 
8142.058 & $K2$ & >21.12 & K2 \\ 
8142.079 & $K2$ & >21.12 & K2 \\ 
8142.099 & $K2$ & >21.12 & K2 \\ 
8142.119 & $K2$ & >21.12 & K2 \\ 
8142.140 & $K2$ & >21.12 & K2 \\ 
8142.160 & $K2$ & >21.12 & K2 \\ 
8142.181 & $K2$ & >21.12 & K2 \\ 
8142.201 & $K2$ & >21.12 & K2 \\ 
8142.222 & $K2$ & >21.12 & K2 \\ 
8142.242 & $K2$ & >21.12 & K2 \\ 
8142.262 & $K2$ & >21.12 & K2 \\ 
8142.283 & $K2$ & >21.12 & K2 \\ 
8142.303 & $K2$ & >21.12 & K2 \\ 
8142.324 & $K2$ & >21.12 & K2 \\ 
8142.344 & $K2$ & >21.12 & K2 \\ 
8142.365 & $K2$ & >21.12 & K2 \\ 
8142.385 & $K2$ & >21.12 & K2 \\ 
8142.405 & $K2$ & >21.12 & K2 \\ 
8142.426 & $K2$ & >21.12 & K2 \\ 
8142.446 & $K2$ & >21.12 & K2 \\ 
8142.467 & $K2$ & >21.12 & K2 \\ 
8142.508 & $K2$ & >21.12 & K2 \\ 
8142.528 & $K2$ & >21.12 & K2 \\ 
8142.548 & $K2$ & >21.12 & K2 \\ 
8142.569 & $K2$ & >21.12 & K2 \\ 
8142.589 & $K2$ & >21.12 & K2 \\ 
8142.610 & $K2$ & >21.12 & K2 \\ 
8142.630 & $K2$ & >21.12 & K2 \\ 
8142.651 & $K2$ & >21.12 & K2 \\ 
8142.671 & $K2$ & >21.12 & K2 \\ 
8142.692 & $K2$ & >21.12 & K2 \\ 
8142.712 & $K2$ & >21.12 & K2 \\ 
8142.732 & $K2$ & >21.12 & K2 \\ 
8142.753 & $K2$ & >21.12 & K2 \\ 
8142.773 & $K2$ & >21.12 & K2 \\ 
8142.794 & $K2$ & >21.12 & K2 \\ 
8142.814 & $K2$ & >21.12 & K2 \\ 
8142.835 & $K2$ & >21.12 & K2 \\ 
8142.855 & $K2$ & >21.12 & K2 \\ 
8142.875 & $K2$ & >21.12 & K2 \\ 
8142.896 & $K2$ & >21.12 & K2 \\ 
8142.916 & $K2$ & >21.12 & K2 \\ 
8142.937 & $K2$ & >21.12 & K2 \\ 
8142.957 & $K2$ & >21.12 & K2 \\ 
8142.978 & $K2$ & >21.12 & K2 \\ 
8142.998 & $K2$ & >21.12 & K2 \\ 
8143.018 & $K2$ & >21.12 & K2 \\ 
8143.039 & $K2$ & >21.12 & K2 \\ 
8143.059 & $K2$ & >21.12 & K2 \\ 
8143.080 & $K2$ & >21.12 & K2 \\ 
8143.100 & $K2$ & >21.12 & K2 \\ 
8143.121 & $K2$ & >21.12 & K2 \\ 
8143.141 & $K2$ & >21.12 & K2 \\ 
8143.161 & $K2$ & >21.12 & K2 \\ 
8143.182 & $K2$ & >21.12 & K2 \\ 
8143.202 & $K2$ & >21.12 & K2 \\ 
8143.243 & $K2$ & >21.12 & K2 \\ 
8143.264 & $K2$ & >21.12 & K2 \\ 
8143.284 & $K2$ & >21.12 & K2 \\ 
8143.305 & $K2$ & >21.12 & K2 \\ 
8143.325 & $K2$ & >21.12 & K2 \\ 
8143.345 & $K2$ & >21.12 & K2 \\ 
8143.366 & $K2$ & >21.12 & K2 \\ 
8143.386 & $K2$ & >21.12 & K2 \\ 
8143.407 & $K2$ & >21.12 & K2 \\ 
8143.427 & $K2$ & >21.12 & K2 \\ 
8143.448 & $K2$ & >21.12 & K2 \\ 
8143.468 & $K2$ & >21.12 & K2 \\ 
8143.488 & $K2$ & >21.12 & K2 \\ 
8143.509 & $K2$ & >21.12 & K2 \\ 
8143.529 & $K2$ & >21.12 & K2 \\ 
8143.550 & $K2$ & >21.12 & K2 \\ 
8143.570 & $K2$ & >21.12 & K2 \\ 
8143.591 & $K2$ & >21.12 & K2 \\ 
8143.611 & $K2$ & >21.12 & K2 \\ 
8143.631 & $K2$ & >21.12 & K2 \\ 
8143.652 & $K2$ & >21.12 & K2 \\ 
8143.672 & $K2$ & >21.12 & K2 \\ 
8143.693 & $K2$ & >21.12 & K2 \\ 
8143.713 & $K2$ & >21.12 & K2 \\ 
8143.734 & $K2$ & >21.12 & K2 \\ 
8143.754 & $K2$ & >21.12 & K2 \\ 
8143.775 & $K2$ & >21.12 & K2 \\ 
8143.795 & $K2$ & >21.12 & K2 \\ 
8143.815 & $K2$ & >21.12 & K2 \\ 
8143.836 & $K2$ & >21.12 & K2 \\ 
8143.856 & $K2$ & >21.12 & K2 \\ 
8143.877 & $K2$ & >21.12 & K2 \\ 
8143.897 & $K2$ & >21.12 & K2 \\ 
8143.918 & $K2$ & >21.12 & K2 \\ 
8143.938 & $K2$ & >21.12 & K2 \\ 
8143.958 & $K2$ & >21.12 & K2 \\ 
8143.979 & $K2$ & >21.12 & K2 \\ 
8143.999 & $K2$ & >21.12 & K2 \\ 
8144.020 & $K2$ & >21.12 & K2 \\ 
8144.040 & $K2$ & >21.12 & K2 \\ 
8144.061 & $K2$ & >21.12 & K2 \\ 
8144.081 & $K2$ & >21.12 & K2 \\ 
8144.101 & $K2$ & >21.12 & K2 \\ 
8144.122 & $K2$ & >21.12 & K2 \\ 
8144.142 & $K2$ & >21.12 & K2 \\ 
8144.163 & $K2$ & >21.12 & K2 \\ 
8144.224 & $K2$ & >21.12 & K2 \\ 
8144.244 & $K2$ & >21.12 & K2 \\ 
8144.265 & $K2$ & >21.12 & K2 \\ 
8144.285 & $K2$ & >21.12 & K2 \\ 
8144.306 & $K2$ & >21.12 & K2 \\ 
8144.326 & $K2$ & >21.12 & K2 \\ 
8144.347 & $K2$ & >21.12 & K2 \\ 
8144.367 & $K2$ & >21.12 & K2 \\ 
8144.388 & $K2$ & >21.12 & K2 \\ 
8144.408 & $K2$ & >21.12 & K2 \\ 
8144.428 & $K2$ & >21.12 & K2 \\ 
8144.469 & $K2$ & >21.12 & K2 \\ 
8144.490 & $K2$ & >21.12 & K2 \\ 
8144.510 & $K2$ & >21.12 & K2 \\ 
8144.531 & $K2$ & >21.12 & K2 \\ 
8144.551 & $K2$ & >21.12 & K2 \\ 
8144.571 & $K2$ & >21.12 & K2 \\ 
8144.592 & $K2$ & >21.12 & K2 \\ 
8144.612 & $K2$ & >21.12 & K2 \\ 
8144.633 & $K2$ & >21.12 & K2 \\ 
8144.674 & $K2$ & >21.12 & K2 \\ 
8144.714 & $K2$ & >21.12 & K2 \\ 
8144.735 & $K2$ & >21.12 & K2 \\ 
8144.755 & $K2$ & >21.12 & K2 \\ 
8144.776 & $K2$ & >21.12 & K2 \\ 
8144.796 & $K2$ & >21.12 & K2 \\ 
8144.817 & $K2$ & >21.12 & K2 \\ 
8144.837 & $K2$ & >21.12 & K2 \\ 
8144.857 & $K2$ & >21.12 & K2 \\ 
8144.878 & $K2$ & >21.12 & K2 \\ 
8144.898 & $K2$ & >21.12 & K2 \\ 
8144.919 & $K2$ & >21.12 & K2 \\ 
8144.960 & $K2$ & >21.12 & K2 \\ 
8144.980 & $K2$ & >21.12 & K2 \\ 
8145.001 & $K2$ & >21.12 & K2 \\ 
8145.021 & $K2$ & >21.12 & K2 \\ 
8145.041 & $K2$ & >21.12 & K2 \\ 
8145.062 & $K2$ & >21.12 & K2 \\ 
8145.082 & $K2$ & >21.12 & K2 \\ 
8145.103 & $K2$ & 20.620(0.229) & K2 \\ 
8145.123 & $K2$ & 20.942(0.307) & K2 \\ 
8145.144 & $K2$ & 20.516(0.208) & K2 \\ 
8145.164 & $K2$ & 20.350(0.178) & K2 \\ 
8145.184 & $K2$ & 20.732(0.253) & K2 \\ 
8145.205 & $K2$ & 20.189(0.154) & K2 \\ 
8145.225 & $K2$ & 20.220(0.158) & K2 \\ 
8145.246 & $K2$ & 20.236(0.161) & K2 \\ 
8145.266 & $K2$ & 20.033(0.133) & K2 \\ 
8145.287 & $K2$ & 19.821(0.110) & K2 \\ 
8145.307 & $K2$ & 19.975(0.126) & K2 \\ 
8145.327 & $K2$ & 19.820(0.109) & K2 \\ 
8145.348 & $K2$ & 19.661(0.095) & K2 \\ 
8145.368 & $K2$ & 19.567(0.087) & K2 \\ 
8145.389 & $K2$ & 19.506(0.082) & K2 \\ 
8145.409 & $K2$ & 19.391(0.074) & K2 \\ 
8145.450 & $K2$ & 19.366(0.072) & K2 \\ 
8145.470 & $K2$ & 19.280(0.067) & K2 \\ 
8145.491 & $K2$ & 19.325(0.069) & K2 \\ 
8145.511 & $K2$ & 19.176(0.060) & K2 \\ 
8145.532 & $K2$ & 19.193(0.061) & K2 \\ 
8145.552 & $K2$ & 19.195(0.062) & K2 \\ 
8145.573 & $K2$ & 19.130(0.058) & K2 \\ 
8145.593 & $K2$ & 19.048(0.054) & K2 \\ 
8145.614 & $K2$ & 19.097(0.056) & K2 \\ 
8145.634 & $K2$ & 19.074(0.055) & K2 \\ 
8145.654 & $K2$ & 19.010(0.052) & K2 \\ 
8145.675 & $K2$ & 18.898(0.047) & K2 \\ 
8145.695 & $K2$ & 18.878(0.046) & K2 \\ 
8145.716 & $K2$ & 18.791(0.042) & K2 \\ 
8145.736 & $K2$ & 18.825(0.044) & K2 \\ 
8145.757 & $K2$ & 18.736(0.040) & K2 \\ 
8145.777 & $K2$ & 18.642(0.037) & K2 \\ 
8145.797 & $K2$ & 18.644(0.037) & K2 \\ 
8145.818 & $K2$ & 18.638(0.037) & K2 \\ 
8145.838 & $K2$ & 18.669(0.038) & K2 \\ 
8145.859 & $K2$ & 18.651(0.037) & K2 \\ 
8145.879 & $K2$ & 18.618(0.036) & K2 \\ 
8145.900 & $K2$ & 18.611(0.036) & K2 \\ 
8145.920 & $K2$ & 18.592(0.035) & K2 \\ 
8145.940 & $K2$ & 18.402(0.030) & K2 \\ 
8145.961 & $K2$ & 18.328(0.028) & K2 \\ 
8145.981 & $K2$ & 18.344(0.028) & K2 \\ 
8146.002 & $K2$ & 18.369(0.029) & K2 \\ 
8146.022 & $K2$ & 18.335(0.028) & K2 \\ 
8146.043 & $K2$ & 18.304(0.027) & K2 \\ 
8146.063 & $K2$ & 18.220(0.025) & K2 \\ 
8146.083 & $K2$ & 18.217(0.025) & K2 \\ 
8146.104 & $K2$ & 18.197(0.025) & K2 \\ 
8146.124 & $K2$ & 18.135(0.023) & K2 \\ 
8146.145 & $K2$ & 18.098(0.022) & K2 \\ 
8146.186 & $K2$ & 18.056(0.022) & K2 \\ 
8146.206 & $K2$ & 18.052(0.021) & K2 \\ 
8146.227 & $K2$ & 18.030(0.021) & K2 \\ 
8146.247 & $K2$ & 18.028(0.021) & K2 \\ 
8146.267 & $K2$ & 18.060(0.022) & K2 \\ 
8146.288 & $K2$ & 18.031(0.021) & K2 \\ 
8146.308 & $K2$ & 18.041(0.021) & K2 \\ 
8146.329 & $K2$ & 18.003(0.021) & K2 \\ 
8146.349 & $K2$ & 18.001(0.020) & K2 \\ 
8146.370 & $K2$ & 17.975(0.020) & K2 \\ 
8146.390 & $K2$ & 17.943(0.019) & K2 \\ 
8146.431 & $K2$ & 17.936(0.019) & K2 \\ 
8146.451 & $K2$ & 17.892(0.019) & K2 \\ 
8146.472 & $K2$ & 17.908(0.019) & K2 \\ 
8146.492 & $K2$ & 17.865(0.018) & K2 \\ 
8146.513 & $K2$ & 17.850(0.018) & K2 \\ 
8146.533 & $K2$ & 17.800(0.017) & K2 \\ 
8146.553 & $K2$ & 17.794(0.017) & K2 \\ 
8146.574 & $K2$ & 17.775(0.017) & K2 \\ 
8146.594 & $K2$ & 17.764(0.016) & K2 \\ 
8146.615 & $K2$ & 17.735(0.016) & K2 \\ 
8146.635 & $K2$ & 17.719(0.016) & K2 \\ 
8146.656 & $K2$ & 17.714(0.016) & K2 \\ 
8146.676 & $K2$ & 17.726(0.016) & K2 \\ 
8146.697 & $K2$ & 17.708(0.016) & K2 \\ 
8146.717 & $K2$ & 17.700(0.016) & K2 \\ 
8146.737 & $K2$ & 17.695(0.015) & K2 \\ 
8146.758 & $K2$ & 17.680(0.015) & K2 \\ 
8146.778 & $K2$ & 17.683(0.015) & K2 \\ 
8146.799 & $K2$ & 17.638(0.015) & K2 \\ 
8146.819 & $K2$ & 17.628(0.015) & K2 \\ 
8146.840 & $K2$ & 17.609(0.014) & K2 \\ 
8146.860 & $K2$ & 17.613(0.014) & K2 \\ 
8146.880 & $K2$ & 17.584(0.014) & K2 \\ 
8146.921 & $K2$ & 17.563(0.014) & K2 \\ 
8146.942 & $K2$ & 17.563(0.014) & K2 \\ 
8146.983 & $K2$ & 17.570(0.014) & K2 \\ 
8147.003 & $K2$ & 17.546(0.013) & K2 \\ 
8147.023 & $K2$ & 17.544(0.013) & K2 \\ 
8147.044 & $K2$ & 17.558(0.014) & K2 \\ 
8147.064 & $K2$ & 17.534(0.013) & K2 \\ 
8147.085 & $K2$ & 17.509(0.013) & K2 \\ 
8147.105 & $K2$ & 17.508(0.013) & K2 \\ 
8147.126 & $K2$ & 17.545(0.013) & K2 \\ 
8147.166 & $K2$ & 17.508(0.013) & K2 \\ 
8147.187 & $K2$ & 17.438(0.012) & K2 \\ 
8147.207 & $K2$ & 17.410(0.012) & K2 \\ 
8147.228 & $K2$ & 17.439(0.012) & K2 \\ 
8147.248 & $K2$ & 17.437(0.012) & K2 \\ 
8147.289 & $K2$ & 17.422(0.012) & K2 \\ 
8147.310 & $K2$ & 17.441(0.012) & K2 \\ 
8147.330 & $K2$ & 17.416(0.012) & K2 \\ 
8147.350 & $K2$ & 17.395(0.012) & K2 \\ 
8147.412 & $K2$ & 17.370(0.011) & K2 \\ 
8147.432 & $K2$ & 17.377(0.012) & K2 \\ 
8147.453 & $K2$ & 17.355(0.011) & K2 \\ 
8147.473 & $K2$ & 17.347(0.011) & K2 \\ 
8147.493 & $K2$ & 17.341(0.011) & K2 \\ 
8147.514 & $K2$ & 17.324(0.011) & K2 \\ 
8147.534 & $K2$ & 17.305(0.011) & K2 \\ 
8147.555 & $K2$ & 17.289(0.011) & K2 \\ 
8147.575 & $K2$ & 17.290(0.011) & K2 \\ 
8147.596 & $K2$ & 17.279(0.011) & K2 \\ 
8147.616 & $K2$ & 17.300(0.011) & K2 \\ 
8147.636 & $K2$ & 17.264(0.010) & K2 \\ 
8147.657 & $K2$ & 17.266(0.010) & K2 \\ 
8147.677 & $K2$ & 17.274(0.010) & K2 \\ 
8147.698 & $K2$ & 17.266(0.010) & K2 \\ 
8147.718 & $K2$ & 17.261(0.010) & K2 \\ 
8147.739 & $K2$ & 17.247(0.010) & K2 \\ 
8147.759 & $K2$ & 17.235(0.010) & K2 \\ 
8147.779 & $K2$ & 17.218(0.010) & K2 \\ 
8147.800 & $K2$ & 17.203(0.010) & K2 \\ 
8147.820 & $K2$ & 17.199(0.010) & K2 \\ 
8147.841 & $K2$ & 17.181(0.010) & K2 \\ 
8147.861 & $K2$ & 17.200(0.010) & K2 \\ 
8147.902 & $K2$ & 17.166(0.009) & K2 \\ 
8147.923 & $K2$ & 17.143(0.009) & K2 \\ 
8147.943 & $K2$ & 17.148(0.009) & K2 \\ 
8147.963 & $K2$ & 17.140(0.009) & K2 \\ 
8147.984 & $K2$ & 17.141(0.009) & K2 \\ 
8148.004 & $K2$ & 17.116(0.009) & K2 \\ 
8148.025 & $K2$ & 17.106(0.009) & K2 \\ 
8148.045 & $K2$ & 17.110(0.009) & K2 \\ 
8148.066 & $K2$ & 17.101(0.009) & K2 \\ 
8148.086 & $K2$ & 17.106(0.009) & K2 \\ 
8148.106 & $K2$ & 17.074(0.009) & K2 \\ 
8148.127 & $K2$ & 17.085(0.009) & K2 \\ 
8148.147 & $K2$ & 17.054(0.009) & K2 \\ 
8148.168 & $K2$ & 17.059(0.009) & K2 \\ 
8148.188 & $K2$ & 17.046(0.009) & K2 \\ 
8148.209 & $K2$ & 17.036(0.008) & K2 \\ 
8148.229 & $K2$ & 17.031(0.008) & K2 \\ 
8148.249 & $K2$ & 17.012(0.008) & K2 \\ 
8148.270 & $K2$ & 17.006(0.008) & K2 \\ 
8148.290 & $K2$ & 16.998(0.008) & K2 \\ 
8148.311 & $K2$ & 16.990(0.008) & K2 \\ 
8148.331 & $K2$ & 16.972(0.008) & K2 \\ 
8148.352 & $K2$ & 16.976(0.008) & K2 \\ 
8148.413 & $K2$ & 16.977(0.008) & K2 \\ 
8148.433 & $K2$ & 16.956(0.008) & K2 \\ 
8148.454 & $K2$ & 16.948(0.008) & K2 \\ 
8148.474 & $K2$ & 16.945(0.008) & K2 \\ 
8148.495 & $K2$ & 16.947(0.008) & K2 \\ 
8148.515 & $K2$ & 16.925(0.008) & K2 \\ 
8148.536 & $K2$ & 16.929(0.008) & K2 \\ 
8148.556 & $K2$ & 16.907(0.007) & K2 \\ 
8148.576 & $K2$ & 16.905(0.007) & K2 \\ 
8148.597 & $K2$ & 16.897(0.007) & K2 \\ 
8148.617 & $K2$ & 16.886(0.007) & K2 \\ 
8148.638 & $K2$ & 16.881(0.007) & K2 \\ 
8148.658 & $K2$ & 16.867(0.007) & K2 \\ 
8148.679 & $K2$ & 16.855(0.007) & K2 \\ 
8148.699 & $K2$ & 16.849(0.007) & K2 \\ 
8148.719 & $K2$ & 16.841(0.007) & K2 \\ 
8148.740 & $K2$ & 16.826(0.007) & K2 \\ 
8148.760 & $K2$ & 16.822(0.007) & K2 \\ 
8148.781 & $K2$ & 16.805(0.007) & K2 \\ 
8148.801 & $K2$ & 16.802(0.007) & K2 \\ 
8148.822 & $K2$ & 16.806(0.007) & K2 \\ 
8148.842 & $K2$ & 16.803(0.007) & K2 \\ 
8148.883 & $K2$ & 16.786(0.007) & K2 \\ 
8148.965 & $K2$ & 16.754(0.006) & K2 \\ 
8148.985 & $K2$ & 16.744(0.006) & K2 \\ 
8149.006 & $K2$ & 16.733(0.006) & K2 \\ 
8149.026 & $K2$ & 16.729(0.006) & K2 \\ 
8149.046 & $K2$ & 16.733(0.006) & K2 \\ 
8149.087 & $K2$ & 16.705(0.006) & K2 \\ 
8149.128 & $K2$ & 16.693(0.006) & K2 \\ 
8149.149 & $K2$ & 16.679(0.006) & K2 \\ 
8149.169 & $K2$ & 16.672(0.006) & K2 \\ 
8149.189 & $K2$ & 16.665(0.006) & K2 \\ 
8149.210 & $K2$ & 16.647(0.006) & K2 \\ 
8149.230 & $K2$ & 16.649(0.006) & K2 \\ 
8149.251 & $K2$ & 16.658(0.006) & K2 \\ 
8149.271 & $K2$ & 16.639(0.006) & K2 \\ 
8149.292 & $K2$ & 16.634(0.006) & K2 \\ 
8149.312 & $K2$ & 16.617(0.006) & K2 \\ 
8149.332 & $K2$ & 16.617(0.006) & K2 \\ 
8149.373 & $K2$ & 16.600(0.006) & K2 \\ 
8149.394 & $K2$ & 16.598(0.006) & K2 \\ 
8149.414 & $K2$ & 16.581(0.006) & K2 \\ 
8149.435 & $K2$ & 16.572(0.005) & K2 \\ 
8149.455 & $K2$ & 16.566(0.005) & K2 \\ 
8149.475 & $K2$ & 16.561(0.005) & K2 \\ 
8149.496 & $K2$ & 16.545(0.005) & K2 \\ 
8149.516 & $K2$ & 16.537(0.005) & K2 \\ 
8149.537 & $K2$ & 16.521(0.005) & K2 \\ 
8149.557 & $K2$ & 16.521(0.005) & K2 \\ 
8149.578 & $K2$ & 16.518(0.005) & K2 \\ 
8149.598 & $K2$ & 16.518(0.005) & K2 \\ 
8149.619 & $K2$ & 16.503(0.005) & K2 \\ 
8149.639 & $K2$ & 16.494(0.005) & K2 \\ 
8149.659 & $K2$ & 16.489(0.005) & K2 \\ 
8149.680 & $K2$ & 16.467(0.005) & K2 \\ 
8149.700 & $K2$ & 16.459(0.005) & K2 \\ 
8149.721 & $K2$ & 16.438(0.005) & K2 \\ 
8149.741 & $K2$ & 16.450(0.005) & K2 \\ 
8149.762 & $K2$ & 16.448(0.005) & K2 \\ 
8149.782 & $K2$ & 16.443(0.005) & K2 \\ 
8149.802 & $K2$ & 16.435(0.005) & K2 \\ 
8149.823 & $K2$ & 16.432(0.005) & K2 \\ 
8149.864 & $K2$ & 16.409(0.005) & K2 \\ 
8149.884 & $K2$ & 16.398(0.005) & K2 \\ 
8149.905 & $K2$ & 16.390(0.005) & K2 \\ 
8149.925 & $K2$ & 16.383(0.005) & K2 \\ 
8149.945 & $K2$ & 16.381(0.005) & K2 \\ 
8149.966 & $K2$ & 16.369(0.005) & K2 \\ 
8149.986 & $K2$ & 16.364(0.005) & K2 \\ 
8150.007 & $K2$ & 16.354(0.004) & K2 \\ 
8150.027 & $K2$ & 16.347(0.004) & K2 \\ 
8150.048 & $K2$ & 16.342(0.004) & K2 \\ 
8150.068 & $K2$ & 16.334(0.004) & K2 \\ 
8150.088 & $K2$ & 16.333(0.004) & K2 \\ 
8150.109 & $K2$ & 16.326(0.004) & K2 \\ 
8150.129 & $K2$ & 16.312(0.004) & K2 \\ 
8150.150 & $K2$ & 16.306(0.004) & K2 \\ 
8150.170 & $K2$ & 16.295(0.004) & K2 \\ 
8150.191 & $K2$ & 16.290(0.004) & K2 \\ 
8150.211 & $K2$ & 16.289(0.004) & K2 \\ 
8150.232 & $K2$ & 16.274(0.004) & K2 \\ 
8150.252 & $K2$ & 16.273(0.004) & K2 \\ 
8150.272 & $K2$ & 16.259(0.004) & K2 \\ 
8150.293 & $K2$ & 16.254(0.004) & K2 \\ 
8150.313 & $K2$ & 16.245(0.004) & K2 \\ 
8150.375 & $K2$ & 16.225(0.004) & K2 \\ 
8150.395 & $K2$ & 16.216(0.004) & K2 \\ 
8150.415 & $K2$ & 16.201(0.004) & K2 \\ 
8150.436 & $K2$ & 16.191(0.004) & K2 \\ 
8150.456 & $K2$ & 16.194(0.004) & K2 \\ 
8150.477 & $K2$ & 16.190(0.004) & K2 \\ 
8150.497 & $K2$ & 16.174(0.004) & K2 \\ 
8150.518 & $K2$ & 16.168(0.004) & K2 \\ 
8150.538 & $K2$ & 16.160(0.004) & K2 \\ 
8150.558 & $K2$ & 16.157(0.004) & K2 \\ 
8150.579 & $K2$ & 16.149(0.004) & K2 \\ 
8150.599 & $K2$ & 16.144(0.004) & K2 \\ 
8150.620 & $K2$ & 16.139(0.004) & K2 \\ 
8150.640 & $K2$ & 16.127(0.004) & K2 \\ 
8150.661 & $K2$ & 16.116(0.004) & K2 \\ 
8150.681 & $K2$ & 16.110(0.004) & K2 \\ 
8150.701 & $K2$ & 16.103(0.004) & K2 \\ 
8150.722 & $K2$ & 16.104(0.004) & K2 \\ 
8150.742 & $K2$ & 16.089(0.004) & K2 \\ 
8150.763 & $K2$ & 16.080(0.003) & K2 \\ 
8150.783 & $K2$ & 16.071(0.003) & K2 \\ 
8150.804 & $K2$ & 16.067(0.003) & K2 \\ 
8150.845 & $K2$ & 16.054(0.003) & K2 \\ 
8150.865 & $K2$ & 16.043(0.003) & K2 \\ 
8150.885 & $K2$ & 16.034(0.003) & K2 \\ 
8150.906 & $K2$ & 16.027(0.003) & K2 \\ 
8150.926 & $K2$ & 16.021(0.003) & K2 \\ 
8150.947 & $K2$ & 16.014(0.003) & K2 \\ 
8150.967 & $K2$ & 16.001(0.003) & K2 \\ 
8150.988 & $K2$ & 16.001(0.003) & K2 \\ 
8151.008 & $K2$ & 15.997(0.003) & K2 \\ 
8151.028 & $K2$ & 15.985(0.003) & K2 \\ 
8151.049 & $K2$ & 15.981(0.003) & K2 \\ 
8151.069 & $K2$ & 15.975(0.003) & K2 \\ 
8151.090 & $K2$ & 15.968(0.003) & K2 \\ 
8151.110 & $K2$ & 15.959(0.003) & K2 \\ 
8151.131 & $K2$ & 15.951(0.003) & K2 \\ 
8151.151 & $K2$ & 15.947(0.003) & K2 \\ 
8151.171 & $K2$ & 15.939(0.003) & K2 \\ 
8151.192 & $K2$ & 15.930(0.003) & K2 \\ 
8151.212 & $K2$ & 15.923(0.003) & K2 \\ 
8151.233 & $K2$ & 15.919(0.003) & K2 \\ 
8151.253 & $K2$ & 15.898(0.003) & K2 \\ 
8151.274 & $K2$ & 15.902(0.003) & K2 \\ 
8151.294 & $K2$ & 15.897(0.003) & K2 \\ 
8151.335 & $K2$ & 15.882(0.003) & K2 \\ 
8151.355 & $K2$ & 15.870(0.003) & K2 \\ 
8151.376 & $K2$ & 15.872(0.003) & K2 \\ 
8151.396 & $K2$ & 15.859(0.003) & K2 \\ 
8151.417 & $K2$ & 15.858(0.003) & K2 \\ 
8151.437 & $K2$ & 15.849(0.003) & K2 \\ 
8151.458 & $K2$ & 15.844(0.003) & K2 \\ 
8151.478 & $K2$ & 15.838(0.003) & K2 \\ 
8151.498 & $K2$ & 15.831(0.003) & K2 \\ 
8151.519 & $K2$ & 15.825(0.003) & K2 \\ 
8151.539 & $K2$ & 15.816(0.003) & K2 \\ 
8151.560 & $K2$ & 15.811(0.003) & K2 \\ 
8151.580 & $K2$ & 15.804(0.003) & K2 \\ 
8151.601 & $K2$ & 15.799(0.003) & K2 \\ 
8151.621 & $K2$ & 15.794(0.003) & K2 \\ 
8151.641 & $K2$ & 15.789(0.003) & K2 \\ 
8151.662 & $K2$ & 15.777(0.003) & K2 \\ 
8151.682 & $K2$ & 15.772(0.003) & K2 \\ 
8151.703 & $K2$ & 15.766(0.003) & K2 \\ 
8151.723 & $K2$ & 15.759(0.003) & K2 \\ 
8151.744 & $K2$ & 15.755(0.003) & K2 \\ 
8151.764 & $K2$ & 15.746(0.003) & K2 \\ 
8151.784 & $K2$ & 15.743(0.003) & K2 \\ 
8151.805 & $K2$ & 15.738(0.003) & K2 \\ 
8151.846 & $K2$ & 15.723(0.003) & K2 \\ 
8151.866 & $K2$ & 15.716(0.002) & K2 \\ 
8151.887 & $K2$ & 15.712(0.002) & K2 \\ 
8151.907 & $K2$ & 15.706(0.002) & K2 \\ 
8151.928 & $K2$ & 15.700(0.002) & K2 \\ 
8151.948 & $K2$ & 15.695(0.002) & K2 \\ 
8151.968 & $K2$ & 15.687(0.002) & K2 \\ 
8152.030 & $K2$ & 15.675(0.002) & K2 \\ 
8152.091 & $K2$ & 15.646(0.002) & K2 \\ 
8152.152 & $K2$ & 15.628(0.002) & K2 \\ 
8152.173 & $K2$ & 15.625(0.002) & K2 \\ 
8152.193 & $K2$ & 15.615(0.002) & K2 \\ 
8152.214 & $K2$ & 15.610(0.002) & K2 \\ 
8152.234 & $K2$ & 15.605(0.002) & K2 \\ 
8152.254 & $K2$ & 15.603(0.002) & K2 \\ 
8152.275 & $K2$ & 15.597(0.002) & K2 \\ 
8152.336 & $K2$ & 15.576(0.002) & K2 \\ 
8152.357 & $K2$ & 15.570(0.002) & K2 \\ 
8152.377 & $K2$ & 15.566(0.002) & K2 \\ 
8152.397 & $K2$ & 15.560(0.002) & K2 \\ 
8152.418 & $K2$ & 15.556(0.002) & K2 \\ 
8152.520 & $K2$ & 15.528(0.002) & K2 \\ 
8152.581 & $K2$ & 15.508(0.002) & K2 \\ 
8152.602 & $K2$ & 15.504(0.002) & K2 \\ 
8152.622 & $K2$ & 15.496(0.002) & K2 \\ 
8152.643 & $K2$ & 15.492(0.002) & K2 \\ 
8152.663 & $K2$ & 15.482(0.002) & K2 \\ 
8152.684 & $K2$ & 15.480(0.002) & K2 \\ 
8152.704 & $K2$ & 15.477(0.002) & K2 \\ 
8152.745 & $K2$ & 15.465(0.002) & K2 \\ 
8152.765 & $K2$ & 15.462(0.002) & K2 \\ 
8152.786 & $K2$ & 15.456(0.002) & K2 \\ 
8152.806 & $K2$ & 15.449(0.002) & K2 \\ 
8152.827 & $K2$ & 15.445(0.002) & K2 \\ 
8152.847 & $K2$ & 15.440(0.002) & K2 \\ 
8152.867 & $K2$ & 15.435(0.002) & K2 \\ 
8152.888 & $K2$ & 15.430(0.002) & K2 \\ 
8152.908 & $K2$ & 15.428(0.002) & K2 \\ 
8152.929 & $K2$ & 15.419(0.002) & K2 \\ 
8152.949 & $K2$ & 15.419(0.002) & K2 \\ 
8152.970 & $K2$ & 15.409(0.002) & K2 \\ 
8152.990 & $K2$ & 15.406(0.002) & K2 \\ 
8153.010 & $K2$ & 15.402(0.002) & K2 \\ 
8153.051 & $K2$ & 15.385(0.002) & K2 \\ 
8153.072 & $K2$ & 15.386(0.002) & K2 \\ 
8153.092 & $K2$ & 15.381(0.002) & K2 \\ 
8153.113 & $K2$ & 15.374(0.002) & K2 \\ 
8153.133 & $K2$ & 15.365(0.002) & K2 \\ 
8153.154 & $K2$ & 15.363(0.002) & K2 \\ 
8153.174 & $K2$ & 15.358(0.002) & K2 \\ 
8153.194 & $K2$ & 15.351(0.002) & K2 \\ 
8153.215 & $K2$ & 15.349(0.002) & K2 \\ 
8153.235 & $K2$ & 15.345(0.002) & K2 \\ 
8153.256 & $K2$ & 15.335(0.002) & K2 \\ 
8153.276 & $K2$ & 15.333(0.002) & K2 \\ 
8153.297 & $K2$ & 15.332(0.002) & K2 \\ 
8153.317 & $K2$ & 15.325(0.002) & K2 \\ 
8153.337 & $K2$ & 15.317(0.002) & K2 \\ 
8153.358 & $K2$ & 15.313(0.002) & K2 \\ 
8153.378 & $K2$ & 15.312(0.002) & K2 \\ 
8153.399 & $K2$ & 15.309(0.002) & K2 \\ 
8153.419 & $K2$ & 15.306(0.002) & K2 \\ 
8153.440 & $K2$ & 15.300(0.002) & K2 \\ 
8153.460 & $K2$ & 15.296(0.002) & K2 \\ 
8153.480 & $K2$ & 15.291(0.002) & K2 \\ 
8153.501 & $K2$ & 15.286(0.002) & K2 \\ 
8153.521 & $K2$ & 15.285(0.002) & K2 \\ 
8153.542 & $K2$ & 15.279(0.002) & K2 \\ 
8153.562 & $K2$ & 15.274(0.002) & K2 \\ 
8153.583 & $K2$ & 15.273(0.002) & K2 \\ 
8153.603 & $K2$ & 15.268(0.002) & K2 \\ 
8153.623 & $K2$ & 15.264(0.002) & K2 \\ 
8153.644 & $K2$ & 15.256(0.002) & K2 \\ 
8153.664 & $K2$ & 15.253(0.002) & K2 \\ 
8153.685 & $K2$ & 15.250(0.002) & K2 \\ 
8153.705 & $K2$ & 15.248(0.002) & K2 \\ 
8153.726 & $K2$ & 15.236(0.002) & K2 \\ 
8153.746 & $K2$ & 15.240(0.002) & K2 \\ 
8153.787 & $K2$ & 15.224(0.002) & K2 \\ 
8153.807 & $K2$ & 15.218(0.002) & K2 \\ 
8153.828 & $K2$ & 15.213(0.002) & K2 \\ 
8153.848 & $K2$ & 15.212(0.002) & K2 \\ 
8153.869 & $K2$ & 15.208(0.002) & K2 \\ 
8153.910 & $K2$ & 15.196(0.002) & K2 \\ 
8153.930 & $K2$ & 15.195(0.002) & K2 \\ 
8153.950 & $K2$ & 15.190(0.002) & K2 \\ 
8153.971 & $K2$ & 15.185(0.002) & K2 \\ 
8153.991 & $K2$ & 15.185(0.002) & K2 \\ 
8154.012 & $K2$ & 15.178(0.002) & K2 \\ 
8154.032 & $K2$ & 15.173(0.002) & K2 \\ 
8154.053 & $K2$ & 15.170(0.002) & K2 \\ 
8154.073 & $K2$ & 15.165(0.002) & K2 \\ 
8154.093 & $K2$ & 15.165(0.002) & K2 \\ 
8154.114 & $K2$ & 15.160(0.001) & K2 \\ 
8154.134 & $K2$ & 15.152(0.001) & K2 \\ 
8154.155 & $K2$ & 15.152(0.001) & K2 \\ 
8154.175 & $K2$ & 15.148(0.001) & K2 \\ 
8154.196 & $K2$ & 15.145(0.001) & K2 \\ 
8154.216 & $K2$ & 15.141(0.001) & K2 \\ 
8154.237 & $K2$ & 15.138(0.001) & K2 \\ 
8154.277 & $K2$ & 15.126(0.001) & K2 \\ 
8154.298 & $K2$ & 15.120(0.001) & K2 \\ 
8154.318 & $K2$ & 15.118(0.001) & K2 \\ 
8154.339 & $K2$ & 15.110(0.001) & K2 \\ 
8154.359 & $K2$ & 15.110(0.001) & K2 \\ 
8154.380 & $K2$ & 15.103(0.001) & K2 \\ 
8154.400 & $K2$ & 15.100(0.001) & K2 \\ 
8154.420 & $K2$ & 15.099(0.001) & K2 \\ 
8154.441 & $K2$ & 15.096(0.001) & K2 \\ 
8154.461 & $K2$ & 15.091(0.001) & K2 \\ 
8154.482 & $K2$ & 15.085(0.001) & K2 \\ 
8154.502 & $K2$ & 15.086(0.001) & K2 \\ 
8154.523 & $K2$ & 15.079(0.001) & K2 \\ 
8154.543 & $K2$ & 15.078(0.001) & K2 \\ 
8154.563 & $K2$ & 15.074(0.001) & K2 \\ 
8154.584 & $K2$ & 15.068(0.001) & K2 \\ 
8154.604 & $K2$ & 15.064(0.001) & K2 \\ 
8154.625 & $K2$ & 15.061(0.001) & K2 \\ 
8154.645 & $K2$ & 15.059(0.001) & K2 \\ 
8154.666 & $K2$ & 15.058(0.001) & K2 \\ 
8154.686 & $K2$ & 15.053(0.001) & K2 \\ 
8154.706 & $K2$ & 15.049(0.001) & K2 \\ 
8154.727 & $K2$ & 15.048(0.001) & K2 \\ 
8154.768 & $K2$ & 15.035(0.001) & K2 \\ 
8154.788 & $K2$ & 15.031(0.001) & K2 \\ 
8154.809 & $K2$ & 15.028(0.001) & K2 \\ 
8154.829 & $K2$ & 15.024(0.001) & K2 \\ 
8154.850 & $K2$ & 15.023(0.001) & K2 \\ 
8154.870 & $K2$ & 15.017(0.001) & K2 \\ 
8154.890 & $K2$ & 15.016(0.001) & K2 \\ 
8154.911 & $K2$ & 15.012(0.001) & K2 \\ 
8154.931 & $K2$ & 15.008(0.001) & K2 \\ 
8154.952 & $K2$ & 15.005(0.001) & K2 \\ 
8154.972 & $K2$ & 15.001(0.001) & K2 \\ 
8154.993 & $K2$ & 15.001(0.001) & K2 \\ 
8155.013 & $K2$ & 14.997(0.001) & K2 \\ 
8155.033 & $K2$ & 14.991(0.001) & K2 \\ 
8155.054 & $K2$ & 14.991(0.001) & K2 \\ 
8155.074 & $K2$ & 14.987(0.001) & K2 \\ 
8155.095 & $K2$ & 14.981(0.001) & K2 \\ 
8155.115 & $K2$ & 14.980(0.001) & K2 \\ 
8155.136 & $K2$ & 14.978(0.001) & K2 \\ 
8155.156 & $K2$ & 14.973(0.001) & K2 \\ 
8155.176 & $K2$ & 14.974(0.001) & K2 \\ 
8155.197 & $K2$ & 14.969(0.001) & K2 \\ 
8155.217 & $K2$ & 14.966(0.001) & K2 \\ 
8155.238 & $K2$ & 14.962(0.001) & K2 \\ 
8155.258 & $K2$ & 14.961(0.001) & K2 \\ 
8155.279 & $K2$ & 14.957(0.001) & K2 \\ 
8155.299 & $K2$ & 14.956(0.001) & K2 \\ 
8155.340 & $K2$ & 14.950(0.001) & K2 \\ 
8155.360 & $K2$ & 14.948(0.001) & K2 \\ 
8155.381 & $K2$ & 14.944(0.001) & K2 \\ 
8155.401 & $K2$ & 14.942(0.001) & K2 \\ 
8155.422 & $K2$ & 14.938(0.001) & K2 \\ 
8155.442 & $K2$ & 14.930(0.001) & K2 \\ 
8155.463 & $K2$ & 14.933(0.001) & K2 \\ 
8155.524 & $K2$ & 14.921(0.001) & K2 \\ 
8155.544 & $K2$ & 14.919(0.001) & K2 \\ 
8155.565 & $K2$ & 14.917(0.001) & K2 \\ 
8155.585 & $K2$ & 14.913(0.001) & K2 \\ 
8155.606 & $K2$ & 14.911(0.001) & K2 \\ 
8155.626 & $K2$ & 14.909(0.001) & K2 \\ 
8155.646 & $K2$ & 14.905(0.001) & K2 \\ 
8155.667 & $K2$ & 14.900(0.001) & K2 \\ 
8155.687 & $K2$ & 14.898(0.001) & K2 \\ 
8155.708 & $K2$ & 14.897(0.001) & K2 \\ 
8155.769 & $K2$ & 14.886(0.001) & K2 \\ 
8155.789 & $K2$ & 14.882(0.001) & K2 \\ 
8155.810 & $K2$ & 14.881(0.001) & K2 \\ 
8155.851 & $K2$ & 14.874(0.001) & K2 \\ 
8156.035 & $K2$ & 14.849(0.001) & K2 \\ 
8156.055 & $K2$ & 14.848(0.001) & K2 \\ 
8156.076 & $K2$ & 14.845(0.001) & K2 \\ 
8156.096 & $K2$ & 14.843(0.001) & K2 \\ 
8156.116 & $K2$ & 14.840(0.001) & K2 \\ 
8156.137 & $K2$ & 14.838(0.001) & K2 \\ 
8156.157 & $K2$ & 14.835(0.001) & K2 \\ 
8156.178 & $K2$ & 14.835(0.001) & K2 \\ 
8156.198 & $K2$ & 14.830(0.001) & K2 \\ 
8156.259 & $K2$ & 14.822(0.001) & K2 \\ 
8156.280 & $K2$ & 14.821(0.001) & K2 \\ 
8156.300 & $K2$ & 14.821(0.001) & K2 \\ 
8156.321 & $K2$ & 14.817(0.001) & K2 \\ 
8156.341 & $K2$ & 14.813(0.001) & K2 \\ 
8156.402 & $K2$ & 14.808(0.001) & K2 \\ 
8156.423 & $K2$ & 14.807(0.001) & K2 \\ 
8156.443 & $K2$ & 14.803(0.001) & K2 \\ 
8156.484 & $K2$ & 14.799(0.001) & K2 \\ 
8156.505 & $K2$ & 14.796(0.001) & K2 \\ 
8156.525 & $K2$ & 14.795(0.001) & K2 \\ 
8156.546 & $K2$ & 14.792(0.001) & K2 \\ 
8156.566 & $K2$ & 14.791(0.001) & K2 \\ 
8156.586 & $K2$ & 14.789(0.001) & K2 \\ 
8156.607 & $K2$ & 14.787(0.001) & K2 \\ 
8156.627 & $K2$ & 14.785(0.001) & K2 \\ 
8156.648 & $K2$ & 14.781(0.001) & K2 \\ 
8156.668 & $K2$ & 14.780(0.001) & K2 \\ 
8156.689 & $K2$ & 14.777(0.001) & K2 \\ 
8156.729 & $K2$ & 14.769(0.001) & K2 \\ 
8156.750 & $K2$ & 14.770(0.001) & K2 \\ 
8156.791 & $K2$ & 14.766(0.001) & K2 \\ 
8156.852 & $K2$ & 14.759(0.001) & K2 \\ 
8156.872 & $K2$ & 14.758(0.001) & K2 \\ 
8156.893 & $K2$ & 14.756(0.001) & K2 \\ 
8156.913 & $K2$ & 14.754(0.001) & K2 \\ 
8156.934 & $K2$ & 14.751(0.001) & K2 \\ 
8156.954 & $K2$ & 14.750(0.001) & K2 \\ 
8156.975 & $K2$ & 14.746(0.001) & K2 \\ 
8156.995 & $K2$ & 14.746(0.001) & K2 \\ 
8157.015 & $K2$ & 14.745(0.001) & K2 \\ 
8157.036 & $K2$ & 14.743(0.001) & K2 \\ 
8157.056 & $K2$ & 14.740(0.001) & K2 \\ 
8157.077 & $K2$ & 14.739(0.001) & K2 \\ 
8157.097 & $K2$ & 14.739(0.001) & K2 \\ 
8157.118 & $K2$ & 14.736(0.001) & K2 \\ 
8157.138 & $K2$ & 14.734(0.001) & K2 \\ 
8157.159 & $K2$ & 14.731(0.001) & K2 \\ 
8157.179 & $K2$ & 14.731(0.001) & K2 \\ 
8157.302 & $K2$ & 14.716(0.001) & K2 \\ 
8157.342 & $K2$ & 14.711(0.001) & K2 \\ 
8157.363 & $K2$ & 14.711(0.001) & K2 \\ 
8157.383 & $K2$ & 14.709(0.001) & K2 \\ 
8157.404 & $K2$ & 14.706(0.001) & K2 \\ 
8157.424 & $K2$ & 14.705(0.001) & K2 \\ 
8157.445 & $K2$ & 14.704(0.001) & K2 \\ 
8157.465 & $K2$ & 14.700(0.001) & K2 \\ 
8157.485 & $K2$ & 14.701(0.001) & K2 \\ 
8157.506 & $K2$ & 14.698(0.001) & K2 \\ 
8157.547 & $K2$ & 14.695(0.001) & K2 \\ 
8157.567 & $K2$ & 14.695(0.001) & K2 \\ 
8157.588 & $K2$ & 14.693(0.001) & K2 \\ 
8157.710 & $K2$ & 14.679(0.001) & K2 \\ 
8157.731 & $K2$ & 14.680(0.001) & K2 \\ 
8157.751 & $K2$ & 14.676(0.001) & K2 \\ 
8157.772 & $K2$ & 14.675(0.001) & K2 \\ 
8157.792 & $K2$ & 14.676(0.001) & K2 \\ 
8157.812 & $K2$ & 14.673(0.001) & K2 \\ 
8157.833 & $K2$ & 14.672(0.001) & K2 \\ 
8157.853 & $K2$ & 14.671(0.001) & K2 \\ 
8157.874 & $K2$ & 14.667(0.001) & K2 \\ 
8157.894 & $K2$ & 14.664(0.001) & K2 \\ 
8157.915 & $K2$ & 14.664(0.001) & K2 \\ 
8157.955 & $K2$ & 14.661(0.001) & K2 \\ 
8157.976 & $K2$ & 14.660(0.001) & K2 \\ 
8157.996 & $K2$ & 14.659(0.001) & K2 \\ 
8158.017 & $K2$ & 14.656(0.001) & K2 \\ 
8158.037 & $K2$ & 14.655(0.001) & K2 \\ 
8158.058 & $K2$ & 14.654(0.001) & K2 \\ 
8158.078 & $K2$ & 14.653(0.001) & K2 \\ 
8158.098 & $K2$ & 14.650(0.001) & K2 \\ 
8158.119 & $K2$ & 14.647(0.001) & K2 \\ 
8158.139 & $K2$ & 14.647(0.001) & K2 \\ 
8158.160 & $K2$ & 14.645(0.001) & K2 \\ 
8158.201 & $K2$ & 14.644(0.001) & K2 \\ 
8158.221 & $K2$ & 14.643(0.001) & K2 \\ 
8158.241 & $K2$ & 14.640(0.001) & K2 \\ 
8158.262 & $K2$ & 14.638(0.001) & K2 \\ 
8158.282 & $K2$ & 14.635(0.001) & K2 \\ 
8158.303 & $K2$ & 14.636(0.001) & K2 \\ 
8158.323 & $K2$ & 14.634(0.001) & K2 \\ 
8158.344 & $K2$ & 14.633(0.001) & K2 \\ 
8158.364 & $K2$ & 14.630(0.001) & K2 \\ 
8158.385 & $K2$ & 14.630(0.001) & K2 \\ 
8158.405 & $K2$ & 14.629(0.001) & K2 \\ 
8158.425 & $K2$ & 14.628(0.001) & K2 \\ 
8158.446 & $K2$ & 14.625(0.001) & K2 \\ 
8158.466 & $K2$ & 14.624(0.001) & K2 \\ 
8158.487 & $K2$ & 14.622(0.001) & K2 \\ 
8158.507 & $K2$ & 14.622(0.001) & K2 \\ 
8158.528 & $K2$ & 14.622(0.001) & K2 \\ 
8158.548 & $K2$ & 14.621(0.001) & K2 \\ 
8158.568 & $K2$ & 14.618(0.001) & K2 \\ 
8158.589 & $K2$ & 14.618(0.001) & K2 \\ 
8158.609 & $K2$ & 14.616(0.001) & K2 \\ 
8158.630 & $K2$ & 14.615(0.001) & K2 \\ 
8158.650 & $K2$ & 14.613(0.001) & K2 \\ 
8158.671 & $K2$ & 14.612(0.001) & K2 \\ 
8158.691 & $K2$ & 14.612(0.001) & K2 \\ 
8158.711 & $K2$ & 14.611(0.001) & K2 \\ 
8158.732 & $K2$ & 14.609(0.001) & K2 \\ 
8158.752 & $K2$ & 14.608(0.001) & K2 \\ 
8158.773 & $K2$ & 14.608(0.001) & K2 \\ 
8158.793 & $K2$ & 14.606(0.001) & K2 \\ 
8158.814 & $K2$ & 14.605(0.001) & K2 \\ 
8158.834 & $K2$ & 14.604(0.001) & K2 \\ 
8158.855 & $K2$ & 14.605(0.001) & K2 \\ 
8158.875 & $K2$ & 14.601(0.001) & K2 \\ 
8158.895 & $K2$ & 14.601(0.001) & K2 \\ 
8158.936 & $K2$ & 14.596(0.001) & K2 \\ 
8158.957 & $K2$ & 14.594(0.001) & K2 \\ 
8158.977 & $K2$ & 14.594(0.001) & K2 \\ 
8158.998 & $K2$ & 14.591(0.001) & K2 \\ 
8159.059 & $K2$ & 14.588(0.001) & K2 \\ 
8159.079 & $K2$ & 14.587(0.001) & K2 \\ 
8159.100 & $K2$ & 14.585(0.001) & K2 \\ 
8159.120 & $K2$ & 14.585(0.001) & K2 \\ 
8159.141 & $K2$ & 14.583(0.001) & K2 \\ 
8159.181 & $K2$ & 14.581(0.001) & K2 \\ 
8159.202 & $K2$ & 14.582(0.001) & K2 \\ 
8159.222 & $K2$ & 14.578(0.001) & K2 \\ 
8159.243 & $K2$ & 14.581(0.001) & K2 \\ 
8159.263 & $K2$ & 14.578(0.001) & K2 \\ 
8159.284 & $K2$ & 14.578(0.001) & K2 \\ 
8159.304 & $K2$ & 14.577(0.001) & K2 \\ 
8159.324 & $K2$ & 14.576(0.001) & K2 \\ 
8159.345 & $K2$ & 14.575(0.001) & K2 \\ 
8159.365 & $K2$ & 14.575(0.001) & K2 \\ 
8159.386 & $K2$ & 14.572(0.001) & K2 \\ 
8159.406 & $K2$ & 14.572(0.001) & K2 \\ 
8159.427 & $K2$ & 14.573(0.001) & K2 \\ 
8159.468 & $K2$ & 14.570(0.001) & K2 \\ 
8159.488 & $K2$ & 14.569(0.001) & K2 \\ 
8159.508 & $K2$ & 14.568(0.001) & K2 \\ 
8159.529 & $K2$ & 14.568(0.001) & K2 \\ 
8159.549 & $K2$ & 14.568(0.001) & K2 \\ 
8159.570 & $K2$ & 14.567(0.001) & K2 \\ 
8159.590 & $K2$ & 14.566(0.001) & K2 \\ 
8159.611 & $K2$ & 14.565(0.001) & K2 \\ 
8159.631 & $K2$ & 14.565(0.001) & K2 \\ 
8159.672 & $K2$ & 14.561(0.001) & K2 \\ 
8159.692 & $K2$ & 14.559(0.001) & K2 \\ 
8159.713 & $K2$ & 14.557(0.001) & K2 \\ 
8159.733 & $K2$ & 14.557(0.001) & K2 \\ 
8159.754 & $K2$ & 14.556(0.001) & K2 \\ 
8159.774 & $K2$ & 14.555(0.001) & K2 \\ 
8159.794 & $K2$ & 14.554(0.001) & K2 \\ 
8159.815 & $K2$ & 14.553(0.001) & K2 \\ 
8159.835 & $K2$ & 14.553(0.001) & K2 \\ 
8159.856 & $K2$ & 14.552(0.001) & K2 \\ 
8159.876 & $K2$ & 14.552(0.001) & K2 \\ 
8159.897 & $K2$ & 14.550(0.001) & K2 \\ 
8159.917 & $K2$ & 14.549(0.001) & K2 \\ 
8159.937 & $K2$ & 14.548(0.001) & K2 \\ 
8159.958 & $K2$ & 14.548(0.001) & K2 \\ 
8159.978 & $K2$ & 14.547(0.001) & K2 \\ 
8159.999 & $K2$ & 14.545(0.001) & K2 \\ 
8160.019 & $K2$ & 14.547(0.001) & K2 \\ 
8160.040 & $K2$ & 14.545(0.001) & K2 \\ 
8160.060 & $K2$ & 14.544(0.001) & K2 \\ 
8160.081 & $K2$ & 14.543(0.001) & K2 \\ 
8160.101 & $K2$ & 14.542(0.001) & K2 \\ 
8160.121 & $K2$ & 14.540(0.001) & K2 \\ 
8160.162 & $K2$ & 14.540(0.001) & K2 \\ 
8160.183 & $K2$ & 14.539(0.001) & K2 \\ 
8160.203 & $K2$ & 14.540(0.001) & K2 \\ 
8160.224 & $K2$ & 14.538(0.001) & K2 \\ 
8160.244 & $K2$ & 14.537(0.001) & K2 \\ 
8160.264 & $K2$ & 14.537(0.001) & K2 \\ 
8160.285 & $K2$ & 14.534(0.001) & K2 \\ 
8160.305 & $K2$ & 14.537(0.001) & K2 \\ 
8160.326 & $K2$ & 14.535(0.001) & K2 \\ 
8160.346 & $K2$ & 14.536(0.001) & K2 \\ 
8160.367 & $K2$ & 14.535(0.001) & K2 \\ 
8160.407 & $K2$ & 14.533(0.001) & K2 \\ 
8160.428 & $K2$ & 14.531(0.001) & K2 \\ 
8160.448 & $K2$ & 14.531(0.001) & K2 \\ 
8160.469 & $K2$ & 14.530(0.001) & K2 \\ 
8160.489 & $K2$ & 14.530(0.001) & K2 \\ 
8160.510 & $K2$ & 14.528(0.001) & K2 \\ 
8160.530 & $K2$ & 14.528(0.001) & K2 \\ 
8160.550 & $K2$ & 14.527(0.001) & K2 \\ 
8160.571 & $K2$ & 14.525(0.001) & K2 \\ 
8160.591 & $K2$ & 14.527(0.001) & K2 \\ 
8160.612 & $K2$ & 14.526(0.001) & K2 \\ 
8160.632 & $K2$ & 14.524(0.001) & K2 \\ 
8160.653 & $K2$ & 14.524(0.001) & K2 \\ 
8160.673 & $K2$ & 14.523(0.001) & K2 \\ 
8160.694 & $K2$ & 14.523(0.001) & K2 \\ 
8160.714 & $K2$ & 14.522(0.001) & K2 \\ 
8160.734 & $K2$ & 14.522(0.001) & K2 \\ 
8160.755 & $K2$ & 14.523(0.001) & K2 \\ 
8160.775 & $K2$ & 14.522(0.001) & K2 \\ 
8160.796 & $K2$ & 14.520(0.001) & K2 \\ 
8160.816 & $K2$ & 14.521(0.001) & K2 \\ 
8160.837 & $K2$ & 14.519(0.001) & K2 \\ 
8160.857 & $K2$ & 14.519(0.001) & K2 \\ 
8160.877 & $K2$ & 14.520(0.001) & K2 \\ 
8160.898 & $K2$ & 14.518(0.001) & K2 \\ 
8160.918 & $K2$ & 14.517(0.001) & K2 \\ 
8160.939 & $K2$ & 14.517(0.001) & K2 \\ 
8160.959 & $K2$ & 14.518(0.001) & K2 \\ 
8160.980 & $K2$ & 14.517(0.001) & K2 \\ 
8161.000 & $K2$ & 14.516(0.001) & K2 \\ 
8161.020 & $K2$ & 14.516(0.001) & K2 \\ 
8161.041 & $K2$ & 14.515(0.001) & K2 \\ 
8161.061 & $K2$ & 14.514(0.001) & K2 \\ 
8161.082 & $K2$ & 14.516(0.001) & K2 \\ 
8161.102 & $K2$ & 14.515(0.001) & K2 \\ 
8161.143 & $K2$ & 14.512(0.001) & K2 \\ 
8161.163 & $K2$ & 14.512(0.001) & K2 \\ 
8161.184 & $K2$ & 14.511(0.001) & K2 \\ 
8161.204 & $K2$ & 14.511(0.001) & K2 \\ 
8161.225 & $K2$ & 14.510(0.001) & K2 \\ 
8161.245 & $K2$ & 14.509(0.001) & K2 \\ 
8161.266 & $K2$ & 14.509(0.001) & K2 \\ 
8161.286 & $K2$ & 14.512(0.001) & K2 \\ 
8161.307 & $K2$ & 14.507(0.001) & K2 \\ 
8161.327 & $K2$ & 14.507(0.001) & K2 \\ 
8161.368 & $K2$ & 14.509(0.001) & K2 \\ 
8161.388 & $K2$ & 14.508(0.001) & K2 \\ 
8161.409 & $K2$ & 14.507(0.001) & K2 \\ 
8161.429 & $K2$ & 14.508(0.001) & K2 \\ 
8161.450 & $K2$ & 14.507(0.001) & K2 \\ 
8161.470 & $K2$ & 14.507(0.001) & K2 \\ 
8161.490 & $K2$ & 14.506(0.001) & K2 \\ 
8161.511 & $K2$ & 14.507(0.001) & K2 \\ 
8161.531 & $K2$ & 14.506(0.001) & K2 \\ 
8161.552 & $K2$ & 14.504(0.001) & K2 \\ 
8161.572 & $K2$ & 14.505(0.001) & K2 \\ 
8161.593 & $K2$ & 14.504(0.001) & K2 \\ 
8161.613 & $K2$ & 14.504(0.001) & K2 \\ 
8161.633 & $K2$ & 14.505(0.001) & K2 \\ 
8161.654 & $K2$ & 14.503(0.001) & K2 \\ 
8161.674 & $K2$ & 14.504(0.001) & K2 \\ 
8161.695 & $K2$ & 14.504(0.001) & K2 \\ 
8161.715 & $K2$ & 14.504(0.001) & K2 \\ 
8161.736 & $K2$ & 14.504(0.001) & K2 \\ 
8161.756 & $K2$ & 14.503(0.001) & K2 \\ 
8161.777 & $K2$ & 14.504(0.001) & K2 \\ 
8161.797 & $K2$ & 14.503(0.001) & K2 \\ 
8161.817 & $K2$ & 14.502(0.001) & K2 \\ 
8161.838 & $K2$ & 14.502(0.001) & K2 \\ 
8161.879 & $K2$ & 14.500(0.001) & K2 \\ 
8161.899 & $K2$ & 14.500(0.001) & K2 \\ 
8161.920 & $K2$ & 14.498(0.001) & K2 \\ 
8161.940 & $K2$ & 14.498(0.001) & K2 \\ 
8161.960 & $K2$ & 14.498(0.001) & K2 \\ 
8161.981 & $K2$ & 14.500(0.001) & K2 \\ 
8162.001 & $K2$ & 14.499(0.001) & K2 \\ 
8162.022 & $K2$ & 14.498(0.001) & K2 \\ 
8162.042 & $K2$ & 14.498(0.001) & K2 \\ 
8162.063 & $K2$ & 14.496(0.001) & K2 \\ 
8162.083 & $K2$ & 14.497(0.001) & K2 \\ 
8162.165 & $K2$ & 14.496(0.001) & K2 \\ 
8162.185 & $K2$ & 14.496(0.001) & K2 \\ 
8162.206 & $K2$ & 14.495(0.001) & K2 \\ 
8162.226 & $K2$ & 14.496(0.001) & K2 \\ 
8162.246 & $K2$ & 14.495(0.001) & K2 \\ 
8162.267 & $K2$ & 14.495(0.001) & K2 \\ 
8162.287 & $K2$ & 14.493(0.001) & K2 \\ 
8162.308 & $K2$ & 14.494(0.001) & K2 \\ 
8162.328 & $K2$ & 14.495(0.001) & K2 \\ 
8162.349 & $K2$ & 14.492(0.001) & K2 \\ 
8162.369 & $K2$ & 14.493(0.001) & K2 \\ 
8162.390 & $K2$ & 14.493(0.001) & K2 \\ 
8162.410 & $K2$ & 14.493(0.001) & K2 \\ 
8162.430 & $K2$ & 14.493(0.001) & K2 \\ 
8162.451 & $K2$ & 14.492(0.001) & K2 \\ 
8162.471 & $K2$ & 14.492(0.001) & K2 \\ 
8162.492 & $K2$ & 14.492(0.001) & K2 \\ 
8162.512 & $K2$ & 14.491(0.001) & K2 \\ 
8162.533 & $K2$ & 14.492(0.001) & K2 \\ 
8162.553 & $K2$ & 14.492(0.001) & K2 \\ 
8162.573 & $K2$ & 14.492(0.001) & K2 \\ 
8162.594 & $K2$ & 14.492(0.001) & K2 \\ 
8162.614 & $K2$ & 14.492(0.001) & K2 \\ 
8162.635 & $K2$ & 14.491(0.001) & K2 \\ 
8162.655 & $K2$ & 14.491(0.001) & K2 \\ 
8162.676 & $K2$ & 14.492(0.001) & K2 \\ 
8162.696 & $K2$ & 14.491(0.001) & K2 \\ 
8162.716 & $K2$ & 14.492(0.001) & K2 \\ 
8162.737 & $K2$ & 14.491(0.001) & K2 \\ 
8162.757 & $K2$ & 14.491(0.001) & K2 \\ 
8162.778 & $K2$ & 14.492(0.001) & K2 \\ 
8162.798 & $K2$ & 14.493(0.001) & K2 \\ 
8162.819 & $K2$ & 14.492(0.001) & K2 \\ 
8162.839 & $K2$ & 14.491(0.001) & K2 \\ 
8162.859 & $K2$ & 14.490(0.001) & K2 \\ 
8162.880 & $K2$ & 14.491(0.001) & K2 \\ 
8162.900 & $K2$ & 14.491(0.001) & K2 \\ 
8162.921 & $K2$ & 14.491(0.001) & K2 \\ 
8162.941 & $K2$ & 14.491(0.001) & K2 \\ 
8162.962 & $K2$ & 14.492(0.001) & K2 \\ 
8162.982 & $K2$ & 14.490(0.001) & K2 \\ 
8163.003 & $K2$ & 14.492(0.001) & K2 \\ 
8163.023 & $K2$ & 14.490(0.001) & K2 \\ 
8163.043 & $K2$ & 14.490(0.001) & K2 \\ 
8163.064 & $K2$ & 14.491(0.001) & K2 \\ 
8163.084 & $K2$ & 14.490(0.001) & K2 \\ 
8163.105 & $K2$ & 14.491(0.001) & K2 \\ 
8163.125 & $K2$ & 14.492(0.001) & K2 \\ 
8163.146 & $K2$ & 14.490(0.001) & K2 \\ 
8163.166 & $K2$ & 14.491(0.001) & K2 \\ 
8163.207 & $K2$ & 14.491(0.001) & K2 \\ 
8163.227 & $K2$ & 14.490(0.001) & K2 \\ 
8163.248 & $K2$ & 14.491(0.001) & K2 \\ 
8163.268 & $K2$ & 14.491(0.001) & K2 \\ 
8163.289 & $K2$ & 14.491(0.001) & K2 \\ 
8163.309 & $K2$ & 14.491(0.001) & K2 \\ 
8163.329 & $K2$ & 14.492(0.001) & K2 \\ 
8163.350 & $K2$ & 14.492(0.001) & K2 \\ 
8163.370 & $K2$ & 14.491(0.001) & K2 \\ 
8163.391 & $K2$ & 14.491(0.001) & K2 \\ 
8163.411 & $K2$ & 14.492(0.001) & K2 \\ 
8163.432 & $K2$ & 14.492(0.001) & K2 \\ 
8163.452 & $K2$ & 14.492(0.001) & K2 \\ 
8163.472 & $K2$ & 14.492(0.001) & K2 \\ 
8163.493 & $K2$ & 14.492(0.001) & K2 \\ 
8163.513 & $K2$ & 14.491(0.001) & K2 \\ 
8163.534 & $K2$ & 14.492(0.001) & K2 \\ 
8163.554 & $K2$ & 14.491(0.001) & K2 \\ 
8163.575 & $K2$ & 14.493(0.001) & K2 \\ 
8163.595 & $K2$ & 14.492(0.001) & K2 \\ 
8163.616 & $K2$ & 14.493(0.001) & K2 \\ 
8163.636 & $K2$ & 14.491(0.001) & K2 \\ 
8163.656 & $K2$ & 14.494(0.001) & K2 \\ 
8163.677 & $K2$ & 14.492(0.001) & K2 \\ 
8163.697 & $K2$ & 14.492(0.001) & K2 \\ 
8163.718 & $K2$ & 14.493(0.001) & K2 \\ 
8163.738 & $K2$ & 14.493(0.001) & K2 \\ 
8163.759 & $K2$ & 14.493(0.001) & K2 \\ 
8163.779 & $K2$ & 14.493(0.001) & K2 \\ 
8163.799 & $K2$ & 14.493(0.001) & K2 \\ 
8163.820 & $K2$ & 14.493(0.001) & K2 \\ 
8163.840 & $K2$ & 14.493(0.001) & K2 \\ 
8163.861 & $K2$ & 14.494(0.001) & K2 \\ 
8163.881 & $K2$ & 14.496(0.001) & K2 \\ 
8163.902 & $K2$ & 14.494(0.001) & K2 \\ 
8163.922 & $K2$ & 14.495(0.001) & K2 \\ 
8163.942 & $K2$ & 14.494(0.001) & K2 \\ 
8163.963 & $K2$ & 14.495(0.001) & K2 \\ 
8163.983 & $K2$ & 14.494(0.001) & K2 \\ 
8164.004 & $K2$ & 14.494(0.001) & K2 \\ 
8164.024 & $K2$ & 14.495(0.001) & K2 \\ 
8164.045 & $K2$ & 14.494(0.001) & K2 \\ 
8164.086 & $K2$ & 14.496(0.001) & K2 \\ 
8164.106 & $K2$ & 14.496(0.001) & K2 \\ 
8164.126 & $K2$ & 14.496(0.001) & K2 \\ 
8164.147 & $K2$ & 14.496(0.001) & K2 \\ 
8164.167 & $K2$ & 14.497(0.001) & K2 \\ 
8164.188 & $K2$ & 14.496(0.001) & K2 \\ 
8164.208 & $K2$ & 14.496(0.001) & K2 \\ 
8164.229 & $K2$ & 14.497(0.001) & K2 \\ 
8164.249 & $K2$ & 14.498(0.001) & K2 \\ 
8164.269 & $K2$ & 14.497(0.001) & K2 \\ 
8164.290 & $K2$ & 14.497(0.001) & K2 \\ 
8164.310 & $K2$ & 14.498(0.001) & K2 \\ 
8164.331 & $K2$ & 14.498(0.001) & K2 \\ 
8164.351 & $K2$ & 14.498(0.001) & K2 \\ 
8164.372 & $K2$ & 14.498(0.001) & K2 \\ 
8164.392 & $K2$ & 14.497(0.001) & K2 \\ 
8164.412 & $K2$ & 14.498(0.001) & K2 \\ 
8164.433 & $K2$ & 14.498(0.001) & K2 \\ 
8164.453 & $K2$ & 14.499(0.001) & K2 \\ 
8164.474 & $K2$ & 14.499(0.001) & K2 \\ 
8164.494 & $K2$ & 14.501(0.001) & K2 \\ 
8164.515 & $K2$ & 14.499(0.001) & K2 \\ 
8164.535 & $K2$ & 14.500(0.001) & K2 \\ 
8164.555 & $K2$ & 14.501(0.001) & K2 \\ 
8164.576 & $K2$ & 14.502(0.001) & K2 \\ 
8164.596 & $K2$ & 14.501(0.001) & K2 \\ 
8164.617 & $K2$ & 14.501(0.001) & K2 \\ 
8164.637 & $K2$ & 14.500(0.001) & K2 \\ 
8164.658 & $K2$ & 14.502(0.001) & K2 \\ 
8164.678 & $K2$ & 14.501(0.001) & K2 \\ 
8164.699 & $K2$ & 14.503(0.001) & K2 \\ 
8164.719 & $K2$ & 14.503(0.001) & K2 \\ 
8164.739 & $K2$ & 14.503(0.001) & K2 \\ 
8164.760 & $K2$ & 14.503(0.001) & K2 \\ 
8164.780 & $K2$ & 14.505(0.001) & K2 \\ 
8164.801 & $K2$ & 14.504(0.001) & K2 \\ 
8164.821 & $K2$ & 14.503(0.001) & K2 \\ 
8164.842 & $K2$ & 14.504(0.001) & K2 \\ 
8164.862 & $K2$ & 14.505(0.001) & K2 \\ 
8164.882 & $K2$ & 14.505(0.001) & K2 \\ 
8164.923 & $K2$ & 14.505(0.001) & K2 \\ 
8164.944 & $K2$ & 14.505(0.001) & K2 \\ 
8164.964 & $K2$ & 14.506(0.001) & K2 \\ 
8164.985 & $K2$ & 14.506(0.001) & K2 \\ 
8165.005 & $K2$ & 14.506(0.001) & K2 \\ 
8165.025 & $K2$ & 14.507(0.001) & K2 \\ 
8165.046 & $K2$ & 14.507(0.001) & K2 \\ 
8165.066 & $K2$ & 14.508(0.001) & K2 \\ 
8165.087 & $K2$ & 14.510(0.001) & K2 \\ 
8165.107 & $K2$ & 14.508(0.001) & K2 \\ 
8165.128 & $K2$ & 14.508(0.001) & K2 \\ 
8165.148 & $K2$ & 14.508(0.001) & K2 \\ 
8165.168 & $K2$ & 14.509(0.001) & K2 \\ 
8165.189 & $K2$ & 14.509(0.001) & K2 \\ 
8165.209 & $K2$ & 14.511(0.001) & K2 \\ 
8165.230 & $K2$ & 14.509(0.001) & K2 \\ 
8165.250 & $K2$ & 14.510(0.001) & K2 \\ 
8165.271 & $K2$ & 14.510(0.001) & K2 \\ 
8165.291 & $K2$ & 14.511(0.001) & K2 \\ 
8165.312 & $K2$ & 14.510(0.001) & K2 \\ 
8165.332 & $K2$ & 14.512(0.001) & K2 \\ 
8165.352 & $K2$ & 14.513(0.001) & K2 \\ 
8165.373 & $K2$ & 14.513(0.001) & K2 \\ 
8165.393 & $K2$ & 14.514(0.001) & K2 \\ 
8165.414 & $K2$ & 14.513(0.001) & K2 \\ 
8165.434 & $K2$ & 14.514(0.001) & K2 \\ 
8165.455 & $K2$ & 14.512(0.001) & K2 \\ 
8165.475 & $K2$ & 14.515(0.001) & K2 \\ 
8165.495 & $K2$ & 14.517(0.001) & K2 \\ 
8165.516 & $K2$ & 14.517(0.001) & K2 \\ 
8165.536 & $K2$ & 14.515(0.001) & K2 \\ 
8165.557 & $K2$ & 14.516(0.001) & K2 \\ 
8165.577 & $K2$ & 14.516(0.001) & K2 \\ 
8165.598 & $K2$ & 14.517(0.001) & K2 \\ 
8165.618 & $K2$ & 14.517(0.001) & K2 \\ 
8165.638 & $K2$ & 14.518(0.001) & K2 \\ 
8165.659 & $K2$ & 14.519(0.001) & K2 \\ 
8165.679 & $K2$ & 14.519(0.001) & K2 \\ 
8165.700 & $K2$ & 14.519(0.001) & K2 \\ 
8165.720 & $K2$ & 14.520(0.001) & K2 \\ 
8165.741 & $K2$ & 14.520(0.001) & K2 \\ 
8165.761 & $K2$ & 14.522(0.001) & K2 \\ 
8165.781 & $K2$ & 14.521(0.001) & K2 \\ 
8165.802 & $K2$ & 14.521(0.001) & K2 \\ 
8165.822 & $K2$ & 14.523(0.001) & K2 \\ 
8165.843 & $K2$ & 14.523(0.001) & K2 \\ 
8165.863 & $K2$ & 14.524(0.001) & K2 \\ 
8165.884 & $K2$ & 14.524(0.001) & K2 \\ 
8165.904 & $K2$ & 14.525(0.001) & K2 \\ 
8165.925 & $K2$ & 14.525(0.001) & K2 \\ 
8165.945 & $K2$ & 14.526(0.001) & K2 \\ 
8165.965 & $K2$ & 14.526(0.001) & K2 \\ 
8165.986 & $K2$ & 14.528(0.001) & K2 \\ 
8166.006 & $K2$ & 14.527(0.001) & K2 \\ 
8166.068 & $K2$ & 14.528(0.001) & K2 \\ 
8166.088 & $K2$ & 14.527(0.001) & K2 \\ 
8166.108 & $K2$ & 14.528(0.001) & K2 \\ 
8166.129 & $K2$ & 14.528(0.001) & K2 \\ 
8166.190 & $K2$ & 14.530(0.001) & K2 \\ 
8166.211 & $K2$ & 14.531(0.001) & K2 \\ 
8166.231 & $K2$ & 14.532(0.001) & K2 \\ 
8166.251 & $K2$ & 14.533(0.001) & K2 \\ 
8166.272 & $K2$ & 14.532(0.001) & K2 \\ 
8166.292 & $K2$ & 14.532(0.001) & K2 \\ 
8166.313 & $K2$ & 14.534(0.001) & K2 \\ 
8166.333 & $K2$ & 14.534(0.001) & K2 \\ 
8166.354 & $K2$ & 14.534(0.001) & K2 \\ 
8166.374 & $K2$ & 14.535(0.001) & K2 \\ 
8166.394 & $K2$ & 14.536(0.001) & K2 \\ 
8166.415 & $K2$ & 14.535(0.001) & K2 \\ 
8166.435 & $K2$ & 14.537(0.001) & K2 \\ 
8166.456 & $K2$ & 14.538(0.001) & K2 \\ 
8166.476 & $K2$ & 14.538(0.001) & K2 \\ 
8166.497 & $K2$ & 14.538(0.001) & K2 \\ 
8166.517 & $K2$ & 14.539(0.001) & K2 \\ 
8166.538 & $K2$ & 14.539(0.001) & K2 \\ 
8166.558 & $K2$ & 14.541(0.001) & K2 \\ 
8166.578 & $K2$ & 14.541(0.001) & K2 \\ 
8166.599 & $K2$ & 14.541(0.001) & K2 \\ 
8166.619 & $K2$ & 14.543(0.001) & K2 \\ 
8166.640 & $K2$ & 14.544(0.001) & K2 \\ 
8166.660 & $K2$ & 14.543(0.001) & K2 \\ 
8166.681 & $K2$ & 14.544(0.001) & K2 \\ 
8166.701 & $K2$ & 14.545(0.001) & K2 \\ 
8166.721 & $K2$ & 14.546(0.001) & K2 \\ 
8166.742 & $K2$ & 14.545(0.001) & K2 \\ 
8166.783 & $K2$ & 14.549(0.001) & K2 \\ 
8166.803 & $K2$ & 14.547(0.001) & K2 \\ 
8166.824 & $K2$ & 14.548(0.001) & K2 \\ 
8166.844 & $K2$ & 14.550(0.001) & K2 \\ 
8166.864 & $K2$ & 14.549(0.001) & K2 \\ 
8166.885 & $K2$ & 14.552(0.001) & K2 \\ 
8166.905 & $K2$ & 14.551(0.001) & K2 \\ 
8166.926 & $K2$ & 14.551(0.001) & K2 \\ 
8166.946 & $K2$ & 14.553(0.001) & K2 \\ 
8166.967 & $K2$ & 14.553(0.001) & K2 \\ 
8167.028 & $K2$ & 14.553(0.001) & K2 \\ 
8167.048 & $K2$ & 14.554(0.001) & K2 \\ 
8167.069 & $K2$ & 14.554(0.001) & K2 \\ 
8167.089 & $K2$ & 14.556(0.001) & K2 \\ 
8167.110 & $K2$ & 14.557(0.001) & K2 \\ 
8167.130 & $K2$ & 14.553(0.001) & K2 \\ 
8167.151 & $K2$ & 14.557(0.001) & K2 \\ 
8167.171 & $K2$ & 14.557(0.001) & K2 \\ 
8167.191 & $K2$ & 14.559(0.001) & K2 \\ 
8167.212 & $K2$ & 14.559(0.001) & K2 \\ 
8167.232 & $K2$ & 14.559(0.001) & K2 \\ 
8167.253 & $K2$ & 14.560(0.001) & K2 \\ 
8167.273 & $K2$ & 14.561(0.001) & K2 \\ 
8167.294 & $K2$ & 14.561(0.001) & K2 \\ 
8167.314 & $K2$ & 14.562(0.001) & K2 \\ 
8167.334 & $K2$ & 14.563(0.001) & K2 \\ 
8167.355 & $K2$ & 14.563(0.001) & K2 \\ 
8167.375 & $K2$ & 14.565(0.001) & K2 \\ 
8167.396 & $K2$ & 14.565(0.001) & K2 \\ 
8167.416 & $K2$ & 14.567(0.001) & K2 \\ 
8167.437 & $K2$ & 14.567(0.001) & K2 \\ 
8167.457 & $K2$ & 14.566(0.001) & K2 \\ 
8167.477 & $K2$ & 14.568(0.001) & K2 \\ 
8167.498 & $K2$ & 14.570(0.001) & K2 \\ 
8167.518 & $K2$ & 14.570(0.001) & K2 \\ 
8167.539 & $K2$ & 14.571(0.001) & K2 \\ 
8167.559 & $K2$ & 14.572(0.001) & K2 \\ 
8167.580 & $K2$ & 14.572(0.001) & K2 \\ 
8167.600 & $K2$ & 14.571(0.001) & K2 \\ 
8167.621 & $K2$ & 14.574(0.001) & K2 \\ 
8167.641 & $K2$ & 14.574(0.001) & K2 \\ 
8167.661 & $K2$ & 14.575(0.001) & K2 \\ 
8167.682 & $K2$ & 14.577(0.001) & K2 \\ 
8167.702 & $K2$ & 14.575(0.001) & K2 \\ 
8167.723 & $K2$ & 14.578(0.001) & K2 \\ 
8167.784 & $K2$ & 14.579(0.001) & K2 \\ 
8167.804 & $K2$ & 14.579(0.001) & K2 \\ 
8167.825 & $K2$ & 14.580(0.001) & K2 \\ 
8167.845 & $K2$ & 14.580(0.001) & K2 \\ 
8167.866 & $K2$ & 14.581(0.001) & K2 \\ 
8167.886 & $K2$ & 14.580(0.001) & K2 \\ 
8167.907 & $K2$ & 14.582(0.001) & K2 \\ 
8167.927 & $K2$ & 14.585(0.001) & K2 \\ 
8167.947 & $K2$ & 14.584(0.001) & K2 \\ 
8167.968 & $K2$ & 14.586(0.001) & K2 \\ 
8168.009 & $K2$ & 14.587(0.001) & K2 \\ 
8168.029 & $K2$ & 14.585(0.001) & K2 \\ 
8168.050 & $K2$ & 14.588(0.001) & K2 \\ 
8168.070 & $K2$ & 14.588(0.001) & K2 \\ 
8168.090 & $K2$ & 14.588(0.001) & K2 \\ 
8168.111 & $K2$ & 14.588(0.001) & K2 \\ 
8168.131 & $K2$ & 14.589(0.001) & K2 \\ 
8168.152 & $K2$ & 14.592(0.001) & K2 \\ 
8168.172 & $K2$ & 14.592(0.001) & K2 \\ 
8168.193 & $K2$ & 14.594(0.001) & K2 \\ 
8168.213 & $K2$ & 14.593(0.001) & K2 \\ 
8168.234 & $K2$ & 14.595(0.001) & K2 \\ 
8168.254 & $K2$ & 14.596(0.001) & K2 \\ 
8168.274 & $K2$ & 14.596(0.001) & K2 \\ 
8168.295 & $K2$ & 14.598(0.001) & K2 \\ 
8168.315 & $K2$ & 14.599(0.001) & K2 \\ 
8168.336 & $K2$ & 14.599(0.001) & K2 \\ 
8168.356 & $K2$ & 14.600(0.001) & K2 \\ 
8168.377 & $K2$ & 14.599(0.001) & K2 \\ 
8168.417 & $K2$ & 14.601(0.001) & K2 \\ 
8168.438 & $K2$ & 14.604(0.001) & K2 \\ 
8168.458 & $K2$ & 14.604(0.001) & K2 \\ 
8168.479 & $K2$ & 14.604(0.001) & K2 \\ 
8168.499 & $K2$ & 14.605(0.001) & K2 \\ 
8168.520 & $K2$ & 14.607(0.001) & K2 \\ 
8168.540 & $K2$ & 14.607(0.001) & K2 \\ 
8168.560 & $K2$ & 14.608(0.001) & K2 \\ 
8168.581 & $K2$ & 14.609(0.001) & K2 \\ 
8168.601 & $K2$ & 14.610(0.001) & K2 \\ 
8168.622 & $K2$ & 14.610(0.001) & K2 \\ 
8168.642 & $K2$ & 14.613(0.001) & K2 \\ 
8168.663 & $K2$ & 14.611(0.001) & K2 \\ 
8168.683 & $K2$ & 14.613(0.001) & K2 \\ 
8168.703 & $K2$ & 14.615(0.001) & K2 \\ 
8168.744 & $K2$ & 14.617(0.001) & K2 \\ 
8168.765 & $K2$ & 14.615(0.001) & K2 \\ 
8168.785 & $K2$ & 14.617(0.001) & K2 \\ 
8168.806 & $K2$ & 14.619(0.001) & K2 \\ 
8168.826 & $K2$ & 14.619(0.001) & K2 \\ 
8168.847 & $K2$ & 14.621(0.001) & K2 \\ 
8168.867 & $K2$ & 14.622(0.001) & K2 \\ 
8168.887 & $K2$ & 14.621(0.001) & K2 \\ 
8168.908 & $K2$ & 14.624(0.001) & K2 \\ 
8168.928 & $K2$ & 14.624(0.001) & K2 \\ 
8168.949 & $K2$ & 14.624(0.001) & K2 \\ 
8168.969 & $K2$ & 14.625(0.001) & K2 \\ 
8168.990 & $K2$ & 14.625(0.001) & K2 \\ 
8169.010 & $K2$ & 14.627(0.001) & K2 \\ 
8169.030 & $K2$ & 14.629(0.001) & K2 \\ 
8169.051 & $K2$ & 14.628(0.001) & K2 \\ 
8169.071 & $K2$ & 14.631(0.001) & K2 \\ 
8169.092 & $K2$ & 14.632(0.001) & K2 \\ 
8169.112 & $K2$ & 14.633(0.001) & K2 \\ 
8169.133 & $K2$ & 14.633(0.001) & K2 \\ 
8169.153 & $K2$ & 14.636(0.001) & K2 \\ 
8169.173 & $K2$ & 14.637(0.001) & K2 \\ 
8169.194 & $K2$ & 14.636(0.001) & K2 \\ 
8169.235 & $K2$ & 14.637(0.001) & K2 \\ 
8169.255 & $K2$ & 14.638(0.001) & K2 \\ 
8169.276 & $K2$ & 14.637(0.001) & K2 \\ 
8169.296 & $K2$ & 14.639(0.001) & K2 \\ 
8169.317 & $K2$ & 14.642(0.001) & K2 \\ 
8169.337 & $K2$ & 14.640(0.001) & K2 \\ 
8169.357 & $K2$ & 14.643(0.001) & K2 \\ 
8169.378 & $K2$ & 14.643(0.001) & K2 \\ 
8169.398 & $K2$ & 14.643(0.001) & K2 \\ 
8169.419 & $K2$ & 14.646(0.001) & K2 \\ 
8169.439 & $K2$ & 14.646(0.001) & K2 \\ 
8169.460 & $K2$ & 14.647(0.001) & K2 \\ 
8169.480 & $K2$ & 14.650(0.001) & K2 \\ 
8169.500 & $K2$ & 14.650(0.001) & K2 \\ 
8169.521 & $K2$ & 14.650(0.001) & K2 \\ 
8169.541 & $K2$ & 14.653(0.001) & K2 \\ 
8169.562 & $K2$ & 14.653(0.001) & K2 \\ 
8169.582 & $K2$ & 14.654(0.001) & K2 \\ 
8169.603 & $K2$ & 14.655(0.001) & K2 \\ 
8169.623 & $K2$ & 14.657(0.001) & K2 \\ 
8169.643 & $K2$ & 14.658(0.001) & K2 \\ 
8169.664 & $K2$ & 14.660(0.001) & K2 \\ 
8169.684 & $K2$ & 14.660(0.001) & K2 \\ 
8169.725 & $K2$ & 14.660(0.001) & K2 \\ 
8169.746 & $K2$ & 14.660(0.001) & K2 \\ 
8169.766 & $K2$ & 14.662(0.001) & K2 \\ 
8169.786 & $K2$ & 14.663(0.001) & K2 \\ 
8169.807 & $K2$ & 14.663(0.001) & K2 \\ 
8169.827 & $K2$ & 14.666(0.001) & K2 \\ 
8169.848 & $K2$ & 14.666(0.001) & K2 \\ 
8169.868 & $K2$ & 14.667(0.001) & K2 \\ 
8169.889 & $K2$ & 14.668(0.001) & K2 \\ 
8169.909 & $K2$ & 14.670(0.001) & K2 \\ 
8169.930 & $K2$ & 14.669(0.001) & K2 \\ 
8169.970 & $K2$ & 14.672(0.001) & K2 \\ 
8169.991 & $K2$ & 14.671(0.001) & K2 \\ 
8170.011 & $K2$ & 14.674(0.001) & K2 \\ 
8170.032 & $K2$ & 14.677(0.001) & K2 \\ 
8170.052 & $K2$ & 14.676(0.001) & K2 \\ 
8170.073 & $K2$ & 14.678(0.001) & K2 \\ 
8170.093 & $K2$ & 14.678(0.001) & K2 \\ 
8170.113 & $K2$ & 14.679(0.001) & K2 \\ 
8170.134 & $K2$ & 14.680(0.001) & K2 \\ 
8170.154 & $K2$ & 14.681(0.001) & K2 \\ 
8170.175 & $K2$ & 14.683(0.001) & K2 \\ 
8170.195 & $K2$ & 14.682(0.001) & K2 \\ 
8170.216 & $K2$ & 14.685(0.001) & K2 \\ 
8170.236 & $K2$ & 14.685(0.001) & K2 \\ 
8170.256 & $K2$ & 14.687(0.001) & K2 \\ 
8170.277 & $K2$ & 14.688(0.001) & K2 \\ 
8170.297 & $K2$ & 14.689(0.001) & K2 \\ 
8170.318 & $K2$ & 14.690(0.001) & K2 \\ 
8170.338 & $K2$ & 14.692(0.001) & K2 \\ 
8170.359 & $K2$ & 14.693(0.001) & K2 \\ 
8170.379 & $K2$ & 14.694(0.001) & K2 \\ 
8170.399 & $K2$ & 14.696(0.001) & K2 \\ 
8170.420 & $K2$ & 14.697(0.001) & K2 \\ 
8170.461 & $K2$ & 14.696(0.001) & K2 \\ 
8170.481 & $K2$ & 14.699(0.001) & K2 \\ 
8170.502 & $K2$ & 14.701(0.001) & K2 \\ 
8170.522 & $K2$ & 14.700(0.001) & K2 \\ 
8170.543 & $K2$ & 14.700(0.001) & K2 \\ 
8170.563 & $K2$ & 14.702(0.001) & K2 \\ 
8170.583 & $K2$ & 14.704(0.001) & K2 \\ 
8170.604 & $K2$ & 14.705(0.001) & K2 \\ 
8170.624 & $K2$ & 14.707(0.001) & K2 \\ 
8170.645 & $K2$ & 14.710(0.001) & K2 \\ 
8170.665 & $K2$ & 14.709(0.001) & K2 \\ 
8170.686 & $K2$ & 14.708(0.001) & K2 \\ 
8170.706 & $K2$ & 14.711(0.001) & K2 \\ 
8170.726 & $K2$ & 14.712(0.001) & K2 \\ 
8170.747 & $K2$ & 14.713(0.001) & K2 \\ 
8170.767 & $K2$ & 14.716(0.001) & K2 \\ 
8170.788 & $K2$ & 14.716(0.001) & K2 \\ 
8170.808 & $K2$ & 14.718(0.001) & K2 \\ 
8170.829 & $K2$ & 14.718(0.001) & K2 \\ 
8170.849 & $K2$ & 14.721(0.001) & K2 \\ 
8170.869 & $K2$ & 14.722(0.001) & K2 \\ 
8170.890 & $K2$ & 14.723(0.001) & K2 \\ 
8170.910 & $K2$ & 14.724(0.001) & K2 \\ 
8170.972 & $K2$ & 14.726(0.001) & K2 \\ 
8170.992 & $K2$ & 14.726(0.001) & K2 \\ 
8171.012 & $K2$ & 14.727(0.001) & K2 \\ 
8171.053 & $K2$ & 14.732(0.001) & K2 \\ 
8171.074 & $K2$ & 14.732(0.001) & K2 \\ 
8171.094 & $K2$ & 14.734(0.001) & K2 \\ 
8171.115 & $K2$ & 14.734(0.001) & K2 \\ 
8171.135 & $K2$ & 14.735(0.001) & K2 \\ 
8171.156 & $K2$ & 14.737(0.001) & K2 \\ 
8171.176 & $K2$ & 14.741(0.001) & K2 \\ 
8171.196 & $K2$ & 14.741(0.001) & K2 \\ 
8171.217 & $K2$ & 14.742(0.001) & K2 \\ 
8171.237 & $K2$ & 14.742(0.001) & K2 \\ 
8171.258 & $K2$ & 14.745(0.001) & K2 \\ 
8171.278 & $K2$ & 14.745(0.001) & K2 \\ 
8171.299 & $K2$ & 14.748(0.001) & K2 \\ 
8171.319 & $K2$ & 14.748(0.001) & K2 \\ 
8171.339 & $K2$ & 14.749(0.001) & K2 \\ 
8171.360 & $K2$ & 14.752(0.001) & K2 \\ 
8171.380 & $K2$ & 14.752(0.001) & K2 \\ 
8171.401 & $K2$ & 14.753(0.001) & K2 \\ 
8171.442 & $K2$ & 14.754(0.001) & K2 \\ 
8171.462 & $K2$ & 14.757(0.001) & K2 \\ 
8171.482 & $K2$ & 14.757(0.001) & K2 \\ 
8171.503 & $K2$ & 14.758(0.001) & K2 \\ 
8171.523 & $K2$ & 14.760(0.001) & K2 \\ 
8171.544 & $K2$ & 14.761(0.001) & K2 \\ 
8171.564 & $K2$ & 14.763(0.001) & K2 \\ 
8171.585 & $K2$ & 14.764(0.001) & K2 \\ 
8171.605 & $K2$ & 14.765(0.001) & K2 \\ 
8171.626 & $K2$ & 14.767(0.001) & K2 \\ 
8171.646 & $K2$ & 14.768(0.001) & K2 \\ 
8171.687 & $K2$ & 14.768(0.001) & K2 \\ 
8171.707 & $K2$ & 14.772(0.001) & K2 \\ 
8171.728 & $K2$ & 14.770(0.001) & K2 \\ 
8171.748 & $K2$ & 14.774(0.001) & K2 \\ 
8171.769 & $K2$ & 14.775(0.001) & K2 \\ 
8171.789 & $K2$ & 14.774(0.001) & K2 \\ 
8171.809 & $K2$ & 14.776(0.001) & K2 \\ 
8171.830 & $K2$ & 14.778(0.001) & K2 \\ 
8171.850 & $K2$ & 14.780(0.001) & K2 \\ 
8171.871 & $K2$ & 14.780(0.001) & K2 \\ 
8171.891 & $K2$ & 14.782(0.001) & K2 \\ 
8171.952 & $K2$ & 14.787(0.001) & K2 \\ 
8171.973 & $K2$ & 14.788(0.001) & K2 \\ 
8171.993 & $K2$ & 14.788(0.001) & K2 \\ 
8172.014 & $K2$ & 14.790(0.001) & K2 \\ 
8172.034 & $K2$ & 14.792(0.001) & K2 \\ 
8172.055 & $K2$ & 14.792(0.001) & K2 \\ 
8172.075 & $K2$ & 14.794(0.001) & K2 \\ 
8172.095 & $K2$ & 14.795(0.001) & K2 \\ 
8172.116 & $K2$ & 14.796(0.001) & K2 \\ 
8172.136 & $K2$ & 14.799(0.001) & K2 \\ 
8172.177 & $K2$ & 14.800(0.001) & K2 \\ 
8172.198 & $K2$ & 14.802(0.001) & K2 \\ 
8172.218 & $K2$ & 14.802(0.001) & K2 \\ 
8172.239 & $K2$ & 14.805(0.001) & K2 \\ 
8172.259 & $K2$ & 14.804(0.001) & K2 \\ 
8172.279 & $K2$ & 14.808(0.001) & K2 \\ 
8172.300 & $K2$ & 14.807(0.001) & K2 \\ 
8172.320 & $K2$ & 14.811(0.001) & K2 \\ 
8172.341 & $K2$ & 14.809(0.001) & K2 \\ 
8172.361 & $K2$ & 14.812(0.001) & K2 \\ 
8172.382 & $K2$ & 14.814(0.001) & K2 \\ 
8172.422 & $K2$ & 14.814(0.001) & K2 \\ 
8172.443 & $K2$ & 14.815(0.001) & K2 \\ 
8172.463 & $K2$ & 14.817(0.001) & K2 \\ 
8172.484 & $K2$ & 14.819(0.001) & K2 \\ 
8172.504 & $K2$ & 14.820(0.001) & K2 \\ 
8172.525 & $K2$ & 14.823(0.001) & K2 \\ 
8172.545 & $K2$ & 14.823(0.001) & K2 \\ 
8172.565 & $K2$ & 14.826(0.001) & K2 \\ 
8172.586 & $K2$ & 14.828(0.001) & K2 \\ 
8172.606 & $K2$ & 14.829(0.001) & K2 \\ 
8172.627 & $K2$ & 14.830(0.001) & K2 \\ 
8172.668 & $K2$ & 14.832(0.001) & K2 \\ 
8172.688 & $K2$ & 14.833(0.001) & K2 \\ 
8172.708 & $K2$ & 14.833(0.001) & K2 \\ 
8172.729 & $K2$ & 14.837(0.001) & K2 \\ 
8172.749 & $K2$ & 14.837(0.001) & K2 \\ 
8172.770 & $K2$ & 14.839(0.001) & K2 \\ 
8172.790 & $K2$ & 14.841(0.001) & K2 \\ 
8172.811 & $K2$ & 14.840(0.001) & K2 \\ 
8172.831 & $K2$ & 14.843(0.001) & K2 \\ 
8172.852 & $K2$ & 14.844(0.001) & K2 \\ 
8172.872 & $K2$ & 14.847(0.001) & K2 \\ 
8172.913 & $K2$ & 14.847(0.001) & K2 \\ 
8172.933 & $K2$ & 14.848(0.001) & K2 \\ 
8172.954 & $K2$ & 14.849(0.001) & K2 \\ 
8172.974 & $K2$ & 14.852(0.001) & K2 \\ 
8172.995 & $K2$ & 14.854(0.001) & K2 \\ 
8173.015 & $K2$ & 14.855(0.001) & K2 \\ 
8173.035 & $K2$ & 14.856(0.001) & K2 \\ 
8173.056 & $K2$ & 14.856(0.001) & K2 \\ 
8173.076 & $K2$ & 14.858(0.001) & K2 \\ 
8173.097 & $K2$ & 14.861(0.001) & K2 \\ 
8173.117 & $K2$ & 14.862(0.001) & K2 \\ 
8173.138 & $K2$ & 14.865(0.001) & K2 \\ 
8173.158 & $K2$ & 14.866(0.001) & K2 \\ 
8173.178 & $K2$ & 14.869(0.001) & K2 \\ 
8173.199 & $K2$ & 14.869(0.001) & K2 \\ 
8173.219 & $K2$ & 14.871(0.001) & K2 \\ 
8173.240 & $K2$ & 14.870(0.001) & K2 \\ 
8173.260 & $K2$ & 14.872(0.001) & K2 \\ 
8173.281 & $K2$ & 14.876(0.001) & K2 \\ 
8173.301 & $K2$ & 14.877(0.001) & K2 \\ 
8173.321 & $K2$ & 14.878(0.001) & K2 \\ 
8173.342 & $K2$ & 14.877(0.001) & K2 \\ 
8173.403 & $K2$ & 14.881(0.001) & K2 \\ 
8173.424 & $K2$ & 14.884(0.001) & K2 \\ 
8173.444 & $K2$ & 14.883(0.001) & K2 \\ 
8173.465 & $K2$ & 14.890(0.001) & K2 \\ 
8173.485 & $K2$ & 14.887(0.001) & K2 \\ 
8173.505 & $K2$ & 14.889(0.001) & K2 \\ 
8173.526 & $K2$ & 14.890(0.001) & K2 \\ 
8173.546 & $K2$ & 14.893(0.001) & K2 \\ 
8173.567 & $K2$ & 14.893(0.001) & K2 \\ 
8173.587 & $K2$ & 14.895(0.001) & K2 \\ 
8173.608 & $K2$ & 14.897(0.001) & K2 \\ 
8173.648 & $K2$ & 14.899(0.001) & K2 \\ 
8173.669 & $K2$ & 14.900(0.001) & K2 \\ 
8173.689 & $K2$ & 14.900(0.001) & K2 \\ 
8173.710 & $K2$ & 14.901(0.001) & K2 \\ 
8173.730 & $K2$ & 14.904(0.001) & K2 \\ 
8173.751 & $K2$ & 14.905(0.001) & K2 \\ 
8173.771 & $K2$ & 14.907(0.001) & K2 \\ 
8173.791 & $K2$ & 14.909(0.001) & K2 \\ 
8173.812 & $K2$ & 14.911(0.001) & K2 \\ 
8173.832 & $K2$ & 14.911(0.001) & K2 \\ 
8173.853 & $K2$ & 14.913(0.001) & K2 \\ 
8173.894 & $K2$ & 14.915(0.001) & K2 \\ 
8173.914 & $K2$ & 14.916(0.001) & K2 \\ 
8173.934 & $K2$ & 14.919(0.001) & K2 \\ 
8173.955 & $K2$ & 14.918(0.001) & K2 \\ 
8173.975 & $K2$ & 14.921(0.001) & K2 \\ 
8173.996 & $K2$ & 14.923(0.001) & K2 \\ 
8174.016 & $K2$ & 14.926(0.001) & K2 \\ 
8174.037 & $K2$ & 14.927(0.001) & K2 \\ 
8174.057 & $K2$ & 14.925(0.001) & K2 \\ 
8174.078 & $K2$ & 14.929(0.001) & K2 \\ 
8174.098 & $K2$ & 14.929(0.001) & K2 \\ 
8174.139 & $K2$ & 14.931(0.001) & K2 \\ 
8174.159 & $K2$ & 14.933(0.001) & K2 \\ 
8174.180 & $K2$ & 14.934(0.001) & K2 \\ 
8174.200 & $K2$ & 14.936(0.001) & K2 \\ 
8174.221 & $K2$ & 14.937(0.001) & K2 \\ 
8174.241 & $K2$ & 14.938(0.001) & K2 \\ 
8148.053 & $o$ & 17.126(0.028) & ATLAS \\ 
8154.005 & $o$ & 15.454(0.006) & ATLAS \\ 
8158.082 & $o$ & 14.825(0.004) & ATLAS \\ 
8162.054 & $o$ & 14.750(0.003) & ATLAS \\ 
8166.079 & $o$ & 14.689(0.003) & ATLAS \\ 
8170.052 & $o$ & 14.882(0.004) & ATLAS \\ 
8183.941 & $o$ & 15.379(0.005) & ATLAS \\ 
8185.929 & $o$ & 15.621(0.006) & ATLAS \\ 
8205.895 & $o$ & 16.452(0.064) & ATLAS \\ 
8207.881 & $o$ & 16.162(0.020) & ATLAS \\ 
8213.879 & $o$ & 16.481(0.012) & ATLAS \\ 
8221.877 & $o$ & 16.820(0.014) & ATLAS \\ 
8243.769 & $o$ & 17.449(0.027) & ATLAS \\ 
8253.760 & $o$ & 17.844(0.035) & ATLAS \\ 
8257.763 & $o$ & 18.035(0.047) & ATLAS \\ 
8261.764 & $o$ & 18.046(0.156) & ATLAS \\ 
8263.781 & $o$ & 18.051(0.073) & ATLAS \\ 
\enddata \tablecomments{$V\--\textrm{band}$ photometry is calibrated in the Vega magnitude system. The Kepler and SDSS $g$-band photometry are calibrated in the AB magnitude system.} 
\label{tab:phot} 
\end{deluxetable} 

